Strategic Budget Selection in a Competitive Autobidding World

We study a game played between advertisers in an online ad platform. The platform sells ad impressions by first-price auction and provides autobidding algorithms that optimize bids on each advertiser's behalf, subject to advertiser constraints such as budgets. Crucially, these constraints are strategically chosen by the advertisers. The chosen constraints define an "inner'' budget-pacing game for the autobidders. Advertiser payoffs in the constraint-choosing "metagame'' are determined by the equilibrium reached by the autobidders. Advertiser preferences can be more general than what is implied by their constraints: we assume only that they have weakly decreasing marginal value for clicks and weakly increasing marginal disutility for spending money. Nevertheless, we show that at any pure Nash equilibrium of the metagame, the resulting allocation obtains at least half of the liquid welfare of any allocation and this bound is tight. We also obtain a 4-approximation for any mixed Nash equilibrium or Bayes-Nash equilibria. These results rely on the power to declare budgets: if advertisers can specify only a (linear) value per click or an ROI target but not a budget constraint, the approximation factor at equilibrium can be as bad as linear in the number of advertisers.

==> Notes/existence.tex <==
\section{Equilibrium Analysis}

In our metagame, there might exist multiple 
pure Nash equilibrium.

\begin{proposition}
    The pure Nash equilibrium is not necessarily unique.
\end{proposition}
\begin{proof}
    We analyze a toy example where there are 
two agents and each agents has quasi-linear utility, i.e., $\moneycost_i(\price) = \price$.
Without loss of generality, we assume $\val_1 > \val_2$.

Given reported budget profile $(\wealth_1, \wealth_2)$,
the allocation, pacing multiplier and price are 
summarized in \Cref{table:outcome quasi linear}.
\begin{table}
    \centering
    \begin{tabular}{c|c|c|c|c|c}
    & $\alloc_1$ & $\pacescalar_1$ 
    & $\alloc_2$ & $\pacescalar_2$ 
    & $\price$
    \\
    \hline
     $\wealth_1 + \wealth_2 \leq \val_2$    
     &  $\frac{\wealth_1}{\wealth_1 + \wealth_2}$ & $\frac{\wealth_1 + \wealth_2}{\val_1}$
     &  $\frac{\wealth_2}{\wealth_1 + \wealth_2}$ & $\frac{\wealth_1 + \wealth_2}{\val_2}$
     & $\wealth_1 + \wealth_2$
     \\
     \hline
     $\wealth_1 + \wealth_2 \geq \val_2$
     and 
     $\wealth_1 \leq \val_2$
     & $\frac{\wealth_1}{\val_2}$ & $\frac{\val_2}{\val_1}$
     & $1 - \frac{\wealth_1}{\val_2}$ & $1$
     & $\val_2$
     \\
     \hline
     $\wealth_1 \geq \val_2$
     & $1$ & $\frac{\min\{\wealth_1,\val_1\}}{\val_1}$
     & $0$ & $1$
     & $\min\{\wealth_1,\val_1\}$
    \end{tabular}
    \caption{Allocation, price, and pacing multiplier under
    budget profile $(\wealth_1, \wealth_2)$.}
    \label{table:outcome quasi linear}
\end{table}

\begin{claim}
$\wealth_1 = \wealth_2 = \val_2$ is a pure Nash equilibrium.
\end{claim}
\begin{proof}
Under budget profile $\wealth_1 = \wealth_2 = \val_2$,
agent 1 receives the whole item and pays $\val_2$.
Fixing agent 1's reported budget $\wealth_1 = \val_2$,
it can be verified that agent 2 always receives nothing
regardless of her reported budget $\wealth_2$.
Fixing agent 2's reported budget $\wealth_2 = \val_2$,
it can be verified that the price is at least $\val_2$
regardless of agent 1's reported budget $\wealth_1$, and her utility is maximized when $\wealth_1 = \val_2$.
\end{proof}

\begin{claim}
\label{claim:quasi linear inefficient equilibrium}
Suppose $(\val_1 + \val_2)\val_2 \geq \val_1^2$.
Then,
$\wealth_1 = \gamma\cdot \val_1$ and
$\wealth_2 = \gamma \cdot \val_2$ 
is a pure Nash equilibrium 
where $\gamma = \frac{\val_1\val_2}{(\val_1 + \val_2)^2}$.
\end{claim}
\begin{proof}
Note that $\wealth_1 + \wealth_2 = \frac{\val_1\val_2(\val_1 + \val_2)}{(\val_1 + \val_2)^2} \leq \val_2$.
Thus, the price is $\wealth_1 + \wealth_2$,
and each agent $i$ receives $\frac{\wealth_i}{\wealth_1 + \wealth_2}$ fraction of the item.
The utility of agent $1$ is 
\begin{align*}
    \util_1 = \frac{\wealth_1}{\wealth_1 + \wealth_2}\left(
    \val_1 - (\wealth_1 + \wealth_2)
    \right)
\end{align*}
Taking the derivative of $\util_1$ with respect to $\wealth_1$, we have 
\begin{align*}
    \frac{\partial \util_1}{\partial \wealth_1}
    = 
    \frac{\val_1 \wealth_2 - (\wealth_1 + \wealth_2)^2}{(\wealth_1 + \wealth_2)^2}
\end{align*}
which is maximized at $\wealth_1 = \gamma \cdot \val_1$ 
when $\wealth_2 = \gamma \cdot \val_2$.
Therefore, agent 1 has no incentive to deviate 
to any other $\wealth_1 \leq \val_2 - \wealth_2$.
To see that agent 1 has no incentive to deviate 
to any $\wealth_1 > \val_2 - \wealth_2$, 
note that her utility is maximized at $\wealth_1 = \val_2$ for all possible $\wealth_1 > \val_2 - \wealth_2$,
and this utility $\val_1 - \val_2$ 
is smaller than the utility $\frac{\val_1}{\val_1 + \val_2}(\val_1 - (\frac{\val_1\val_2}{\val_1 + \val_2}))$
at $\wealth_1 = \gamma\cdot \val_1$
under the assumption $(\val_1 + \val_2)\val_2 \geq \val_1^2$.

By similar calculation, it can be verified that
agent 2 has no incentive to deviate to any other $\wealth_2 \leq \val_2 - \wealth_1$.
To see that agent 2 has no incentive to deviate 
to any $\wealth_2 > \val_2 - \wealth_1$, 
note that her utility is upperbouned by 
the utility at $\wealth_2 = \val_2 - \wealth_1$.
\end{proof}
\end{proof}


In our metagame, the pure Nash equilibrium 
may not exist.

\begin{proposition}
     The pure Nash equilibrium do not necessarily exist.
\end{proposition}
\begin{proof}
    Consider a toy example where 
    there are two agents and two items.
    Each agent $i\in[2]$ has 
    a hard budget $\frac{1}{2}$
    and linear value 
    $\val_{ij} = 1 + \indicator{i=j}$
    for each item $j\in[2]$.
    To show that the pure Nash equilibrium does not exists, 
    we argue that for every possible allocation,
    it cannot be induced by a pure Nash equilibrium.
    In this argument, we consider two cases:
    (i) agent 1 wins one item;
    and (ii) agent 1 wins positive fraction from 
    both items.
    Note that due to symmetry of the example, 
    the remaining case (iii) that agent 1 wins positive fraction from one item is equivalent to case (ii) by switching the indexes of two agents.
    
    \paragraph{Case 1- agent 1 wins one item}
    In this case, we further divide it into two subcases.

    \paragraph{Case 1a- agent 1 wins item 1}
    In this case, agent 1 gets item 1 and agent 2 gets item 2.
    We prove that this outcome cannot be induced by pure Nash
    by contradiction.
    Suppose there exists a pure Nash induces this outcome. 
    Without loss of generality, we assume the payment of agent 1
    is weakly higher than agent 2.

    \paragraph{Case 1b- agent 1 wins item 2}

    \paragraph{Case (ii) - agent 1 wines positive fraction from both items}
\end{proof}

==> Notes/fpa-pacing.tex <==
\section{Pacing Equilibrium in First-price Auction}

We first revisit the model studied in 
\citet{CJNKOM-07,CKPSSSW-22}.

\subsection{Model}

There exists $n$ agents and $m$ items. 
Each agent $i$ has budget $\wealth_i$ and $\val_{ij}$ for each item $j$. 
\begin{definition}[\citealp{CKPSSSW-22}]
A set of \emph{budget-feasible first price pacing multipliers (BFPM)} is a tuple $(\pacescalar, \alloc)$ of pacing multipliers $\pacescalar_i\in[0,1]$
for each agent $i$, and fractional allocation $\alloc_{ij}\in[0,1]$ for each 
agent $i$ and item $j$, that satisfies the following properties
\begin{itemize}
    \item (Price) Per-unit price $\price_j = \max_{i} \pacescalar_i \val_{ij}$
    \item (Highest bid wins) 
    If $\alloc_{ij} > 0$, then $\pacescalar_i \val_{ij} = \price_j$
    \item (Budget feasible) $\sum_{j} \alloc_{ij}\price_j \leq \wealth_i$
    \item (Demanded goods sold completely)
    If $\price_j > 0$, then $\sum_{i}\alloc_{ij} = 1$
    \item (No overselling) $\sum_{i}\alloc_{ij}  \leq 1$
\end{itemize}
\end{definition}

Among all BFPM, \citet{CKPSSSW-22} are particularly interested in
pacing equilibrium where no agent is unnecessarily paced.

\begin{definition}[\citealp{CKPSSSW-22}]
A \emph{first price pacing equilibrium (FPPE)} is a BFPM tuple $(\pacescalar,\alloc)$
with this additional property:
\vspace{-1.5mm}
\begin{itemize}
    \item (No unnecessary pacing) If $\sum_{j}\alloc_{ij}\price_j < \wealth_i$,
    then $\pacescalar_i = 1$.
\end{itemize}
\end{definition}
Namely, a BFPM is FPPE if for
every agent who does not exhaust her budget,
her bid profile equals her value profile.

\begin{example}
Suppose there is a single item and a single agent.
The agent has value $\val = 1$ and budget $\wealth = \infty$.
The FPPE allocates the item to the agent and charge her a per-unit price equal to her value $\val = 1$.
\end{example}

\begin{theorem}[\citealp{CKPSSSW-22}]
For any problem instance, FPPE
\begin{itemize}
    \item always exists 
    \item is essentially unique, i.e., the pacing multipliers are unique
    \item maximizes revenue among all BFPM.
\end{itemize}
\end{theorem}


\subsection{Extension to First-price Auction with Anonymous Reserve}
First, we assume that there exists an (agent-)anonymous reserve prices $\reserve = (\reserve_1, \dots, \reserve_m)$.

\begin{definition}
A set of \emph{budget-feasible first price pacing multipliers with anonymous reserve $\reserve$} is a tuple $(\pacescalar, \alloc)$ of pacing multipliers $\pacescalar_i\in[0,1]$
for each agent $i$, and fractional allocation $\alloc_{ij}\in[0,1]$ for each 
agent $i$ and item $j$, that satisfies the following properties
\begin{itemize}
    \item (Price) Per-unit price $\price_j = 
    \max\{\max_{i} \pacescalar_i \val_{ij},
    \reserve_j\}$
    \item (Highest bid wins) 
    If $\alloc_{ij} > 0$, then $\pacescalar_i \val_{ij} = 
    \price_j$
    \item (Budget feasible) $\sum_{j} \alloc_{ij}\price_j \leq \wealth_i$
    \item (Demanded goods sold completely)
    If $\price_j > \reserve_j$, then $\sum_{i}\alloc_{ij} = 1$
    \item (No overselling) $\sum_{i}\alloc_{ij}  \leq 1$
\end{itemize}
A BFPM (with reserve $\reserve$) is FPPE (with reserve $\reserve$)
under additional properties:
\begin{itemize}
    \item (No unnecessary pacing) If $\sum_{j}\alloc_{ij}\price_j < \wealth_i$,
    then $\pacescalar_i = 1$.
    \item (Seller prefer)  For each 
    item $j$ with price $\price_j = \reserve_j$,
    if there exists an agent $i$ such that 
    $\sum_{\ell} \alloc_{i\ell}\price_j < \wealth_i$
    and $\pacescalar_i\val_{ij} = \price_j$,
    then $\sum_{i}\alloc_{ij} = 1$.
\end{itemize}
\end{definition}
Comparing to the definition of FPPE (without reserve),
the definition of FPPE (with reserve $\reserve$)
further impose an additional property (seller prefer).
This property ensures that  
for each item $j$ whose per-unit price $\price_j$ is binding at 
the reserve $\reserve_j$,
either (i) every winners (if exists) exhausts her budget; or (i) this item $j$ is sold completely.
Due to property (no unnecessary pacing), 
for such item $j$ with $\price_j = \reserve_j$,
if winner $i$ does not exhaust her budget, 
then $\val_{ij} = \price_j$ and thus this winner 
is indifferent between purchasing or not purchasing.
However, if $\price_j = \reserve_j> 0$,
the seller strictly prefer to sell item $j$ to 
winner $i$, which increases his revenue.

\subsubsection{Homogeneous Items}
To establish better understanding of pacing equilibrium under reserve,
here we consider a simplified settings with homogeneous items,
i.e., for each agent $i$, each item $j, j'$, $\val_{ij} = \val_{i,j'} 
\triangleq \val_i$.
Note that this is equivalent to multi-item first-price auction 
with additive (instead of unit-demand) agents. 
Without loss of generality, we assume that agents has monotone values,
i.e., $\val_1 \leq \val_2\leq\dots\leq \val_n$,
and 
reserves are also monotone 
i.e., $\reserve_1 \leq \reserve_2 \leq \dots\leq \reserve_m$.

% \smallskip
First, we show that FPPE (without reserve) is equivalent to selling at the market 
clearing price.
\begin{proposition}
\label{prop:FPPE market clearing no reserve}
In the homogeneous-item setting,
FPPE (without reserve) is equivalent to selling at the market clearing price.
\end{proposition}
\begin{proof}
In the homogeneous-item setting, 
by property (price),
FPPE has identical per-unit price $\price_j \triangleq \price$
for every item $j$.
It is sufficient to show that $\price$ is the market clearing price,
i.e.,
$$\displaystyle\sum_{i:\val_i > \price} \frac{\wealth_i}{\price} \leq  m
\leq \displaystyle\sum_{i:\val_i \geq \price} \frac{\wealth_i}{\price}$$

Suppose $\price > 0$.\footnote{Price $\price = 0$ only happens in the 
degenerated instance where $\val_1 =\dots = \val_n = 0$.
It is straightforward to verify that the proposition statement holds in this case.}
Property (demand goods sold completely) implies that 
$\sum_{j}\sum_{i}\alloc_{ij} = m$.

Next we argue that 
(a) for each agent $i$ with value $\val_i < \price$, 
$\sum_{j}\alloc_{ij} = 0$;
(b) for each agent $i$ with value $\val_i> \price$, $\sum_j \alloc_{ij} = \frac{\wealth_i}{\price}$;
and (c) for each agent $i$ with value $\val_i =\price$,
$\sum_j \alloc_{ij} \leq \frac{\wealth_i}{\price}$.
Here (a) is guaranteed by property (highest bid wins);
(b) is guaranteed by property (price) and property (no unnecessary pacing);\footnote{Suppose agent $i$ has $\val_i > \price$.
By property (price), pacing multiplier $\pacescalar_i = \frac{\price}{\val_i} < 1$.
Invoking property (no unnecessary pacing), we have $\sum_j \alloc_{ij}\price = \wealth_i$.}
and (c) is guaranteed by property~(budget feasible).

Putting all pieces together,
\begin{align*}
    \sum_{i:\val_i > \price} \frac{\wealth_i}{\price} 
    \overset{(b)}{=}
    \sum_{i:\val_i > \price}\sum_j \alloc_{ij}
    \leq \sum_{i}\sum_{j}\alloc_{ij} = m
    \overset{(a)}{=}
    \sum_{i:\val_i \geq \price}\sum_{j}\alloc_{ij} 
    \overset{(c)}{\leq} \sum_{i:\val_i \geq \price} \frac{\wealth_i}{\price}
\end{align*}
as desired.
\end{proof}

\begin{theorem}[\citet{abr-06}]
In the homogeneous-item setting, selling at the market clearing price 
achieves at least half of optimal revenue (i.e., allowing to assign each agent,
each item a different per-unit price).
\end{theorem}

We can further extend the characterization of FPPE in \Cref{prop:FPPE market clearing no reserve} to FPPE with (agent-)anonymous reserve.
\begin{proposition}
\label{prop:FPPE market clearing}
In the homogeneous-item setting,
FPPE (with reserve $\reserve$) is equivalent to selling 
$\min\{\sum_{i:\val_i \geq \price}\frac{\wealth_i}{\price}, |\{j: \reserve_j \leq \price\}|\}$ units (of homogeneous items)
at per-unit price $\price$
such that\footnote{As a sanity check,
when there is no reserve (a.k.a., $\reserve_j \equiv 0$ for all item $j$), 
$|\{j: \reserve_j < \price\}| = |\{j: \reserve_j \leq \price\}| = m$, and 
thus $\price$ is indeed the market clearing price.}
\footnote{To see the existence of price $\price$,
note that $|\{j: \reserve_j \leq \price\}|$ is increasing in $\price$
from $0$ to $m$,
and $\sum_{i:\val_i > \price} \frac{\wealth_i}{\price}$ is decreasing from 
infinite to $0$. A formal argument will be added later.}
\begin{align*}
    \left[\sum_{i:\val_i > \price} \frac{\wealth_i}{\price},
    \sum_{i:\val_i \geq \price} \frac{\wealth_i}{\price}
    \right]
    \cap 
    \Big[
    |\{j: \reserve_j < \price\}|,
    |\{j: \reserve_j \leq \price\}|
    \Big] 
    \not= 
    \emptyset
\end{align*}
\end{proposition}
\begin{proof}
In the homogeneous-item setting, 
by property (price),
FPPE has identical per-unit price $\price_j \triangleq \price$
for every item $j$ with reserve $\reserve_j \leq \price$;
and per-unit price $\price_j = \reserve_j$
for other item $j$ with reserve $\reserve_j > \price$.

Property (demand goods sold completely) 
together with property (highest bid wins) implies that 

First, consider the allocation in FPPE, 
\begin{align*}
\sum_{j}\sum_{i}\alloc_{ij} &= 
\sum_{j:\reserve_j < \price}\sum_i \alloc_{ij} 
+
\sum_{j:\reserve_j = \price}\sum_i \alloc_{ij} 
+
\sum_{j:\reserve_j > \price}\sum_i \alloc_{ij} 
= |\{j:\reserve_j < \price\}|
+
\sum_{j:\reserve_j = \price}\sum_i \alloc_{ij} 
\end{align*}
where the second equality uses property (demand goods sold completely) and 
property (highest bid wins).
Combining with property (no overselling),
we conclude that 
\begin{align*}
    |\{j:\reserve_j < \price\}| 
    \leq \sum_{j}\sum_{i}\alloc_{ij} \leq 
    |\{j:\reserve_j \leq \price\}| 
\end{align*}
% It remains to show that $\sum_{j}\sum_{i}\alloc_{ij} =\min\{ \sum_{i:\val_i \geq \price}\frac{\wealth_i}{\price},
%     |\{j:\reserve_j \leq \price\}|\}$,
%     and 

Next we argue that 
(a) for each agent $i$ with value $\val_i < \price$, 
$\sum_{j}\alloc_{ij} = 0$;
(b) for each agent $i$ with value $\val_i> \price$, $\sum_j \alloc_{ij} = \frac{\wealth_i}{\price}$;
and (c) for each agent $i$ with value $\val_i =\price$,
$\sum_j \alloc_{ij} \leq \frac{\wealth_i}{\price}$.
Here (a) is guaranteed by property (highest bid wins);
(b) is guaranteed by property (price) and property (no unnecessary pacing);
and (c) is guaranteed by property~(budget feasible).
Thus,
\begin{align*}
    \sum_{i:\val_i > \price} \frac{\wealth_i}{\price} 
    \overset{(b)}{=}
    \sum_{i:\val_i > \price}\sum_j \alloc_{ij}
    \leq \sum_{i}\sum_{j}\alloc_{ij} 
    \overset{(a)}{=}
    \sum_{i:\val_i \geq \price}\sum_{j}\alloc_{ij} 
    \overset{(c)}{\leq} \sum_{i:\val_i \geq \price} \frac{\wealth_i}{\price}
\end{align*}
Therefore, we have 
\begin{align*}
    \left[\sum_{i:\val_i > \price} \frac{\wealth_i}{\price},
    \sum_{i:\val_i \geq \price} \frac{\wealth_i}{\price}
    \right]
    \cap 
    \Big[
    |\{j: \reserve_j < \price\}|,
    |\{j: \reserve_j \leq \price\}|
    \Big] 
    \not= 
    \emptyset
\end{align*}
To conclude the proof, note that 
$\sum_{i}\sum_{j}\alloc_{ij}  =
\min\{\sum_{i:\val_i \geq \price}\frac{\wealth_i}{\price}, |\{j: \reserve_j \leq \price\}|\}$
due to property (seller prefer)
\end{proof}

Note that \Cref{prop:FPPE market clearing} implies 
that FPPE without reserve maximizes the revenue.
\begin{corollary}
In the homogeneous-item setting,
for any (agent-)anonymous reserve $\reserve$,
the revenue of 
FPPE with reserve $\reserve$ 
is weakly smaller than the revenue in FPPE without 
reserve.
\end{corollary}

\begin{conjecture}
Reserve is not helpful even if items are hetergeneous.
\end{conjecture}
\newpage

==> Notes/metagame-SPA.tex <==
\section{Metagame in Second Price Auction}
\label{sec:metagame spa}
In this section, we consider the same setting
as \Cref{sec:metagame fpa}.
However, instead of competing 
in the first-price auction,
here we consider the second-price auction instead.

Each agent $i$ 
reports a hard budget $\wealth_i$ and 
the seller implements the allocation and payment profile 
induced by the second-price pacing equilibrium \citep{CKSS-22}
assuming each agent $i$ has valuation profile $\val_i$ and budget $\wealth_i$.
\begin{definition}[\citealp{CKSS-22}]
A set of \emph{budget-feasible second price pacing multiplier (BSPM)}
is a tuple $(\pacescalar, \allocs)$ of pacing multipliers $\pacescalar_i\in[0,1]$
for each agent $i$, and fractional allocation $\allocij\in[0,1]$ for each 
agent $i$ and item $j$, that satisfies the following properties
\begin{itemize}
    \item (Price) Per-unit price $\price_j$ 
    is second highest of $\{\pacescalar_i \valij\}_i$.
    \item (Highest bid wins) 
    If $\allocij > 0$, then $\pacescalar_i \valij = \max_{k} \pacescalar_k \val_{kj}$
    \item (Budget feasible) $\sum_j \allocij\price_j \leq \wealth_i$
    \item (Demanded goods sold completely)
    If $\price_j > 0$, then $\sum_{i}\alloc_{ij} = 1$
    \item (No overselling) $\sum_{i}\alloc_{ij}  \leq 1$ for each item $j$
    \end{itemize}
    A 
\emph{second price pacing equilibrium (SPPE)} 
is a BSPM which additionally satisfies
    \begin{itemize}
    \item (No unnecessary pacing) If $\sum_{j}\alloc_{ij}\price_j < \wealth_i$,
    then $\pacescalar_i = 1$.
\end{itemize}
\end{definition}

\citet{CKSS-22}
show that the SPPE always exists
but is not necessarily unique.
Furthermore, SPPE is a refinement of 
competitive equilibrium
for
(supply-aware) agents.\footnote{As a comparison,
FPPE is the unique
(equal-rates) competitive equilibrium
even for (supply-unaware) agents.}

Due to the non-uniqueness of SPPE, to ensure that 
the metagame is well-defined, we consider the following
two modeling assumptions:
\begin{enumerate}
    \item \emph{Metagame under a fixed SPPE selection rule}:
    let $\phi$ be a SPPE selection rule which maps from 
    the budget profile to a SPPE. 
    Fixing a budget profile, 
    each agent evaluates her utility under
    the allocation and payment induced by the SPPE selected by $\phi$.
    \item \emph{Metagame between pessimistic agents}:
    Fixing a budget profile, 
    each agent evaluates her utility under
    the allocation and payment induced by the worst SPPE (for her).
\end{enumerate}








==> Notes/metagame-budget.tex <==
\section{Meta Game between Advertisers}


There is a (divisible) item and $n$ agents (aka advertisers).
Each agent $i$ has value $\val_i$.
% a value function 
% $\val_i:[0, 1]\rightarrow\reals_+$ 
% mapping from her allocation to her value.
Each agent $i$ also has an outside option value for money, described by a function $\moneycost_i: \reals_+ \rightarrow \reals_+\cup\{\infty\}$, which is strictly increasing and weakly convex. 
Given allocation $\alloc_i$ and payment $\price_i$,
agent $i$ has utility $
    \util_i(\alloc_i, \price_i) = 
    % \val_i(\alloc) -
    \val_i \cdot \alloc_i -
    \moneycost_i(\price_i)$.\footnote{This model is 
    similar to the model considered in \citet{BCHNL-21}.}
    When $\moneycost_i$ is differentiable, we will write
 $\moneycostderivative_i(\price_i)$ for the derivative of
 $\moneycost_i$ at $\price_i$.
 Without loss of generality, we assume that $\moneycostderivative_i(0) = 1$ for every agent $i$.

All agents compete for the item 
in the first-price pacing game. 
In particular, 
each agent reports a hard budget $\wealth_i$ and 
the seller implements the allocation and payment profile 
induced by the first-price pacing equilibrium \citep{CKPSSSW-22}
assuming each agent $i$ has value $\val_i$ and budget $\wealth_i$.
In this section, we focus in the \emph{pure} Nash equilibrium of reported budget profile $(\wealth_1,\dots,\wealth_n)$.

\begin{definition}[\citealp{CKPSSSW-22}]
A set of \emph{first price pacing equilibrium (FPPE)} is a tuple $(\pacescalar, \alloc)$ of pacing multipliers $\pacescalar_i\in[0,1]$
for each agent $i$, and fractional allocation $\alloc_{i}\in[0,1]$ for each 
agent $i$, that satisfies the following properties
\begin{itemize}
    \item (Price) Per-unit price $\price = \max_{i} \pacescalar_i \val_{i}$
    \item (Highest bid wins) 
    If $\alloc_{i} > 0$, then $\pacescalar_i \val_{i} = \price$
    \item (Budget feasible) $\alloc_{i}\price \leq \wealth_i$
    \item (Demanded goods sold completely)
    If $\price > 0$, then $\sum_{i}\alloc_{i} = 1$
    \item (No overselling) $\sum_{i}\alloc_{i}  \leq 1$
    \item (No unnecessary pacing) If $\alloc_{i}\price < \wealth_i$,
    then $\pacescalar_i = 1$.
\end{itemize}
\end{definition}

\begin{theorem}[\citealp{CKPSSSW-22}]
For any problem instance, FPPE
exists and is essentially unique (i.e., the pacing multipliers and agents' quasi-linear hutility are unique).
\end{theorem}


Given allocation profile $\allocbf$, the \emph{transferable welfare}
is $\twelfare(\allocbf) = \sum_i \wtp_i(\alloc_i)$
where $\wtp_i(\alloc_i) = \moneycost^{-1}(\val_i\cdot\alloc_i)$ 
is agent $i$'s \emph{willingness to pay} for allocation $\alloc_i$.
Recall that $\moneycost_i$ is convex and its derivative
$\moneycostderivative_i(0) = 1$.
Hence, $\wtp_i(\alloc_i) \leq \val_i \cdot \alloc_i$
and thus transferable welfare is upperbounded by welfare.

\subsection{Warmup: two agents with quasi-linear utility}
In this subsection, we analyze a toy example where there are 
two agents and each agents has quasi-linear utility, i.e., $\moneycost_i(\price) = \price$.
Without loss of generality, we assume $\val_1 > \val_2$.

\paragraph{Allocation, pacing multiplier, and price under budget profile.}
Given reported budget profile $(\wealth_1, \wealth_2)$,
the allocation, pacing multiplier and price are 
summarized in \Cref{table:outcome quasi linear}.
\begin{table}
    \centering
    \begin{tabular}{c|c|c|c|c|c}
    & $\alloc_1$ & $\pacescalar_1$ 
    & $\alloc_2$ & $\pacescalar_2$ 
    & $\price$
    \\
    \hline
     $\wealth_1 + \wealth_2 \leq \val_2$    
     &  $\frac{\wealth_1}{\wealth_1 + \wealth_2}$ & $\frac{\wealth_1 + \wealth_2}{\val_1}$
     &  $\frac{\wealth_2}{\wealth_1 + \wealth_2}$ & $\frac{\wealth_1 + \wealth_2}{\val_2}$
     & $\wealth_1 + \wealth_2$
     \\
     \hline
     $\wealth_1 + \wealth_2 \geq \val_2$
     and 
     $\wealth_1 \leq \val_2$
     & $\frac{\wealth_1}{\val_2}$ & $\frac{\val_2}{\val_1}$
     & $1 - \frac{\wealth_1}{\val_2}$ & $1$
     & $\val_2$
     \\
     \hline
     $\wealth_1 \geq \val_2$
     & $1$ & $\frac{\min\{\wealth_1,\val_1\}}{\val_1}$
     & $0$ & $1$
     & $\min\{\wealth_1,\val_1\}$
    \end{tabular}
    \caption{Allocation, price, and pacing multiplier under
    budget profile $(\wealth_1, \wealth_2)$.}
    \label{table:outcome quasi linear}
\end{table}

\paragraph{Equilibrium analysis.}
\begin{claim}
$\wealth_1 = \wealth_2 = \val_2$ is a pure Nash equilibrium.
\end{claim}
\begin{proof}
Under budget profile $\wealth_1 = \wealth_2 = \val_2$,
agent 1 receives the whole item and pays $\val_2$.
Fixing agent 1's reported budget $\wealth_1 = \val_2$,
it can be verified that agent 2 always receives nothing
regardless of her reported budget $\wealth_2$.
Fixing agent 2's reported budget $\wealth_2 = \val_2$,
it can be verified that the price is at least $\val_2$
regardless of agent 1's reported budget $\wealth_1$, and her utility is maximized when $\wealth_1 = \val_2$.
\end{proof}

\begin{claim}
\label{claim:quasi linear inefficient equilibrium}
Suppose $(\val_1 + \val_2)\val_2 \geq \val_1^2$.
Then,
$\wealth_1 = \gamma\cdot \val_1$ and
$\wealth_2 = \gamma \cdot \val_2$ 
is a pure Nash equilibrium 
where $\gamma = \frac{\val_1\val_2}{(\val_1 + \val_2)^2}$.
\end{claim}
\begin{proof}
Note that $\wealth_1 + \wealth_2 = \frac{\val_1\val_2(\val_1 + \val_2)}{(\val_1 + \val_2)^2} \leq \val_2$.
Thus, the price is $\wealth_1 + \wealth_2$,
and each agent $i$ receives $\frac{\wealth_i}{\wealth_1 + \wealth_2}$ fraction of the item.
The utility of agent $1$ is 
\begin{align*}
    \util_1 = \frac{\wealth_1}{\wealth_1 + \wealth_2}\left(
    \val_1 - (\wealth_1 + \wealth_2)
    \right)
\end{align*}
Taking the derivative of $\util_1$ with respect to $\wealth_1$, we have 
\begin{align*}
    \frac{\partial \util_1}{\partial \wealth_1}
    = 
    \frac{\val_1 \wealth_2 - (\wealth_1 + \wealth_2)^2}{(\wealth_1 + \wealth_2)^2}
\end{align*}
which is maximized at $\wealth_1 = \gamma \cdot \val_1$ 
when $\wealth_2 = \gamma \cdot \val_2$.
Therefore, agent 1 has no incentive to deviate 
to any other $\wealth_1 \leq \val_2 - \wealth_2$.
To see that agent 1 has no incentive to deviate 
to any $\wealth_1 > \val_2 - \wealth_2$, 
note that her utility is maximized at $\wealth_1 = \val_2$ for all possible $\wealth_1 > \val_2 - \wealth_2$,
and this utility $\val_1 - \val_2$ 
is smaller than the utility $\frac{\val_1}{\val_1 + \val_2}(\val_1 - (\frac{\val_1\val_2}{\val_1 + \val_2}))$
at $\wealth_1 = \gamma\cdot \val_1$
under the assumption $(\val_1 + \val_2)\val_2 \geq \val_1^2$.

By similar calculation, it can be verified that
agent 2 has no incentive to deviate to any other $\wealth_2 \leq \val_2 - \wealth_1$.
To see that agent 2 has no incentive to deviate 
to any $\wealth_2 > \val_2 - \wealth_1$, 
note that her utility is upperbouned by 
the utility at $\wealth_2 = \val_2 - \wealth_1$.
\end{proof}

\begin{remark}
The equilibrium in \Cref{claim:quasi linear inefficient equilibrium} is not efficient. 
However, its allocation is continuous in both agents'
values as long as $(\val_1 + \val_2)\val_2 \geq 
(\val_1)^2$. In contrast, the allocation in efficient equilibrium
is discontinuous near $\val_1 = \val_2$. 
\end{remark}

\begin{task}
Identify PoA for transferable welfare 
in the warmup example.
\end{task}

\begin{task}
Characterize pure Nash equilibrium for general utilities.
\end{task}


\subsection{Price of anarchy for exogenously-budgeted agents}
In this section, we consider instances where 
there are $n$ agents and each agent $i$ has an exogenous budget $\truewealth_i$, 
i.e., $\moneycost_i(\price) = \price$
if $\price \leq \truewealth_i$, and $\moneycost_i(\price) = \infty$ otherwise.
We show that the PoA of transferable welfare is at most 8.

\begin{theorem}
\label{thm:PoA exogenous budget}
    For exogenously-budgeted agents, the PoA of transferable welfare is at most~8.
\end{theorem}

To show the above theorem, we first build a connection between the optimal 
transferable welfare and the market clearing price $\marketclearing$.

\begin{definition}
    For $n$ exogenously-budgeted agents $\{(\val_i,\truewealth_i)\}_{i\in[n]}$,
    the \emph{market clearing price $\marketclearing$} and 
    \emph{market clearing allocation profile ${\marketclearingallocs}$}
    satisfies
    \begin{itemize}
        \item $0\leq \marketclearingalloc_i \leq 
        \min\{1, \frac{\truewealth_i}{\marketclearing}\}$
        \item $\sum_i \marketclearingalloc_i = 1$
        \item If $\val_i > \marketclearing$, then $\marketclearingalloc_i = 
        \frac{\truewealth_i}{\marketclearing}$
        \item If $\val_i < \marketclearing$, then $\marketclearingalloc_i = 
        0$
    \end{itemize}
\end{definition}


\begin{lemma}
\label{lem:market clearing price exogenous budget}
    The transferable welfare of 
    market clearing allocation profile ${\marketclearingallocs}$
    is a 2-approximation of optimal transferable welfare.
\end{lemma}
\begin{proof}
    By definition, the transferable welfare of 
    market clearing allocation profile ${\marketclearingallocs}$
    equals to the market clearing price $\marketclearing$.
    Thus, it is sufficient to upperbound 
    the optimal transferable welfare by $2\marketclearing$.
    We analyze the contribution of agents with values higher or lower than 
    market clearing price $\marketclearing$ separately.
    For all agents $i$ with $\val_i \leq \marketclearing$, their total contribution
    in the optimal transferable welfare is at most $\marketclearing$ since there is 
    a single item to allocate.
    For all agents $i$ with $\val_i > \marketclearing$,
    their total contribution in the optimal transferable welfare is at most 
    $\sum_{i:\val_i > \marketclearing}\truewealth_i$.
    By definition of market clearing price $\marketclearing$,
    $\sum_{i:\val_i > \marketclearing}\truewealth_i \leq \marketclearing$ as desired.
\end{proof}

\begin{example}[Tightness of \Cref{lem:market clearing price exogenous budget}]
    Consider two exogenously-budgeted agents as follows:
    \begin{align*}
        \val_1 = K,
        \qquad 
        \truewealth_1 = 1,
        \qquad
        \val_2 = 1,
        \qquad
        \truewealth_2 = \infty
    \end{align*}
    where $K$ is a sufficiently large constant.
    The optimal transferable welfare is $(2 - 1/K)$
    by allocating agent $1$ with $\frac{1}{K}$-fraction 
    and allocating agent $2$ with $\frac{K-1}{K}$-fraction.
    The market clearing price is $\marketclearing = 1$,
    and achieves transferable welfare $1$,
    by allocating agent $1$ with the whole item.
\end{example}

We are ready to show \Cref{thm:PoA exogenous budget}.
\begin{proof}[Proof of \Cref{thm:PoA exogenous budget}]
    Fix an arbitrary equilibrium $\{\wealth_i\}$, 
    denote $\price$ and $\allocs$ by the per-unit price and allocation profile in the induced FPPE, respectively.
    We consider two cases separately.

    \smallskip
    \noindent
    \textbf{Case 1- $\price \geq \frac{1}{4}\marketclearing$.}
    In equilibrium, each agent $i$ pays
    at most her exogenous budget $\truewealth_i$. Otherwise, 
    she can increase her negative utility to zero utility 
    by deviating to $\wealth_i\primed = 0$.
    Therefore, 
    the transferable welfare of the equilibrium is $\price \geq \frac{1}{4}\marketclearing$.
    Invoking \Cref{lem:market clearing price exogenous budget} finishes this case.

    \smallskip
    \noindent
    \textbf{Case 2- $\price \leq \frac{1}{4}\marketclearing$.}
    Due to the definition of market clearing allocation profile $\marketclearingallocs$ and \Cref{lem:market clearing price exogenous budget},
    it is sufficient to show that $\alloc_i \geq \frac{1}{4} \marketclearingalloc_i$
    for each agent $i$.
    This is trivially true for agent $i$ with $\val_i < \marketclearing$.
    Below, we consider the remaining agents.

    Fix an arbitrary agent $i$ with $\val_i \geq \marketclearing$.
    Since the payment is non-negative,
    it is sufficient to show that her utility in the equilibrium is 
    at least $\frac{1}{4}\marketclearingalloc_i \cdot \val_i$.
    Suppose agent $i$ deviates to 
    $\wealth_i\primed = \frac{1}{4}\marketclearingalloc_i\marketclearing$.
    Let $\price\primed$ and $\alloc_i\primed$ be 
    new per-unit price and new allocation in the newly induced FPPE.
    
    First we claim that  
    $\price\primed\leq \frac{1}{2}\marketclearing$.
    Note that this is trivially true if $\price\primed \leq \price$.
    If $\price\primed \geq \price$,
    \begin{align*}
        \price\primed 
        \overset{(a)}{\leq}
        \sum_{j\not= i:\val_j \geq \price\primed} \wealth_j
        + \wealth_i\primed
        % \\
        % &
        \overset{(b)}{\leq} \sum_{j\not= i:\val_j \geq \price} \wealth_j
        + \wealth_i\primed
        % \\
        % &
        \overset{(c)}{\leq} \price 
        + \wealth_i\primed
        % \\
        % &
        \leq 
        \frac{1}{4}\marketclearing + \frac{1}{4}\marketclearingalloc_i\marketclearing 
        \leq \frac{1}{2}\marketclearing 
    \end{align*}
    where inequalities~(a) (c) holds due to the definition of per-unit price $\price\primed$, $\price$ in FPPE; and inequality~(b) holds since $\price\primed \geq \price$.

    Since agent $i$ has value $\val_i \geq \marketclearing > \price\primed$,
    by deviating to $\wealth_i\primed$,
    she receives allocation $\alloc_i\primed = \frac{\wealth_i\primed}{\price\primed}$,
    and pays $\wealth_i\primed$. By definition of market clearing price $\marketclearing$, 
    $\marketclearingalloc_i\marketclearing \leq \truewealth_i$ and thus 
    $\wealth_i\primed \leq \frac{1}{4}\truewealth_i$.
    Therefore, by deviating to $\wealth_i\primed$, agent $i$ has utility
    \begin{align*}
        \alloc_i\primed\cdot \val_i - 
        \moneycost_i(\alloc_i\primed\cdot\price\primed)
        =
        \alloc_i\primed\cdot (\val_i - \price\primed)
        \geq
        \frac{\frac{1}{4}\marketclearingalloc_i\marketclearing}{\frac{1}{2}\marketclearing}
        \cdot \left(
        \val_i - \frac{1}{2}\marketclearing
        \right)
        \geq 
        \frac{1}{4}\marketclearingalloc_i\cdot \val_i
    \end{align*}
    as desired.
\end{proof}

\subsection{Price of anarchy for general 
non-quasilinear agents}
In this subsection, we 
extend the analysis in \Cref{thm:PoA exogenous budget}
for exogenously-budgeted agents
to agents with general non-quasilinear utility.
For ease of presentation, we assume that 
the outside option value for money
$\moneycost_i$ is differentiable, and 
thus its derivative $\moneycostderivative_i$
exists for every agent $i$.\footnote{Similar argument
can be extended
for non-differentiable $\{\moneycost_i\}$.
The same PoA bound and argument hold
in the alternative model 
where agents can misreport both 
their values and budgets.}
\begin{theorem}
\label{thm:poa strictly convex}
    For non-quasilinear agents 
    with differentiable
    $\{\moneycost_i\}_{i\in[n]}$, the
    PoA of transferable welfare is at most
    $\frac{2}{3-2\sqrt{2}} \approx 11.66$.
\end{theorem}

First, we define the market clearing price $\marketclearing$
in this setting.

\begin{definition}
    For non-quasilinear agents
    with values $\{\val_i\}$
    and differentiable
    $\{\moneycost_i\}$,
    the \emph{market clearing price $\marketclearing$} and 
    \emph{market clearing allocation profile ${\marketclearingallocs}$}
    guarantees
    \begin{itemize}
        \item for every agent $i$, $0\leq \marketclearingalloc_i \leq 1$
        \item $\sum_i \marketclearingalloc_i = 1$
        \item for every agent $i$ with
        $\val_i \geq \marketclearing$,  
        her market clearing allocation $\marketclearingalloc_i$
        satisfies
        $\moneycostderivative_i(\alloc\cdot \marketclearing) \leq 
        \frac{\val_i}{\marketclearing}$
        for all $\alloc \in[0, \marketclearingalloc_i)$
        and $\moneycostderivative_i(\alloc\cdot \marketclearing) 
        \geq 
        \frac{\val_i}{\marketclearing}$
        for all $\alloc \in [\marketclearingalloc_i,\infty)$
        \item for every agent $i$ with
        $\val_i < \marketclearing$, 
        her market clearing allocation $\marketclearingalloc_i$
        satisfies
        $\marketclearingalloc_i = 
        0$
        % \item for every agent $i$ with
        % $\val_i = \marketclearing$, 
        % her market clearing allocation $\marketclearingalloc_i$
        % satisfies
        % $\moneycostderivative_i(\alloc\cdot \marketclearing) \leq 
        % \frac{\val_i}{\marketclearing}=1$
        % for all $\alloc\in[0,\marketclearingalloc_i)$
    \end{itemize}
\end{definition}
Since $\{\moneycost_i\}_{i\in[n]}$
is convex and increasing,
it can be verified that 
there exists unique market clearing price $\marketclearing$. Furthermore, 
by definition, for each agent $i$,
give market clearing price $\marketclearing$,
her utility is maximized at 
allocation $\marketclearingalloc_i$.


\begin{lemma}
\label{lem:market clearing price strictly convex}   
For non-quasilinear agents 
    with differentiable
    $\{\moneycost_i\}_{i\in[n]}$,
    the transferable welfare of 
    market clearing allocation profile ${\marketclearingallocs}$
    is at most $2\marketclearing$.
\end{lemma}
\begin{proof}
Let $\marketclearingwtp_i = \wtp_i(\marketclearingalloc_i)$
be the contribution of transferable welfare for each agent $i$.
Below we upperbound $\marketclearingwtp_i$ 
for each agent $i$
based on her value $\val_i$ with two cases.

\smallskip
Fix an arbitrary agent $i$ with value $\val_i \leq \marketclearing$.
Note that
her contribution to transferable welfare
is at most her contribution to welfare,
i.e., $\marketclearingwtp_i \leq \marketclearingalloc_i\cdot \val_i 
\leq \marketclearingalloc_i\cdot \marketclearing$.

\smallskip
Fix an arbitrary agent $i$ with value $\val_i > \marketclearing$.
Note that her contribution of transferable welfare 
$\marketclearingwtp_i$ satisfies
\begin{align*}
    \displaystyle \int_{0}^{\marketclearingwtp_i}
    \moneycostderivative_i(t)\,dt
    =
    \marketclearingalloc_i \cdot \val_i
    \end{align*}
{where the right-hand side can be rewritten as}
\begin{align*}
    \marketclearingalloc_i \cdot \val_i
    =
    \displaystyle \int_{0}^{\marketclearingalloc_i\cdot \marketclearing}
    \frac{\val_i}{\marketclearing}\,dt
    \leq
    \displaystyle \int_{0}^{\marketclearingalloc_i\cdot \marketclearing}
    \frac{\val_i}{\marketclearing} 
    % - \moneycostderivative_i(t)
    \,dt
    +
    \displaystyle \int_{0}^{\marketclearingalloc_i\cdot \marketclearing}\moneycostderivative_i(t)\,dt
\end{align*}
Therefore, 
\begin{align*}
    \displaystyle \int_{\marketclearingalloc_i\cdot \marketclearing}^{\marketclearingwtp_i}
    \moneycostderivative_i(t)\,dt
    \leq 
    \displaystyle \int_{0}^{\marketclearingalloc_i\cdot \marketclearing}
    \frac{\val_i}{\marketclearing} 
    % - \moneycostderivative_i(t)
    \,dt
\end{align*}
By definition, $\moneycostderivative_i(\alloc\cdot \marketclearing)
\geq \frac{\val_i}{\marketclearing}$
for all $\alloc > \marketclearingalloc_i$. Thus,
\begin{align*}
    \marketclearingwtp_i \leq 2 \marketclearingalloc_i
    \cdot \marketclearing
\end{align*}

\noindent
Putting all pieces together finishes the proof.
\end{proof}


\begin{lemma}
\label{lem:strictly convex approx to market clearing}
For non-quasilinear agents 
    with differentiable
    $\{\moneycost_i\}_{i\in[n]}$,
    the transferable welfare 
    of any equilibrium is an $\frac{1}{3-2\sqrt{2}}$-approximation
    to 
    the transferable welfare of 
    market clearing allocation profile ${\marketclearingallocs}$.
\end{lemma}
\begin{proof}
    Fix an arbitrary equilibrium $\{\wealth_i\}$, 
    denote $\price$ and $\allocs$ by the per-unit price and allocation profile in the induced FPPE, respectively.
    We consider two cases separately.

    \smallskip
    \noindent
    \textbf{Case 1- $\price \geq (6-4\sqrt{2})\marketclearing$.}
    In equilibrium, each agent $i$ has non-negative utility.
    Otherwise, 
    she can increase her negative utility to zero utility 
    by deviating to $\wealth_i\primed = 0$.
    Therefore, 
    the transferable welfare of the equilibrium is 
    at least the revenue in FPPE, i.e., at least $\price$.
    Invoking \Cref{lem:market clearing price strictly convex} with the assumption that $\price\geq (6-4\sqrt{2})\marketclearing$ finishes this case.

    \smallskip
    \noindent
    \textbf{Case 2- $\price \leq (6-4\sqrt{2})\marketclearing$.}
    Due to the definition of market clearing allocation profile $\marketclearingallocs$, \Cref{lem:market clearing price strictly convex} and the convexity of
    $\moneycost_i$ (aka., concavity of $\wtp_i$),
    it is sufficient to show that $\alloc_i \geq 
    (3-2\sqrt{2})\marketclearingalloc_i$
    for each agent $i$.
    This is trivially true for agent $i$ with $\val_i < \marketclearing$.
    Below, we consider the remaining agents.

    Fix an arbitrary agent $i$ with $\val_i \geq \marketclearing$.
    Since the payment is non-negative,
    it is sufficient to show that her utility in the equilibrium is 
    at least $(3-2\sqrt{2})\marketclearingalloc_i \cdot \val_i$.
    Suppose agent $i$ deviates to 
    $\wealth_i\primed = 
    (3\sqrt{2} - 4)\marketclearingalloc_i\marketclearing$.
    Let $\price\primed$ and $\alloc_i\primed$ be 
    new per-unit price and new allocation in the newly induced FPPE.
    
    First we claim that  
    $\price\primed\leq (2-\sqrt{2})\marketclearing$.
    Note that this is trivially true if $\price\primed \leq \price$.
    If $\price\primed \geq \price$,
    \begin{align*}
        \price\primed 
        &\overset{(a)}{\leq}
        \sum_{j\not= i:\val_j \geq \price\primed} \wealth_j
        + \wealth_i\primed
        % \\
        % &
        \overset{(b)}{\leq} \sum_{j\not= i:\val_j \geq \price} \wealth_j
        + \wealth_i\primed
        % \\
        % &
        \overset{(c)}{\leq} \price 
        + \wealth_i\primed
        \\
        &
        \leq 
        (6-4\sqrt{2})\marketclearing + 
        (3\sqrt{2}-4)\marketclearingalloc_i\marketclearing 
        \leq 
        (2-\sqrt{2})\marketclearing 
    \end{align*}
    where inequalities~(a) (c) holds due to the definition of per-unit price $\price\primed$, $\price$ in FPPE; and inequality~(b) holds since $\price\primed \geq \price$.

    Since agent $i$ has value $\val_i \geq \marketclearing > \price\primed$,
    by deviating to $\wealth_i\primed$,
    she receives allocation $\alloc_i\primed = \frac{\wealth_i\primed}{\price\primed}
    \geq 
    \frac{3\sqrt{2}-4}{2-\sqrt{2}}
    \marketclearingalloc_i$,
    and pays $\wealth_i\primed$. 
    Note that holding all other agents' reported budgets fixed, 
    the per-unit price induced by FPPE is decreasing continuously 
    as agent $i$'s reported budget decreases.
    Furthermore, 
    the allocation of agent $i$ induced by FPPE changes continuously 
    as agent $i$'s reported budget decreases; and becomes zero when 
    agent $i$ reports zero budget.
    Therefore, there exists $\wealth_i\doubleprimed \leq \wealth_i\primed$ 
    such that
    when agent $i$ deviates to $\wealth_i\doubleprimed$,
    allocation $\alloc_i\doubleprimed = \frac{3\sqrt{2}-4}{2-\sqrt{2}}
    \marketclearingalloc_i$
    and per-unit price $\price\doubleprimed 
    \leq \price\primed
    \leq (2-\sqrt{2})\marketclearing$.
    By deviating to $\wealth_i\doubleprimed$, agent $i$ has utility
    \begin{align*}
        \alloc_i\doubleprimed\cdot \val_i - 
        \moneycost_i(\alloc_i\doubleprimed\cdot\price\doubleprimed)
        &\geq 
        \frac{3\sqrt{2}-4}{2-\sqrt{2}}
    \marketclearingalloc_i\cdot \val_i 
    -
        \moneycost_i\left(
        \frac{3\sqrt{2}-4}{2-\sqrt{2}}
    \marketclearingalloc_i \cdot (2-\sqrt{2})\marketclearing
    \right)
    \\
       & =
        (3-2\sqrt{2})\marketclearingalloc_i\cdot \val_i
        +
        (3\sqrt{2} - 4)\marketclearingalloc_i\cdot \val_i
        -
        \moneycost_i\left((3\sqrt{2} - 4)
        \marketclearingalloc_i\cdot 
        \marketclearing\right)
        \\
        &\overset{(a)}{\geq} 
        (3-2\sqrt{2})\marketclearingalloc_i\cdot \val_i
        +
        (3\sqrt{2} - 4)
        \left(\marketclearingalloc_i\cdot \val_i
        -
        \moneycost_i\left(
        \marketclearingalloc_i\cdot 
        \marketclearing\right)
        \right)
        \\
        &\overset{(b)}{\geq} 
        (3-2\sqrt{2})\marketclearingalloc_i\cdot \val_i
    \end{align*}
    where inequality~(a) holds due to the convexity of $\moneycost_i$;
    and inequality~(b) holds due to $\marketclearingalloc_i\cdot \val_i
        -
        \moneycost_i\left(
        \marketclearingalloc_i\cdot 
        \marketclearing\right) \geq 0$,
        which is
    implied by the definition of market clearing allocation $\marketclearingalloc_i$ and market clearing price $\marketclearing$.
\end{proof}

To upperbound the PoA, it remains to show the following 
lemma.
\begin{lemma}
For non-quasilinear agents 
    with differentiable
    $\{\moneycost_i\}_{i\in[n]}$,
the transferable welfare of 
    market clearing allocation profile ${\marketclearingallocs}$
    is a 2-approximation
of the optimal transferable welfare.
\end{lemma}
\begin{proof}
Let  
$\optalloc_i$ be the allocation for each 
agent $i$ in the optimal transferable welfare. Note that
\begin{align*}
    % &
    % 2\cdot \overbrace{\sum_{i:\val_i = \marketclearing}
    % \marketclearingalloc_i\cdot \marketclearing
    % +
    % \sum_{i:\val_i > \marketclearing}
    % \wtp_i(\marketclearingalloc_i) 
    % }^{\text{lowerbound of 
    % transferable welfare in $\marketclearingallocs$}}
    % -
    % \overbrace{\sum_{i:\val_i>\marketclearing}
    % \wtp_i(\optalloc_i)}^{
    % \substack{
    % % \text{contribution 
    % % of agents with $\val_i > \marketclearing$}
    % % \\
    % \text{
    % optimal transferable welfare}
    % }}
    &2\cdot 
    \sum_{i\in[n]}
    \wtp_i(\marketclearingalloc_i)
    -
    \sum_{i\in[n]}\wtp_i(\optalloc_i)
    \\
    \overset{(a)}{\geq}&
    ~
    \marketclearing 
    + \sum_{i\in[n]}
    \wtp_i(\marketclearingalloc_i)
    -
    \sum_{i\in[n]}\wtp_i(\optalloc_i)
    \\
    \geq&~
    \marketclearing
    +
    \sum_{i\in[n]}
    \min\left\{
    0, \wtp_i(\marketclearingalloc_i) - \wtp_i(\optalloc_i)
    \right\}
    \\
    \geq&~
    \marketclearing
    -
    \sum_{i:
    \marketclearingalloc_i < \optalloc_i}
    \displaystyle
    \int_{\marketclearingalloc_i}^{\optalloc_i}
    \wtp_i'(x)\,dx
    \\
    \overset{}{=}&~
    \marketclearing
    -
    \sum_{i:
    \marketclearingalloc_i < \optalloc_i}
    \displaystyle
    \int_{\marketclearingalloc_i}^{\optalloc_i}
    \frac{\val_i}{
    \moneycostderivative_i(\alloc \cdot \val_i)}\,dx
    \\
    \overset{}{=}&~
    \marketclearing
    -
    \sum_{i:\val_i > \marketclearing\land 
    \marketclearingalloc_i < \optalloc_i}
    \displaystyle
    \int_{\marketclearingalloc_i}^{\optalloc_i}
    \frac{\val_i}{
    \moneycostderivative_i(\alloc \cdot \val_i)}\,dx
    -
    \sum_{i:\val_i \leq \marketclearing\land
    \marketclearingalloc_i < \optalloc_i}
    \displaystyle
    \int_{\marketclearingalloc_i}^{\optalloc_i}
    \frac{\val_i}{
    \moneycostderivative_i(\alloc \cdot \val_i)}\,dx
    \\
    \overset{}{\geq}&~
    \marketclearing
    -
    \sum_{i:\val_i > \marketclearing\land 
    \marketclearingalloc_i < \optalloc_i}
    \displaystyle
    \int_{\marketclearingalloc_i}^{\optalloc_i}
    \frac{\val_i}{
    \moneycostderivative_i(\alloc \cdot \marketclearing)}\,dx
    -
    \sum_{i:\val_i \leq \marketclearing\land
    \marketclearingalloc_i < \optalloc_i}
    \displaystyle
    \int_{\marketclearingalloc_i}^{\optalloc_i}
    \frac{\marketclearing}{
    \moneycostderivative_i(\alloc \cdot \val_i)}\,dx
    \\
    \overset{(b)}{\geq}&~
    \marketclearing
    -
    \sum_{i:\val_i > \marketclearing \land 
    \marketclearingalloc_i < \optalloc_i}
    \displaystyle
    \int_{\marketclearingalloc_i}^{\optalloc_i}
    \marketclearing\,dx
    -
    \sum_{i:\val_i \leq \marketclearing \land 
    \marketclearingalloc_i < \optalloc_i}
    \displaystyle
    \int_{\marketclearingalloc_i}^{\optalloc_i}
    \marketclearing\,dx
    \\
    \overset{}{\geq}& 
    ~0
\end{align*}
where
inequality~(a) uses the fact that transferable welfare $\sum_{i}\wtp_i(\marketclearingalloc_i)$ is lowerbounded by revenue $\marketclearing$;
and inequality~(b) uses the 
the definition
of market clearing price and market clearing allocation,
i.e., $\moneycostderivative_i(\alloc\cdot \marketclearing) > 
        \frac{\val_i}{\marketclearing}$
        for all $\alloc \in [\marketclearingalloc_i,\infty)$,
        and the assumption that $\moneycostderivative_i(\price)\geq 1$
        for all $\price$.
\end{proof}

\subsection{Extension to concave valuation function}

Our results can be approximately extended to the model 
where each agent $i$ has an increasing and 
\emph{concave} valuation function 
$\valuefunc:[0,1]\rightarrow \reals_+$.
Given allocation $\alloc_i$ and payment $\price_i$,
the utility of agent $i$ is 
$\util_i(\alloc_i, \price_i) = \valuefunc_i(\alloc_i) - \moneycost_i(\price_i)$.
We write $\valuefuncderivative_i(\alloc_i)$ for the derivative of 
$\valuefunc_i$ at $\alloc_i$.
Since $\valuefunc$ is increasing and concave, its derivative $\valuefuncderivative_i$
is non-negative and monotone decreasing.
We use $\valuefunccurvature \triangleq \max_{i\in[n]} \frac{\valuefuncderivative_i(0)}{\valuefuncderivative_i(1)}$ to denote the largest ratio
of value function derivative.

\begin{definition}
    For non-quasilinear agents
    with increasing concave valuation functions $\{\valuefunc_i\}$
    and increasing convex outside option value function 
    $\{\moneycost_i\}$ for money,
    the \emph{market clearing price $\marketclearing$} and 
    \emph{market clearing allocation profile ${\marketclearingallocs}$}
    satisfies
    \begin{itemize}
        \item for every agent $i$, 
        $\marketclearingalloc_i 
        \in \argmax_{0\leq \alloc \leq 1} 
        \valuefunc_i(\alloc) - 
        \moneycost_i(\alloc\cdot \marketclearing)
        $
        \item $\sum_i \marketclearingalloc_i = 1$
    \end{itemize}
\end{definition}
\begin{lemma}
    For non-quasilinear agents
    with increasing concave valuation functions $\{\valuefunc_i\}$
    and increasing convex outside option value function 
    $\{\moneycost_i\}$ for money,
    the market clearing price $\marketclearing$ exists and 
    is unique. 
    Furthermore, agents can be partitioned into two 
    disjoint subsets as follows,
    \begin{itemize}
        \item for every agent $i$
        with $\valuefuncderivative_i(0) \geq \marketclearing\cdot 
        \moneycostderivative_i(0)$, 
        her market clearing allocation $\marketclearingalloc_i$
        satisfies
        $\moneycostderivative_i(\alloc\cdot \marketclearing)
        \leq 
        \frac{\valuefuncderivative_i(\alloc)}
        {\marketclearing}$
        for all $\alloc \in [0, \marketclearingalloc_i)$
        and 
        $\moneycostderivative_i(\alloc\cdot \marketclearing)
        \geq  
        \frac{\valuefuncderivative_i(\alloc)}
        {\marketclearing}$
        for all $\alloc \in [\marketclearingalloc_i,\infty)$
        
        \item for every agent $i$
        with $\valuefuncderivative_i(0) < \marketclearing\cdot 
        \moneycostderivative_i(0)$, 
        her market clearing allocation $\marketclearingalloc_i$
        satisfies
        $\marketclearingalloc_i = 0$ and 
        $\moneycostderivative_i(\alloc\cdot \marketclearing)
        >  
        \frac{\valuefuncderivative_i(\alloc)}
        {\marketclearing}$
        for all $\alloc \in [0, \infty)$
        
    \end{itemize}
\end{lemma}

\begin{lemma}
\label{lem:market clearing approx single item}
  For non-quasilinear agents
    with increasing concave valuation functions $\{\valuefunc_i\}$
    and increasing convex outside option value function 
    $\{\moneycost_i\}$ for money,
the transferable welfare of 
    market clearing allocation profile ${\marketclearingallocs}$
    is a 2-approximation
of the optimal transferable welfare.
\end{lemma}
\begin{proof}
Let  
$\optalloc_i$ be the allocation for each 
agent $i$ in the optimal transferable welfare. Note that
\begin{align*}
    &2\cdot 
    \sum_{i\in[n]}
    \wtp_i(\marketclearingalloc_i)
    -
    \sum_{i\in[n]}\wtp_i(\optalloc_i)
    \\
    \overset{(a)}{\geq}&
    ~
    \marketclearing 
    + \sum_{i\in[n]}
    \wtp_i(\marketclearingalloc_i)
    -
    \sum_{i\in[n]}\wtp_i(\optalloc_i)
    \\
    \geq&~
    \marketclearing
    +
    \sum_{i\in[n]}
    \min\left\{
    0, \wtp_i(\marketclearingalloc_i) - \wtp_i(\optalloc_i)
    \right\}
    \\
    \geq&~
    \marketclearing
    -
    \sum_{i:
    \marketclearingalloc_i < \optalloc_i}
    \displaystyle
    \int_{\marketclearingalloc_i}^{\optalloc_i}
    \wtp_i'(x)\,dx
    \\
    \overset{}{=}&~
    \marketclearing
    -
    \sum_{i:
    \marketclearingalloc_i < \optalloc_i}
    \displaystyle
    \int_{\marketclearingalloc_i}^{\optalloc_i}
    \frac{\valuefuncderivative_i(\alloc)}{
    \moneycostderivative_i(\valuefunc_i(\alloc))}\,dx
    \\
    \overset{}{=}&~
    \marketclearing
    -
    \sum_{i:\valuefuncderivative_i(0) > \marketclearing\land 
    \marketclearingalloc_i < \optalloc_i}
    \displaystyle
    \int_{\marketclearingalloc_i}^{\optalloc_i}
    \frac{\valuefuncderivative_i(\alloc)}{
    \moneycostderivative_i(\valuefunc_i(\alloc))}\,dx
    -
    \sum_{i:\valuefuncderivative_i(0) \leq \marketclearing\land
    \marketclearingalloc_i < \optalloc_i}
    \displaystyle
    \int_{\marketclearingalloc_i}^{\optalloc_i}
    \frac{\valuefuncderivative_i(\alloc)}{
    \moneycostderivative_i(\valuefunc_i(\alloc))}\,dx
    \\
    \overset{}{\geq}&~
    \marketclearing
    -
    \sum_{i:\valuefuncderivative_i(0) > \marketclearing\land 
    \marketclearingalloc_i < \optalloc_i}
    \displaystyle
    \int_{\marketclearingalloc_i}^{\optalloc_i}
    \frac{\valuefuncderivative_i(\alloc)}{
    \moneycostderivative_i(\alloc \cdot \marketclearing)}\,dx
    -
    \sum_{i:\valuefuncderivative_i(0) \leq \marketclearing\land
    \marketclearingalloc_i < \optalloc_i}
    \displaystyle
    \int_{\marketclearingalloc_i}^{\optalloc_i}
    \frac{\marketclearing}{
    \moneycostderivative_i(\valuefunc_i(\alloc))}\,dx
    \\
    \overset{(b)}{\geq}&~
    \marketclearing
    -
    \sum_{i:\valuefuncderivative_i(0) > \marketclearing \land 
    \marketclearingalloc_i < \optalloc_i}
    \displaystyle
    \int_{\marketclearingalloc_i}^{\optalloc_i}
    \marketclearing\,dx
    -
    \sum_{i:\valuefuncderivative_i(0) \leq \marketclearing \land 
    \marketclearingalloc_i < \optalloc_i}
    \displaystyle
    \int_{\marketclearingalloc_i}^{\optalloc_i}
    \marketclearing\,dx
    \\
    \overset{}{\geq}& 
    ~0
\end{align*}
where
inequality~(a) uses the fact that transferable welfare $\sum_{i}\wtp_i(\marketclearingalloc_i)$ is lowerbounded by revenue $\marketclearing$;
and inequality~(b) uses the 
the definition
of market clearing price and market clearing allocation,
i.e., $\moneycostderivative_i(\alloc\cdot \marketclearing) \geq 
        \frac{\valuefuncderivative_i(\alloc)}{\marketclearing}$
        for all $\alloc \in [\marketclearingalloc_i,\infty)$,
        and the assumption that $\moneycostderivative_i(\price)\geq 1$
        for all $\price$.
\end{proof}

\begin{lemma}  
  For non-quasilinear agents
    with increasing concave valuation functions $\{\valuefunc_i\}$
    and increasing convex outside option value function 
    $\{\moneycost_i\}$ for money,
    the transferable welfare of 
    market clearing allocation profile ${\marketclearingallocs}$
    is at most $(\valuefunccurvature+1)\marketclearing$.
\end{lemma}
\begin{proof}
Let $\marketclearingwtp_i = \wtp_i(\marketclearingalloc_i)$
be the contribution of transferable welfare for each agent $i$.
Below we upperbound $\marketclearingwtp_i$ 
for each agent $i$
based on her value $\val_i$ with two cases.

\smallskip
Fix an arbitrary agent $i$ with $\valuefuncderivative_i(0) 
\leq \marketclearing$.
Note that
her contribution to transferable welfare
is at most her contribution to welfare,
i.e., $\marketclearingwtp_i \leq 
\valuefunc_i(\marketclearingalloc_i)
\leq \marketclearingalloc_i\cdot \valuefuncderivative_i(0)
\leq \marketclearingalloc_i\cdot \marketclearing$.

\smallskip
Fix an arbitrary agent $i$ with value $\valuefuncderivative_i(0)
> \marketclearing$.
Note that her contribution of transferable welfare 
$\marketclearingwtp_i$ satisfies
\begin{align*}
    \displaystyle \int_{0}^{\marketclearingwtp_i}
    \moneycostderivative_i(t)\,dt
    =
    \valuefunc_i(\marketclearingalloc_i)
    \end{align*}
{where the right-hand side can be rewritten as}
\begin{align*}
    \valuefunc_i(\marketclearingalloc_i)
    =
    \displaystyle \int_{0}^{\marketclearingalloc_i\cdot \marketclearing}
    \frac{\valuefuncderivative_i(t/\marketclearing)}{\marketclearing}\,dt
    \leq
    \displaystyle \int_{0}^{\marketclearingalloc_i\cdot \marketclearing}
    \frac{\valuefuncderivative_i(t/\marketclearing)}{\marketclearing}\,dt
    % - \moneycostderivative_i(t)
    \,dt
    +
    \displaystyle \int_{0}^{\marketclearingalloc_i\cdot \marketclearing}\moneycostderivative_i(t)\,dt
\end{align*}
Therefore, 
\begin{align*}
    \displaystyle \int_{\marketclearingalloc_i\cdot \marketclearing}^{\marketclearingwtp_i}
    \moneycostderivative_i(t)\,dt
    \leq 
    \displaystyle \int_{0}^{\marketclearingalloc_i\cdot \marketclearing}
   \frac{\valuefuncderivative_i(t/\marketclearing)}{\marketclearing}\,dt
    % - \moneycostderivative_i(t)
    \,dt
\end{align*}
By definition, $\moneycostderivative_i(\alloc\cdot \marketclearing)
\geq \frac{\valuefuncderivative_i(\alloc)}{\marketclearing}
\geq \frac{\valuefuncderivative_i(1)}{\marketclearing}$
for all $\alloc > \marketclearingalloc_i$,
and $\valuefuncderivative_i(\alloc) \leq \valuefunccurvature\cdot 
\valuefuncderivative_i(1)$ for all $\alloc \in[0,1]$. 
Thus,
\begin{align*}
    \marketclearingwtp_i \leq (\valuefunccurvature + 1) \marketclearingalloc_i
    \cdot \marketclearing
\end{align*}

\noindent
Putting all pieces together finishes the proof.
\end{proof}

\newpage



==> Notes/metagame-multiple-FPPE-issue.tex <==
\section{Multiplicity Issue of Allocation 
in FPPE}

Given a fixed valuation and budget profile, the pacing 
multipliers and per-unit prices in FPPE are unique. 
However, the allocation is not unique, and thus the 
non-quasi-linear agents' utility in the metagame 
may not be unique. 
To resolve this issue, in the metagame we also specify 
an allocation selection rule when multiple 
allocation profiles exists for a FPPE.

When agents only report budget 
in the metagame, 
the allocation selection rule 
has no impact on the possible equilibrium.
% on the agents' utility in equilibrium.

\begin{conjecture}
Consider the metagame where each agent $i$ reports 
budget $\wealth_i$.
For arbitrary selection rules $\sigma,\sigma\primed$,
if $\eqlb$ 
is a equilibrium 
under selection rule $\sigma$;
then
there exists a equilibrium $\eqlb\primed$
under selection rule $\sigma\primed$
such that every agent's utility in $\eqlb$
under selection rule $\sigma$
is the same as her utility in $\eqlb\primed$
under selection rule $\sigma\primed$.
\end{conjecture}


\begin{conjecture}
Consider the metagame where each agent $i$ reports 
budget $\wealth_i$.
For arbitrary selection rules $\sigma,\sigma\primed$,
if $\eqlb$ 
is a equilibrium 
under selection rule $\sigma$;
then
there exists a equilibrium $\eqlb\primed$
under selection rule $\sigma\primed$
such that the transferable welfare in $\eqlb$
under selection rule $\sigma$
is the same as the transferable welfare in $\eqlb\primed$
under selection rule $\sigma\primed$
\end{conjecture}

==> Notes/metagame-value-reporting.tex <==
\section{Metagame under Value Reporting}

\newcommand{\valreported}{\tilde{\val}}

In this section, we consider an alternative metagame
where each agent $i$ reports her valuation profile $\valreported_i$
and the seller implements 
the allocation and payment profile
induced by the FPPE assuming each agent $i$
has valuation profile $\valreported_i$
and budget $\wealth_i = \infty$, i.e., assuming agents are quasi-linear.
Below we give an example to show that the PoA
can be unbounded in this alternative metagame.

\begin{example}[{Unbounded Bayesian Nash}]
There is a single item and $N + 2$ agents. 
For the first $N$ agents $i= 1, \dots, N$, 
they all have deterministic value $N^2$ and 
budget $\frac{1}{2}$.
For the last
two agent $i = N+1, N+2$,
they have value $2$ 
with probability $1-\epsilon$,
value $0$ with probability $\epsilon$;
and deterministic budget $1$.

The optimal transferable welfare is $\frac{N}{2}$ by allocating 
$\frac{1}{N}$ fraction of the item to each of the first $N$ agents.

Consider the following Bayesian Nash equilibrium:
the first $N$ agents report value $\frac{1}{2}$;
the last two agents report value $1$ when their true value is $2$,
and report value $0$ when their true value is $0$.
In this equilibrium, the expected transferable welfare
is $(1 - \epsilon^2)\cdot 2 + \epsilon \cdot \frac{N}{2}$.
Letting $\epsilon$ goes to zero and $N$ goes to infinite leads to an unbounded Bayesian Nash
as desired.

Finally, we verify that this equilibrium is valid by 
arguing that the all agents have no profitable deviations.
For each of the first $N$ agents, 
deviating to a smaller reported value reduces 
her utility to zero, while deviating to a higher reported value 
leads to a violation of her hard budget constraint and thus 
reduces her utility as well.
For the last two agents with realized value zero, 
reporting value zero is optimal.
For the last two agents with realized value two, 
deviating to a smaller reported value reduces 
her winning probability down to $\epsilon$,
while deviating to a higher reported value leads 
to a violation of her hard budget constraint,
and thus in both cases her utility is reduced.\footnote{Here we assume that 
when last two agents both report value $1$, each of them wins 
a fraction of the item greater than $2\epsilon$.}
\end{example}

\paragraph{Unbounded PoA 
under uniform tie breaking}
There is a single item and $N + 2$ agents. 
For the first $N$ agents $i= 1, \dots, N$, 
they all have value $N^2$ and 
budget $\frac{1}{3} - \epsilon$
with $\epsilon = o(1)$.
For the last
two agent $i = N+1, N+2$,
they have value $1$ and no budget.

The optimal transferable welfare is 
$\frac{N}{3} - \epsilon N = \Theta(N)$ 
by allocating $\frac{1}{N}$ fraction of the item
to each of the first $N$ agents.
 
Consider the following reported valuation profile in the meta game:
the first $N$ agents report value $0$,
and the last two agents report value $1$.
In this case, the per-unit price is $1$,
and 
each of the two agents
gets $\frac{1}{2}$ fraction of the item,
due to the uniform tie breaking rule.
Note that this reported valuation profile
in indeed an equilibrium.
In particular, for every agent $i\in [N]$,
she either receives nothing and pays nothing
by reporting value smaller than 1;
or receives $\frac{1}{3}$ or more fraction of the item, pays strictly more than her budget,
and gains negative utility 
by reporting value equal or larger than 1.
Finally, note that the transferable welfare 
in this equilibrium is 1,
which indicates a PoA of $\Theta(N)$ 
as desired.

\begin{comment}
\paragraph{Unbounded PoA.}
There is a single item and $N + 1$ agents. 
The first $N$ agents all have value $N$ and 
budget $\frac{1}{\sqrt{N}}$,
and the last agent $N+1$ has value $1$ and no budget.

The optimal transferable welfare is $\sqrt{N}$ 
by allocating $\frac{1}{N}$ fraction of the item
to each of the first $N$ agents.

Now we consider the metagame. 
Consider the following reported valuation profile:
all agents report value $1$.
In this case, the per-unit price is $1$,
and the FPPE can be implemented by multiple allocation profiles.
Suppose we use allocation selection rule such that
it always serves the last agent $N + 1$ first. 
Then, the transferable welfare is 1, and this reporting 
profile is indeed an equilibrium.\footnote{This argument can be extended to allocation selection rule
which maintains a preference over agents where agent $N+1$
is not the least preferred. 
For such an allocation rule, 
the following valuation profile is an equilibrium:
every agent whom is weakly less preferred than agent $N+1$ report value 1, and all other agents report value 0.}
\end{comment}


==> Notes/multi-item-new-analysis-old.tex <==
\section{New Analysis for Multiple Items}

\newcommand{\ctr}{\phi}
\newcommand{\ctrij}{\ctr_{ij}}
\newcommand{\purchaseset}{H}
\newcommand{\purchaseseti}{\purchaseset_i}
\newcommand{\pricej}{\price_j}

In this section, we consider the multi-item environments,
where each agent $i$'s utility given allocation $\allocs$
and per-unit prices $\prices$ is 
$$\util_i(\allocs, \prices) = 
\valuefunc_i\left(
\sum_{j\in[m]} 
\ctrij \cdot \allocij
\right)
-
\moneycost_i\left(
\sum_{j\in[m]}\price_j \cdot \allocij
\right)$$
where $\ctrij$ is the \emph{click-through-rate}
commonly known in the inner FPPE.
Each agent $i$ reports a value $\val_i$ and budget $\wealth_i$, and the inner FPPE assumes 
that agent $i$ has $\val_i \cdot \ctrij$ for
each item $j$ and budget $\wealth_i$.

\subsection{A 2-approximation Analysis for Pure Nash}

The pure Nash PoA guarantee is as follows.
 
\begin{theorem}
\label{thm:multi item concave value convex budget pure}
    In the multi-item environment,
    for agents with (differentiable) concave valuation functions 
 $\{\valuefunc_i\}$ and 
 (differentiable) convex disutilities of money $\{\moneycost_i\}$
 up to heterogeneous budgets $\{\truewealth_i\}$,
    the pure Nash PoA of transferable welfare 
    is at most $2$.
\end{theorem}

Our analysis relies on the following technical lemma, which generalizes
\Cref{lem:alloc lower bound single item concave value hard budget}
from single-item environment to the multi-item environment.
\begin{lemma}
\label{lem:budget lower bound multi item concave value hard budget}
    In the multi-item environment,
    for agents with (differentiable) concave valuation functions 
 $\{\valuefunc_i\}$ and 
 (differentiable) convex disutilities of money $\{\moneycost_i\}$
 up to heterogeneous budgets $\{\truewealth_i\}$,
and every pure Nash equilibrium $\eqlb$,
suppose $\xbf, \prices$
are the allocation and per-unit prices in the induced FPPE.
For every agent $i$ who does not exhaust her true budget $\truewealth_i$,
i.e., $\sum_{j}\alloc_{ij}\cdot \price_j < \truewealth_i$,
her payment $\sum_{j\in[m]}\price_j\allocij$ is at least 
\begin{align*}
\frac
    {\valuefuncderivative_i
    \left(\sum_{j\in[m]}\ctrij\allocij\right)}
{\moneycostderivative_i
    \left(\sum_{j\in[m]}\price_j\allocij\right)}
    \leq 
    \frac{\sum_{j\in \purchaseseti}\price_j}{\sum_{j\in \purchaseseti}(1-\allocij)\ctrij}
\end{align*}
where $H_i \triangleq \{j\in[m]: \alloc_{ij} > 0\}$
includes all items which agent $i$ is allocated.
\end{lemma}

To see \Cref{lem:budget lower bound multi item concave value hard budget} extends \Cref{lem:alloc lower bound single item concave value hard budget},
observe that $\ctrij=1$ in the single-item environment.

\begin{proof}[Proof of \Cref{lem:budget lower bound multi item concave value hard budget}]
    Fix an arbitrary Nash equilibrium $\eqlb$.
    Suppose $\allocs,\prices$ are the allocation and per-unit price in the induced FPPE.
    Fix an arbitrary agent $i$ who does not exhaust her true budget $\truewealth_i$,
i.e., $\sum_j\price_j\allocij < \truewealth_i$.
Let $\Delta \triangleq \frac{\sum_{j\in \purchaseseti}\price_j}{\sum_{j\in \purchaseseti}\ctrij}$.
Due to the definition of FPPE, 
$\frac{\price_j}{\ctrij} \geq \Delta$ for every item $j\in[m]$,
and it becomes equality when $j\in \purchaseseti$.
In the remaining argument, we further assume 
that $\valuefuncderivative_i(\sum_{j\in[m]}\ctrij\allocij) > \Delta$;
otherwise, 
\begin{align*}
    \frac
    {\valuefuncderivative_i
    \left(\sum_{j\in[m]}\ctrij\allocij\right)}
{\moneycostderivative_i
    \left(\sum_{j\in[m]}\price_j\allocij\right)}
    \leq 
    \valuefuncderivative_i
    \left(\sum\nolimits_{j\in[m]}\ctrij\allocij\right)
    \leq 
    \Delta 
    =
    \frac{\sum_{j\in \purchaseseti}\price_j}{\sum_{j\in \purchaseseti}\ctrij}
    \leq 
    \frac{\sum_{j\in \purchaseseti}\price_j}{\sum_{j\in \purchaseseti}(1-\allocij)\ctrij}
\end{align*}
and thus the lemma statement holds trivially.



    Firstly,
    we note that the same FPPE and thus the same utility for every agent are induced
    if 
    we hold all other agents' reports fixed and let 
    agent $i$ report
    $\val_i\primed \triangleq
    \valuefuncderivative_i(\sum_{j\in[m]}\ctrij\allocij)$ 
    and $\wealth_i\primed \triangleq \sum_{j\in [m]} \price_j\allocij$.
    By the definition of $\purchaseseti$, we know that $
    \wealth_i\primed = 
    \sum_{j\in \purchaseseti}\pricej\allocij$.
    Now suppose that
    agent $i$ keeps her reported value $\val\doubleprimed = \val\primed$ the same, but
    increases her reported budget by $\epsilon$
    for sufficiently small and positive $\epsilon < 
    \min\{\truewealth_i - \wealth_i\primed,
    \min_{j\in \purchaseseti}
    \val_i\doubleprimed \ctrij - \price_j
    \}
    $,
    i.e., $\wealth_i\doubleprimed = \wealth_i\primed + \epsilon < \truewealth_i$.
    Let $\allocs\doubleprimed,\prices\doubleprimed$ be 
    the allocation and per-unit price in the new induced FPPE.
    We have 
    \begin{align*}
        \sum_{j\in \purchaseseti}\price_j\doubleprimed \overset{(a)}{\leq} 
        \epsilon + \sum_{j\in \purchaseseti}\price_j
    \end{align*}
    where inequality~(a) holds due to the construction of per-unit price in FPPE (\Cref{lem:fppe increasing budget}).
    In this new induced FPPE, the utility $\util_i\doubleprimed$ of agent $i$ is 
    \begin{align*}
    \util_i\doubleprimed
    &\overset{(a)}{=}
        \valuefunc_i\left(
        \left(\max_{j\in[m]}
        \frac{\ctrij}{\price_j\doubleprimed}
        \right)
        \cdot 
        \sum_{j\in[m]}
            \price_j\doubleprimed
            \allocij\doubleprimed
        \right) 
        - \moneycost_i\left(
            \sum_{j\in[m]}
            \price_j\doubleprimed
            \allocij\doubleprimed
        \right)
        \\
        &\geq 
        \valuefunc_i\left(
        \frac{\sum_{j\in \purchaseseti}\ctrij}
        {\sum_{j\in \purchaseseti}
        \price_j\doubleprimed}
        \cdot 
        \sum_{j\in[m]}
            \price_j\doubleprimed
            \allocij\doubleprimed
        \right) 
        - \moneycost_i\left(
            \sum_{j\in[m]}
            \price_j\doubleprimed
            \allocij\doubleprimed
        \right)
        \\
        &\overset{(b)}{=} 
        \valuefunc_i\left(
        \frac{\sum_{j\in \purchaseseti}\ctrij}
        {\sum_{j\in \purchaseseti}
        \price_j\doubleprimed}
        \cdot 
        \wealth\doubleprimed
        \right) 
        - \moneycost_i\left(
            \wealth\doubleprimed
        \right)
        \\
        &\geq  
        \valuefunc_i\left(
        \frac{\sum_{j\in \purchaseseti}\ctrij}
        {\epsilon+ \sum_{j\in \purchaseseti}
        \price_j}
        \cdot 
        \left(
        \wealth\primed
        +
        \epsilon
        \right)
        \right) 
        - \moneycost_i\left(
            \wealth\primed
            +
            \epsilon
        \right)
        \\
        &\overset{(c)}{=}  
        \valuefunc_i\left(
        % \frac{1}{\frac{\epsilon}{\sum_{j\in\purchaseseti}\price_j}+1}
        \frac{\sum_{j\in\purchaseseti}\price_j}
        {\epsilon+\sum_{j\in\purchaseseti}\price_j}
        \frac{
        \wealth\primed
        +
        \epsilon
        }{\Delta}
        \right) 
        - \moneycost_i\left(
            \wealth\primed
            +
            \epsilon
        \right)
    \end{align*}
    where 
    equality~(a) holds by 
    the construction of FPPE;
    equality~(b) holds due to 
    the unnecessary pacing constraint implied 
    by the construction of $\val_i\doubleprimed$ and $\epsilon$;
    and equality~(c) holds 
    since $\frac{\price_j}{\ctrij} = \Delta$
    for every $j\in \purchaseseti$.
    With a similar argument, the utility $\util_i$
    of agent $i$ in the original FPPE induced by equilibrium $\eqlb$
    is 
    \begin{align*}
    \util_i
    &=
        \valuefunc_i\left(
        \left(\max_{j\in[m]}
        \frac{\ctrij}{\price_j}
        \right)
        \cdot 
        \sum_{j\in[m]}
            \price_j
            \allocij
        \right) 
        - \moneycost_i\left(
            \sum_{j\in[m]}
            \price_j
            \allocij
        \right)
        \\
        &= 
        \valuefunc_i\left(
        \frac{\sum_{j\in \purchaseseti}\ctrij}
        {\sum_{j\in \purchaseseti}
        \price_j}
        \cdot 
        \sum_{j\in[m]}
            \price_j
            \allocij
        \right) 
        - \moneycost_i\left(
            \sum_{j\in[m]}
            \price_j
            \allocij
        \right)
        \\
        &= 
        \valuefunc_i\left(
        \frac{\sum_{j\in \purchaseseti}\ctrij}
        {\sum_{j\in \purchaseseti}
        \price_j}
        \cdot 
        \wealth\primed
        \right) 
        - \moneycost_i\left(
            \wealth\primed
        \right)
        \\
        &=  
        \valuefunc_i\left(
        \frac{
        \wealth\primed}
        {\Delta}
        \right) 
        - \moneycost_i\left(
            \wealth\primed
        \right)
    \end{align*}
    Note that $\util_i - \util_i\doubleprimed \geq 0$ 
    since the former is the utility in the equilibrium, and the later
    is the utility after the deviation.
    Furthermore, we have 
    \begin{align*}
        \util_i - \util_i\doubleprimed
        &\leq \valuefunc_i\left(
        \frac{\wealth\primed}
        {\Delta}
        \right) 
        - \moneycost_i\left(
            \wealth\primed
        \right)
        - 
        \left(
        \valuefunc_i\left(
        \frac{\sum_{j\in\purchaseseti}\price_j}
        {\epsilon+\sum_{j\in\purchaseseti}\price_j}
        \frac{
        \wealth\primed
        +
        \epsilon
        }{\Delta}
        \right) 
        - \moneycost_i\left(
            \wealth\primed
            +
            \epsilon
        \right)
        \right)
        \\
        &= 
        \moneycost_i(\wealth_i\primed + \epsilon)
        - 
        \moneycost_i(\wealth_i\primed)
        -
         \left(
         \valuefunc_i\left(
        \frac{\sum_{j\in\purchaseseti}\price_j}
        {\epsilon+\sum_{j\in\purchaseseti}\price_j}
        \frac{
        \wealth\primed
        +
        \epsilon
        }{\Delta}
        \right) 
        -
        \valuefunc_i\left(
        \frac{
        \wealth\primed
        }{\Delta}
        \right) 
         \right)
        \\
        &\overset{(a)}{\leq}
        \epsilon
        \cdot 
        \moneycostderivative_i(\wealth\primed + \epsilon)
        -
        \left(
        \frac{\sum_{j\in\purchaseseti}\price_j}
        {\epsilon+\sum_{j\in\purchaseseti}\price_j}
        \frac{
        \wealth\primed
        +
        \epsilon
        }{\Delta}
        -
        \frac{
        \wealth\primed
        }{\Delta}
        \right)
        \cdot 
         \valuefuncderivative_i
         \left(
         \frac{\sum_{j\in\purchaseseti}\price_j}
        {\epsilon+\sum_{j\in\purchaseseti}\price_j}
        \frac{
        \wealth\primed
        +
        \epsilon
        }{\Delta}
        \right)
         \\
         &\overset{}{=}
         \epsilon
        \cdot 
        \moneycostderivative_i(\wealth\primed + \epsilon)
        -
        \frac{\epsilon}{\Delta}
        \cdot 
        \frac{\sum_{j\in\purchaseseti}\pricej -
        \wealth_i\primed}{\sum_{j\in\purchaseseti}\price_j + \epsilon}
        \cdot 
         \valuefuncderivative_i
         \left(
         \frac{\sum_{j\in\purchaseseti}\price_j}
        {\epsilon+\sum_{j\in\purchaseseti}\price_j}
        \frac{
        \wealth\primed
        +
        \epsilon
        }{\Delta}
        \right)
         \\
         &\overset{(b)}{=}
         \epsilon
        \cdot 
        \moneycostderivative_i(\wealth\primed + \epsilon)
        -
        \epsilon
        \cdot 
        \frac{\sum_{j\in\purchaseseti}(1-\allocij)\ctrij
        }
        {\sum_{j\in\purchaseseti}\price_j + \epsilon}
        \cdot 
         \valuefuncderivative_i
         \left(
         \frac{\sum_{j\in\purchaseseti}\price_j}
        {\epsilon+\sum_{j\in\purchaseseti}\price_j}
        \frac{
        \wealth\primed
        +
        \epsilon
        }{\Delta}
        \right)
    \end{align*}
    where inequality~(a) holds since $\alloci\doubleprimed > \alloci$, valuation function $\valuefunc_i$
    is concave and differentiable,
    and 
    disutility of money $\moneycost_i$
    is convex and differentiable up to $\truewealth_i$;
    and equality~(b) holds since $\frac{\price_j}{\ctrij} = \Delta$
    for every $j\in \purchaseseti$, and thus $\frac{1}{\Delta}(\sum_{j\in\purchaseseti}\pricej - \wealth_i\primed) =
    \frac{1}{\Delta}(\sum_{j\in\purchaseseti}\pricej - \sum_{j\in\purchaseseti}\pricej\allocij) = 
    \sum_{j\in\purchaseseti}(1-\allocij)\ctrij$.
    After rearranging the terms,
    we have 
    \begin{align*}
           \frac
    {\valuefuncderivative_i
         \left(
         \frac{\sum_{j\in\purchaseseti}\price_j}
        {\epsilon+\sum_{j\in\purchaseseti}\price_j}
        \frac{
        \wealth\primed
        +
        \epsilon
        }{\Delta}
        \right)}
{\moneycostderivative_i(\wealth\primed + \epsilon)}
    \leq 
    \frac{\sum_{j\in \purchaseseti}\price_j + \epsilon}{\sum_{j\in \purchaseseti}(1-\allocij)\ctrij}
    \end{align*}
    for all positive $\epsilon$ that is sufficiently small.
    Finally, letting $\epsilon$ go to zero, 
    the lemma statement is obtained as
    \begin{align*}
    &\lim_{\epsilon\rightarrow 0}
    \moneycostderivative_i(\wealth\primed + \epsilon)
    \overset{(a)}{=}
    \moneycostderivative_i(\wealth\primed)
    =
    \moneycostderivative_i\left(\sum_{j\in [m]}\pricej\allocij\right)
    \\
        &\lim_{\epsilon\rightarrow 0}
        \valuefuncderivative_i
         \left(
         \frac{\sum_{j\in\purchaseseti}\price_j}
        {\epsilon+\sum_{j\in\purchaseseti}\price_j}
        \frac{
        \wealth\primed
        +
        \epsilon
        }{\Delta}
        \right)
        \overset{(b)}{=}
        \valuefuncderivative_i
         \left(
        \frac{
        \wealth\primed
        }{\Delta}
        \right)
    %     =
    %     \valuefuncderivative_i
    % \left(\frac{\sum_{j\in[m]}\pricej\allocij}{\Delta}\right)
        \overset{(c)}{=}
    \valuefuncderivative_i
    \left(\sum_{j\in[m]}\ctrij\allocij\right)
    \end{align*}
    where 
    equalities~(a) (b) hold since $\moneycost_i$
    is differentiable at $\wealth\primed + \epsilon < \truewealth_i$ 
    and $\valuefunc_i$ is differentiable everywhere;
    and equality~(c) holds due to the construction 
    of $\wealth_i\primed$ and the fact that $\frac{\price_j}{\ctrij} = \Delta$
    for every $j\in \purchaseseti$ and $\allocij = 0$ for every $j\notin\purchaseseti$.
\end{proof}

Now we are ready to prove \Cref{thm:multi item concave value convex budget pure}.

\begin{proof}[Proof of \Cref{thm:multi item concave value convex budget pure}]
    Fix an arbitrary Nash equilibrium $\eqlb$.
    Suppose $\allocs,\prices$ are the allocation and per-unit price in the induced FPPE. 
    Let  
    $\mathbf\optalloc$ be the allocation in the optimal transferable welfare.
    We introduce the following partition $A_1\bigsqcup A_2\bigsqcup A_3$
    of agents based on $\allocs$, $\prices$, and $\mathbf\optalloc$:
    \begin{align*}
        A_1 &\triangleq 
        \left\{i\in[n]: \sum_{j\in[m]}\pricej\allocij = \truewealth_i\right\}
        \\
        A_2 &\triangleq
        \left\{i\in[n]: i \not\in A_1
        \land 
        \sum_{j\in[m]} \ctrij\optalloc_{ij} \leq 
        \sum_{j\in[m]} \ctrij\allocij
        \right\}
        \\
        A_3 &\triangleq
        \left\{i\in[n]: i \not\in A_1
        \land 
        \sum_{j\in[m]} \ctrij\optalloc_{ij} > 
        \sum_{j\in[m]} \ctrij\allocij
        \right\}
    \end{align*}
    In words, $A_1$ corresponds to every agent $i$ who exhausts her true budget $\truewealth_i$ in the equilibrium;
    and $A_2$, $A_3$ correspond to the remaining agents.
% 
    % For every agent $i\in A_4$, her allocation $\alloc_i$
    % is the equilibrium is at least 
    % \begin{align*}
    %     \alloci 
    %     % \overset{(a)}{\geq}
    %     % 1 - \frac{\price}{\valuefuncderivative_i(\alloci)}
    %     \overset{(a)}{\geq} 
    %     1 - \frac{\price}{\valuefuncderivative_i(\alloc_i)}
    %     \moneycostderivative_i(\price\alloci)
    %     \overset{(b)}{\geq}
    %     1 - \frac{1}{\pricethreshold}
    %     = 
    %     \frac{\pricethreshold - 1}{\pricethreshold}
    % \end{align*}
    % where inequality~(a) is guaranteed due to \Cref{lem:alloc lower bound single item concave value hard budget};
    % % inequality~(b) holds since $\optalloc_i > \alloci$
    % % and the concavity of valuation function $\valuefunc_i$;
    % and inequality~(b) is guaranteed since $\valuefuncderivative_i(\alloc_i) > \pricethreshold\cdot \price\moneycostderivative_i(\price\alloci)$.
% 
    Next, we compare the transferable welfare contribution from $A_1, A_2, A_3$ separately.

    \smallskip
    For every agent $i\in A_1$, note that 
    \begin{align*}
        \wtp_i(\optalloc_i) 
        \overset{(a)}{\leq} \truewealth_i
        \overset{(b)}{=}
        \wtp_i(\alloci)
    \end{align*}
    where the inequality holds due to the definition of $\wtp_i$;
    and the equality holds due to the definition of $A_1$.
    
    For every agent $i\in A_2$, note that 
    \begin{align*}
        \wtp_i(\optalloc_i) \leq \wtp_i(\alloci)
    \end{align*}
    where the inequality holds since 
    $\sum_{j\in[m]} \ctrij\optalloc_{ij} \leq 
        \sum_{j\in[m]} \ctrij\allocij$
        implied by the definition of $A_2$.

    For every agent $i\in A_3$, 
    let $\purchaseseti \triangleq \{j\in[m]:\allocij > 0\}$
    be the subset of items allocated to agent $i$,
    and $\Delta \triangleq \frac{\sum_{j\in \purchaseseti}\price_j}{\sum_{j\in \purchaseseti}\ctrij}$.
Due to the definition of FPPE, 
$\frac{\price_j}{\ctrij} \geq \Delta$ for every item $j\in[m]$,
and it becomes equality when $j\in \purchaseseti$.
    Note that 
    \begin{align*}
        \wtp_i(\optalloc_i) 
        &\overset{(a)}{\leq} 
        \wtp_i(\alloci) + 
        \frac{
        \valuefunc_i\left(\sum_{j\in[m]} \ctrij\optalloc_{ij}  
        \right) - 
        \valuefunc_i\left(
        \sum_{j\in[m]} \ctrij\allocij
        \right)
        }{
        \moneycostderivative_i(\wtp_i(\alloci))
        }
        \\
        &\overset{(b)}{\leq} 
         \wtp_i(\alloci) + 
        \frac{
        \valuefunc_i\left(\sum_{j\in[m]} \ctrij\optalloc_{ij}  
        \right) - 
        \valuefunc_i\left(
        \sum_{j\in[m]} \ctrij\allocij
        \right)
        }{
        \moneycostderivative_i\left(
        \sum_{j\in[m]} \pricej\allocij\right)
        }
        \\
        &\overset{(c)}{\leq} 
         \wtp_i(\alloci) 
         + 
         \left(
         \sum_{j\in[m]} (\optalloc_{ij} -\allocij)\ctrij
         \right)
         \cdot \frac{
        \valuefuncderivative_i\left(
        \sum_{j\in[m]} \ctrij\allocij
        \right)
         }{
        \moneycostderivative_i\left(
        \sum_{j\in[m]} \pricej\allocij\right)
         }
         \\
        &\overset{(d)}{\leq}
        \wtp_i(\alloci) + 
       \left(
         \sum_{j\in[m]} (\optalloc_{ij} -\allocij)\ctrij
         \right)
         \cdot 
    \frac{\sum_{j\in \purchaseseti}\price_j}{\sum_{j\in \purchaseseti}(1-\allocij)\ctrij}
    \\
        &\overset{(e)}{\leq}
        \wtp_i(\alloci) + 
       \left(
         \sum_{j\in[m]} \optalloc_{ij}\ctrij
         \right)
         \cdot 
    \frac{\sum_{j\in \purchaseseti}\price_j}{\sum_{j\in \purchaseseti}\ctrij}
    \\
        &\overset{(g)}{=}
        \wtp_i(\alloci) + 
       \left(
         \sum_{j\in[m]} \optalloc_{ij}\ctrij
         \right)
         \cdot \Delta
        \\
        &\overset{(f)}{\leq}
        \wtp_i(\alloci) + 
        \sum_{j\in[m]} \optalloc_{ij}\pricej
    \end{align*}
    where inequality~(a) holds due to the definition of $\wtp_i$ and the convexity of $\moneycost_i$;
    inequality~(b) holds since 
    $\moneycostderivative_i$ is weakly increasing implied by
    the convexity of 
    $\moneycost_i$,
    and 
    $\wtp_i(\alloci) \geq \sum_{j\in[m]}\pricej\allocij$ which is implied by the definition of $\wtp_i$ and 
    the fact that 
    agent $i$'s utility is non-negative in the equilibrium allocation $\allocs$ and per-unit prices $\prices$;
    inequality~(c) holds due to the concavity of valuation function $\valuefunc_i$;
    inequality~(d) holds due to \Cref{lem:budget lower bound multi item concave value hard budget};
    and inequality~(e) holds 
    since $\frac{\sum_{j\in[m](\optalloc_{ij}-\allocij)\ctrij}}{\sum_{j\in[m]}(1-\allocij)\ctrij} 
    \leq \frac{\sum_{j\in[m]\optalloc_{ij}\ctrij}}{\sum_{j\in[m]}\ctrij}$ 
    by algebra;
    equality~(f) holds by the definition of $\Delta$;
    and inequality~(g) holds since
    $\frac{\price_j}{\ctrij} \geq \Delta$ for every item $j\in[m]$.

    \smallskip
    Putting all pieces together, we have the following upper bound of
    the optimal transferable welfare $\wtp(\mathbf\optalloc)$,
    \begin{align*}
    % \label{eq:welfare upper bound single item concave value hard budget}
    \begin{split}
        \wtp(\mathbf\optalloc) 
        &= 
        \sum_{i\in[n]} \wtp_i(\optalloc_i)
        % \\
        \leq \sum_{i\in A_3}\sum_{j\in[m]} \optalloc_{ij}\pricej
        +
        \sum_{i\in A_1\sqcup A_2 \sqcup A_3}
        \wtp_i(\alloci)
        \\
        &
        \overset{(a)}{\leq} 
        \sum_{j\in[m]}\pricej
        +
        \sum_{i\in A_1\sqcup A_2 \sqcup A_3}
        \wtp_i(\alloci)
        % \\
        \overset{(b)}{\leq} 
        2\wtp(\allocs)
        \end{split}
    \end{align*}
    where inequality~(a) holds since $\sum_{i\in A_3}\optalloc_{ij} \leq 1$
    for every item $j\in[m]$;
    and inequality~(b) holds since 
    $\sum_{j\in[m]}\pricej \leq \wtp(\allocs)$
    since all agents receive non-negative utility in the equilibrium allocation $\allocs$ and per-unit prices $\prices$.
\end{proof}

\subsection{A $4$-approximation Analysis for Mixed Nash}

In this subsection, we present a $4$-approximation PoA (\Cref{thm:multi item concave value convex budget mixed}) and 
an 8-approximation PoA (\Cref{thm:multi item concave value convex budget mixed 8-approx}) 
for mixed Nash when agents have linear and concave valuation functions, respectively. 
% The analysis is inspired by \citet{CST-15b}.

\begin{theorem}
\label{thm:multi item concave value convex budget mixed}
    In the multi-item environment,
    for agents with (differentiable) {\color{red}linear} valuation functions 
 $\{\valuefunc_i\}$ and 
 (differentiable) convex disutilities of money $\{\moneycost_i\}$
 up to heterogeneous budgets $\{\truewealth_i\}$,
    the mixed Nash PoA of transferable welfare 
    is at most $4$.
\end{theorem}

\newcommand{\tildePj}{\tildeP_j}
\newcommand{\optallocij}{\optalloc_{ij}}

\begin{proof}
   Fix an arbitrary mixed Nash equilibrium $\eqlb$.
    Suppose $\allocs,\prices$ are the randomized allocation and per-unit prices in the induced FPPE. 
    Let  
    $\mathbf\optalloc$ be the allocation in the optimal transferable welfare.    

    For each agent $i$, we present the following upper bound 
    of its contribution $\wtp_i(\optalloc_i)$ in the optimal transferable welfare allocation,
    \begin{align}
    \label{eq:multi item mixed wtp bound}
        \frac{1}{2}\wtp_i(\optalloc_i) \leq 
        \moneycost_i^{-1}(\util_i) + 
        \sum_{j\in[m]}\optalloc_{ij} \expect{\pricej}
    \end{align}
    where $\util_i$ is the expected utility of agent $i$ in the equilibrium $\eqlb$.
    Note that inequality~\eqref{eq:multi item mixed wtp bound}
    immediately implies the lemma statement since
    \begin{align*}
        \wtp(\mathbf\optalloc) 
        = \sum_{i\in[n]}
        \wtp_i(\optalloc_i)
        \leq 
        2
        \left(
        \sum_{i\in[n]} 
        \moneycost_i^{-1}(\util_i)
        +
        \optalloc_i \expect{\price}
        \right)
        \leq 
        4\wtp(\allocs)
    \end{align*}
    where the last inequality holds since $\moneycost_i^{-1}(\util_i) \leq 
    \moneycost_i^{-1}
    \left(
    \expect{\val_i
    \left(
    \sum_{j\in[m]}\allocij\ctrij
    \right)
    }
    \right)
    \equiv
    \wtp_i(\alloci)$;
    $\sum_{j\in[m]}\expect{\pricej} \leq  \wtp(\allocs)$;
    and $\sum_{i\in[n]}\optalloc_{ij} = 1$
    for every item $j\in[m]$.

    \smallskip
    Below we proof inequality~\eqref{eq:single item mixed wtp bound}
    by considering a specific deviation strategy for agent $i$.
    Let $\prices\doubleprimed$ be the randomized per-unit prices induced by the FPPE where agent $i$ is not participated, or equivalently, reporting $\wealth_i\doubleprimed = 0$.
    As a sanity check randomized price $\pricej\doubleprimed$ is first order stochastically dominated by randomized price $\pricej$ for every item $j\in[m]$.
    
    Let $\tildePj\doubleprimed \triangleq \expect{\pricej\doubleprimed}$
    for every item $j\in[m]$.
    Now consider the following deviating strategy for agent $i$
    where agent $i$ deterministically reports 
    \begin{align*}
        \val_i\primed = \infty,\quad 
        \wealth_i\primed = 
        \sum_{j\in[m]}
        \optalloc_{ij}  
        \tildePj\doubleprimed
    \end{align*}
    Let $\allocs\primed,\prices\primed$ be the randomized allocation and per-unit prices in the induced FPPE after this deviation of agent $i$.
    Since agent $i$ reports $\val_i\primed = \infty$, 
    she always exhausts her reported budget$~\wealth_i\primed$.
    
    In the remaining analysis,
    we couple the report profiles of all other agents except agent~$i$ in the FPPE inducing randomized per-unit prices $\prices\doubleprimed$, and the FPPE inducing randomized 
    allocation~$\allocs\primed$ and per-unit prices $\prices\primed$.
    As a sanity check, 
    it is straightforward to verify that 
    \begin{align*}
        \pricej\doubleprimed \leq \pricej\primed
        \text{ for every $j\in[m]$, and }
        \sum_{j\in[m]}\pricej\primed \leq 
        \sum_{j\in[m]}\pricej\doubleprimed + \wealth_i\primed
    \end{align*}
    for every realization of agents' reports.
    Let $\tildePj\primed = \expect{\pricej\primed}$.
    By definition, $\sum_{j\in[m]}\tildePj\primed - \tildePj\doubleprimed\leq \wealth\primed$.
    
    The expected utility $\util_i$
    of agent $i$ is at least her expected utility under this deviation,
    i.e., 
    \begin{align*}
        \util_i 
        &\overset{(a)}{\geq} 
        \expect
        [\price\primed]
        {
        \valuefunc_i\left(
        \left(
        \max_{j\in[m]}
        \frac{\ctrij}{\pricej\primed}
        \right)
        \wealth_i\primed
        \right)
        -
        \moneycost_i\left(\wealth_i\primed\right)}
        \\
        &\overset{(b)}{\geq} 
        \expect
        [\price\primed]
        {
        \valuefunc_i\left(
        \left(
        \max_{j\in[m]}
        \frac{\ctrij}{\pricej\primed}
        \right)
        \left(
        \sum_{j\in[m]}
        \frac{1}{2}
        \left(
        \optallocij\tildePj\doubleprimed +
        \left(\tildePj\primed - \tildePj\doubleprimed\right)
        \right)
        \right)
        \right)}
        -
        \moneycost_i\left(
        \sum_{j\in[m]}
        \optalloc_{ij}  
        \tildePj\doubleprimed
        \right)
        \\
        &\overset{(c)}{\geq} 
        \expect
        [\price\primed]
        {
        \valuefunc_i\left(
        \left(
        \max_{j\in[m]}
        \frac{\ctrij}{\pricej\primed}
        \right)
        \left(
        \sum_{j\in[m]}
        \frac{1}{2}
        \optallocij
        \tildePj\primed
        \right)
        \right)}
        -
        \moneycost_i\left(
        \sum_{j\in[m]}
        \optalloc_{ij}  
        \tildePj\doubleprimed
        \right)
        \\
        &\overset{(d)}{\geq} 
        \expect
        [\price\primed]
        {
        \valuefunc_i\left(
        \sum_{j\in[m]}
        \frac{1}{2}
        \frac{\ctrij}{\pricej\primed}
        \optallocij
        \tildePj\primed
        \right)}
        -
        \moneycost_i\left(
        \sum_{j\in[m]}
        \optalloc_{ij}  
        \tildePj\doubleprimed\right)
        \\
        &\overset{(e)}{=} 
        \expect
        [\price\primed]
        {
        \sum_{j\in[m]}
        \frac{\tildePj\primed}{\pricej\primed}
        \valuefunc_i\left(
        \frac{1}{2}
        {\ctrij}
        \optallocij
        \right)}
        -
        \moneycost_i\left(
        \sum_{j\in[m]}
        \optalloc_{ij}  
        \tildePj\doubleprimed\right)
        \\
        &\overset{(f)}{\geq} 
        {
        \sum_{j\in[m]}
        \frac{\tildePj\primed}{\expect
        [\price\primed]{\pricej\primed}}
        \valuefunc_i\left(
        \frac{1}{2}
        {\ctrij}
        \optallocij
        \right)}
        -
        \moneycost_i\left(
        \sum_{j\in[m]}
        \optalloc_{ij}  
        \tildePj\doubleprimed\right)
        \\
        &\overset{(g)}{=} 
        \valuefunc_i\left(
        \sum_{j\in[m]}
        \frac{1}{2}
        {\ctrij}
        \optallocij
        \right)
        -
        \moneycost_i\left(
        \sum_{j\in[m]}
        \optalloc_{ij}  
        \tildePj\doubleprimed\right)
    \end{align*}
    where inequality~(a) holds due to the construction of FPPE;
    inequality~(b) holds since $\wealth_i\primed = \sum_{j\in[m]}\optallocij\tildePj\doubleprimed$
    and $\wealth_i\primed \geq \sum_{j\in[m]}\tildePj\primed - \tildePj\doubleprimed$;
     inequality~(c) holds since $\optallocij \leq 1$;
     inequality~(d) holds by algebra;
     {\color{red}equalities~(e) (g) hold due to the linearity of valuation function $\valuefunc_i$};
     and inequality~(f) holds due to Jensen's inequality.

    Finally, applying concave function 
    $\moneycost_i^{-1}$ 
    to both side,
        we obtain
    \begin{align*}
        \frac{1}{2}\wtp_i(\optalloc_i) 
        &\leq 
        \moneycost_i^{-1}\left(
        \valuefunc_i\left(
        \sum_{j\in[m]}
        \frac{1}{2}
        {\ctrij}
        \optallocij
        \right)
        \right)
        \leq 
        \moneycost_i^{-1}\left(
        \util_i + 
        \moneycost_i\left(\sum_{j\in[m]}
        \optalloc_{ij}  
        \tildePj\doubleprimed\right)
        \right)
        \\
        &\leq 
        \moneycost_i^{-1}\left(
        \util_i  \right)
        +
        \sum_{j\in[m]}
        \optalloc_{ij}  
        \tildePj\doubleprimed
        \leq 
        \moneycost_i^{-1}\left(
        \util_i  \right)
        +
        \sum_{j\in[m]}
        \optalloc_{ij}  
        \expect{\pricej}
    \end{align*}
    where the first and third inequality hold
    due to the convexity of $\moneycost_i$;
    the second inequality holds due to the monotonicity of $\moneycost_i$;
    and the last inequality holds since $\pricej$
    first order stochastically dominates $\pricej\doubleprimed$ and thus $\expect{\pricej}
    \geq \expect{\pricej\doubleprimed} \equiv \tildePj\doubleprimed$
    for every item $j\in[m]$.
\end{proof}

Below we present an 8-approximation PoA guarantee for mixed Nash
when agents have concave valuation functions. 

\begin{theorem}
\label{thm:multi item concave value convex budget mixed 8-approx}
    In the multi-item environment,
    for agents with (differentiable) {\color{black}concave} valuation functions 
 $\{\valuefunc_i\}$ and 
 (differentiable) convex disutilities of money $\{\moneycost_i\}$
 up to heterogeneous budgets $\{\truewealth_i\}$,
    the mixed Nash PoA of transferable welfare 
    is at most $8$.
\end{theorem}
\begin{proof}
    The analysis follows the same argument as the one in \Cref{thm:multi item concave value convex budget mixed} 
    until the step where we present the lower bound of the agent $i$'s utility, 
    i.e., 
    
    \begin{align}
    \nonumber
        \util_i 
        &\overset{}{\geq} 
        \expect
        [\price\primed]
        {
        \valuefunc_i\left(
        \left(
        \max_{j\in[m]}
        \frac{\ctrij}{\pricej\primed}
        \right)
        \wealth_i\primed
        \right)
        -
        \moneycost_i\left(\wealth_i\primed\right)}
        \\
        \label{eq:multi item 2 approx relax}
        &\overset{}{\geq} 
        \expect
        [\price\primed]
        {
        \valuefunc_i\left(
        \frac{1}{2}
        \sum_{j\in[m]}
        \frac{\optallocij\tildePj\doubleprimed}{\pricej\doubleprimed
        +\tildePj\doubleprimed}
        \ctrij
        \right)}
        -
        \moneycost_i\left(
        \sum_{j\in[m]}
        \optalloc_{ij}  
        \tildePj\doubleprimed
        \right)
        \\
        \label{eq:multi item expectation}
        &\overset{}{\geq} 
        {
        \frac{1}{4}
        \valuefunc_i\left(
        \sum_{j\in[m]}
        \optallocij
        \ctrij
        \right)}
        -
        \moneycost_i\left(
        \sum_{j\in[m]}
        \optalloc_{ij}  
        \tildePj\doubleprimed
        \right)
    \end{align}
    Below we discuss inequalities~\eqref{eq:multi item 2 approx relax}\eqref{eq:multi item expectation} in details.
    
    \paragraph{Inequality~\eqref{eq:multi item 2 approx relax}}
    It 
    is sufficient to argue that for every realization of agents' reports and thus induced per-unit prices $\pricej\primed$,
    \begin{align*}
    \left(
        \max_{j\in[m]}
        \frac{\ctrij}{\pricej\primed}
        \right)
        \wealth_i\primed
        \geq 
        \frac{1}{2}
        \sum_{j\in[m]}
        \frac{\optallocij\tildePj\doubleprimed}{\pricej\doubleprimed
        +\tildePj\doubleprimed}
        \ctrij
    \end{align*}
    To see this, we first partition all $m$ items into $\hitems\sqcup \litems$ where 
    \begin{align*}
        \hitems &\triangleq \left\{j\in[m]: \pricej\primed \geq \pricej\doubleprimed + \optallocij\tildePj\doubleprimed
        \right\}
        \\
        \litems &\triangleq \left\{j\in[m]: \pricej\primed < \pricej\doubleprimed + \optallocij\tildePj\doubleprimed
        \right\}
    \end{align*}
    For every item $j\in \hitems$, we have
    \begin{align*}
        \frac{\optallocij\tildePj\doubleprimed}{\pricej\doubleprimed
        +\tildePj\doubleprimed}
        \ctrij
        &
        \overset{(a)}{\leq}
        \frac{\optallocij\tildePj\doubleprimed}{\pricej\doubleprimed
        +\optallocij\tildePj\doubleprimed}
        \ctrij
        \overset{(b)}{\leq}
        \frac{\pricej\primed - \pricej\doubleprimed}
        {\pricej\doubleprimed
        +\left(\pricej\primed - \pricej\doubleprimed\right)}
        \ctrij
        =
        \frac{\ctrij}
        {\pricej\primed
        }
        \left(\pricej\primed - \pricej\doubleprimed\right)
    \end{align*}
    where inequality~(a) holds since $\optallocij \leq 1$;
    and inequality~(b) holds since $j\in \hitems$.

    For every item $j\in\litems$, we have  
    \begin{align*}
        \frac{\optallocij\tildePj\doubleprimed}{\pricej\doubleprimed
        +\tildePj\doubleprimed}
        \ctrij
        &
        \overset{(a)}{\leq}
        \frac{\optallocij\tildePj\doubleprimed}{\pricej\doubleprimed
        +\optallocij\tildePj\doubleprimed}
        \ctrij
        \overset{(b)}{\leq}
        \frac{\optallocij\tildePj\doubleprimed}
        {\pricej\primed}
        \ctrij
        =
        \frac{\ctrij}
        {\pricej\primed
        }
        \optallocij\tildePj\doubleprimed
    \end{align*}
    where inequality~(a) holds since $\optallocij \leq 1$;
    and inequality~(b) holds since $j\in \litems$.

    Note that by construction
    \begin{align*}
        \sum_{j\in[m]}\optallocij\tildePj\doubleprimed = \wealth_i\primed;
        \qquad
        \sum_{j\in[m]}\pricej\primed - \pricej\doubleprimed \leq \wealth_i\primed;   
        \qquad
        \text{and}
        \qquad
        \pricej\primed \geq \pricej\doubleprimed
        \text{ for every $j\in[m]$}
    \end{align*}
    and thus
    \begin{align*}
        \left(
        \max_{j\in[m]}
        \frac{\ctrij}{\pricej\primed}
        \right)
        \wealth_i\primed
        &\geq 
        \frac{1}{2}
        \left(
        \max_{j\in[m]}
        \frac{\ctrij}{\pricej\primed}
        \right)
        \left(
        \sum_{j\in[m]}\optallocij\tildePj\doubleprimed
        +
        \sum_{j\in[m]}\pricej\primed - \pricej\doubleprimed
        \right)
        \\
        &\geq 
        \frac{1}{2}
        \left(
        \max_{j\in[m]}
        \frac{\ctrij}{\pricej\primed}
        \right)
        \left(
        \sum_{j\in\litems}\optallocij\tildePj\doubleprimed
        +
        \sum_{j\in\hitems}\pricej\primed - \pricej\doubleprimed
        \right)
        \\
        &\geq 
        \frac{1}{2}
        \left(
        \sum_{j\in\litems}
        \frac{\ctrij}{\pricej\primed}
        \optallocij\tildePj\doubleprimed
        +
        \sum_{j\in\hitems}
        \frac{\ctrij}{\pricej\primed}
        \left(\pricej\primed - \pricej\doubleprimed\right)
        \right)
        \\
        &\geq 
        \frac{1}{2}
        \sum_{j\in[m]}
        \frac{\optallocij\tildePj\doubleprimed}{\pricej\doubleprimed
        +\tildePj\doubleprimed}
        \ctrij
    \end{align*}
    as desired.

    \paragraph{Inequality~\eqref{eq:multi item expectation}}
    By algebra, we have 
    \begin{align*}
        &\expect
        [\price\primed]
        {
        \valuefunc_i\left(
        \frac{1}{2}
        \sum_{j\in[m]}
        \frac{\optallocij\tildePj\doubleprimed}{\pricej\doubleprimed
        +\tildePj\doubleprimed}
        \ctrij
        \right)}
        \\
        \overset{(a)}{\geq} 
        &
        \expect
        [\price\primed]
        {
        \frac{1}{2}
        \frac{
        \sum_{j\in[m]}
        \frac{\tildePj\doubleprimed}{\pricej\doubleprimed
        +\tildePj\doubleprimed}
        \optallocij\ctrij
        }{\sum_{j\in[m]}
        \optallocij\ctrij
        }
        \valuefunc_i\left(
        \sum_{j\in[m]}
        \optallocij
        \ctrij
        \right)}
        \\
        \overset{(b)}{\geq} 
        &
        \frac{1}{2}
        \frac{
        \sum_{j\in[m]}
        \expect
        [\pricej\doubleprimed]
        {
        \frac{\tildePj\doubleprimed}{\pricej\doubleprimed
        +\tildePj\doubleprimed}
        \optallocij\ctrij
        }
        }
        {\sum_{j\in[m]}
        \optallocij\ctrij
        }
        \valuefunc_i\left(
        \sum_{j\in[m]}
        \optallocij
        \ctrij
        \right)
        \\
        \overset{(c)}{\geq} 
        &
        \frac{1}{2}
        \frac{
        \sum_{j\in[m]}
        {
        \frac{\tildePj\doubleprimed}{
        \expect
        [\pricej\doubleprimed]{\pricej\doubleprimed}
        +\tildePj\doubleprimed}
        \optallocij\ctrij
        }
        }
        {\sum_{j\in[m]}
        \optallocij\ctrij
        }
        \valuefunc_i\left(
        \sum_{j\in[m]}
        \optallocij
        \ctrij
        \right)
        \\
        \overset{(d)}{=} 
        &
        \frac{1}{4}
        \valuefunc_i\left(
        \sum_{j\in[m]}
        \optallocij
        \ctrij
        \right)
    \end{align*}
    where inequality~(a) holds 
    since valuation function $\valuefunc_i$ is concave and 
    $0\leq 
        \frac{1}{2}
        \frac{
        \sum_{j\in[m]}
        \frac{\tildePj\doubleprimed}{\pricej\doubleprimed
        +\tildePj\doubleprimed}
        \optallocij\ctrij
        }{\sum_{j\in[m]}
        \optallocij\ctrij
        } \leq 1$;
    inequality~(b) holds due to the linearity of expectation;
    inequality~(c) holds since $\frac{\tildePj\doubleprimed}{a + \tildePj\doubleprimed}$ is convex in $a\geq 0$;
    and equality~(d) holds since $\expect{\pricej\doubleprimed} = \tildePj\doubleprimed$.
\end{proof}

\begin{remark}
    To improve the 8-approximation 
    in \Cref{thm:multi item concave value convex budget mixed 8-approx}
    to a 4-approximation,
    one natural attempt is to show inequality~\eqref{eq:multi item 2 approx relax} holds without the additional loss factor of 2, i.e., 
\begin{align*}
    \left(
        \max_{j\in[m]}
        \frac{\ctrij}{\pricej\primed}
        \right)
        \wealth_i\primed
        \geq 
        \sum_{j\in[m]}
        \frac{\optallocij\tildePj\doubleprimed}{\pricej\doubleprimed
        +\tildePj\doubleprimed}
        \ctrij
\end{align*}
Unfortunately, this inequality does not holds (given the current characterization of $\wealth_i\primed, \pricej\primed, \pricej\doubleprimed$). 
To see this, consider the following variable assignment:
there are $m=2$ items, and other variables are as follows\footnote{For notation simplicity, we drop index $i$.}
\begin{align*} 
    \ctr_{1} &= 2 \quad \ctr_2 = 1
    \\
    \price_1\doubleprimed &= 1 \quad \price_2\doubleprimed = 1
    \\
    \optalloc_1 &= 1 \quad \optalloc_2 = 1
    \\
    \tildeP_1\doubleprimed &= 1 \quad \tildeP_2\doubleprimed = \frac{1}{2}
    \\
    \price_1\primed &= \frac{7}{3}
    \quad 
    \price_2\primed = \frac{7}{6}
    \\
    \wealth\primed &= \frac{3}{2}
\end{align*}
It is straightforward to verify that 
\begin{align*}
\sum_{j\in[m]}\optalloc_j\tildePj\doubleprimed = \wealth\primed;
        \mbox{   and    }
        \sum_{j\in[m]}\pricej\primed - \pricej\doubleprimed = \wealth\primed    
\end{align*}
but 
\begin{align*}
     \left(
        \max_{j\in[m]}
        \frac{\ctr_j}{\pricej\primed}
        \right)
        \wealth\primed
        =
        \frac{9}{7}
        <
        \frac{4}{3}
        =
        \sum_{j\in[m]}
        \frac{\optalloc_j\tildePj\doubleprimed}{\pricej\doubleprimed
        +\tildePj\doubleprimed}
        \ctr_j
\end{align*}
\end{remark}

==> Notes/multi-item-new-analysis.tex <==
\section{New Analysis for Multiple Items}



In this section, we consider the multi-item environments,
where each agent $i$'s utility given allocation $\allocs$
and per-unit prices $\prices$ is 
$$\util_i(\allocs, \prices) = 
\valuefunc_i\left(
\sum_{j\in[m]} 
\ctrij \cdot \allocij
\right)
-
\moneycost_i\left(
\sum_{j\in[m]}\price_j \cdot \allocij
\right)$$
where $\ctrij$ is the \emph{click-through-rate}
commonly known in the inner FPPE.
Each agent $i$ reports a value $\val_i$ and budget $\wealth_i$, and the inner FPPE assumes 
that agent $i$ has $\val_i \cdot \ctrij$ for
each item $j$ and budget $\wealth_i$.

\subsection{A 2-approximation Analysis for Pure Nash}

The pure Nash PoA guarantee is as follows.
 
\begin{theorem}
\label{thm:multi item concave value convex budget pure}
    In the multi-item environment,
    for agents with (differentiable) concave valuation functions 
 $\{\valuefunc_i\}$ and 
 (differentiable) convex disutilities of money $\{\moneycost_i\}$
 up to heterogeneous budgets $\{\truewealth_i\}$,
    the pure Nash PoA of transferable welfare 
    is at most $2$.
\end{theorem}

Our analysis relies on the following technical lemma, which generalizes
\Cref{lem:alloc lower bound single item concave value hard budget}
from single-item environment to the multi-item environment.
\begin{lemma}
\label{lem:budget lower bound multi item concave value hard budget}
    In the multi-item environment,
    for agents with (differentiable) concave valuation functions 
 $\{\valuefunc_i\}$ and 
 (differentiable) convex disutilities of money $\{\moneycost_i\}$
 up to heterogeneous budgets $\{\truewealth_i\}$,
and every pure Nash equilibrium $\eqlb$,
suppose $\xbf, \prices$
are the allocation and per-unit prices in the induced FPPE.
For every agent $i$ who does not exhaust her true budget $\truewealth_i$,
i.e., $\sum_{j}\alloc_{ij}\cdot \price_j < \truewealth_i$,
her payment $\sum_{j\in[m]}\price_j\allocij$ is at least 
\begin{align*}
\frac
    {\valuefuncderivative_i
    \left(\sum_{j\in[m]}\ctrij\allocij\right)}
{\moneycostderivative_i
    \left(\sum_{j\in[m]}\price_j\allocij\right)}
    \leq 
    \frac{\sum_{j\in \purchaseseti}\price_j}{\sum_{j\in \purchaseseti}(1-\allocij)\ctrij}
\end{align*}
where $H_i \triangleq \{j\in[m]: \alloc_{ij} > 0\}$
includes all items which agent $i$ is allocated.
\end{lemma}

To see \Cref{lem:budget lower bound multi item concave value hard budget} extends \Cref{lem:alloc lower bound single item concave value hard budget},
observe that $\ctrij=1$ in the single-item environment.

\begin{proof}[Proof of \Cref{lem:budget lower bound multi item concave value hard budget}]
    Fix an arbitrary Nash equilibrium $\eqlb$.
    Suppose $\allocs,\prices$ are the allocation and per-unit price in the induced FPPE.
    Fix an arbitrary agent $i$ who does not exhaust her true budget $\truewealth_i$,
i.e., $\sum_j\price_j\allocij < \truewealth_i$.
Let $\Delta \triangleq \frac{\sum_{j\in \purchaseseti}\price_j}{\sum_{j\in \purchaseseti}\ctrij}$.
Due to the definition of FPPE, 
$\frac{\price_j}{\ctrij} \geq \Delta$ for every item $j\in[m]$,
and it becomes equality when $j\in \purchaseseti$.
In the remaining argument, we further assume 
that $\valuefuncderivative_i(\sum_{j\in[m]}\ctrij\allocij) > \Delta$;
otherwise, 
\begin{align*}
    \frac
    {\valuefuncderivative_i
    \left(\sum_{j\in[m]}\ctrij\allocij\right)}
{\moneycostderivative_i
    \left(\sum_{j\in[m]}\price_j\allocij\right)}
    \leq 
    \valuefuncderivative_i
    \left(\sum\nolimits_{j\in[m]}\ctrij\allocij\right)
    \leq 
    \Delta 
    =
    \frac{\sum_{j\in \purchaseseti}\price_j}{\sum_{j\in \purchaseseti}\ctrij}
    \leq 
    \frac{\sum_{j\in \purchaseseti}\price_j}{\sum_{j\in \purchaseseti}(1-\allocij)\ctrij}
\end{align*}
and thus the lemma statement holds trivially.



    Firstly,
    we note that the same FPPE and thus the same utility for every agent are induced
    if 
    we hold all other agents' reports fixed and let 
    agent $i$ report
    $\val_i\primed \triangleq
    \valuefuncderivative_i(\sum_{j\in[m]}\ctrij\allocij)$ 
    and $\wealth_i\primed \triangleq \sum_{j\in [m]} \price_j\allocij$.
    By the definition of $\purchaseseti$, we know that $
    \wealth_i\primed = 
    \sum_{j\in \purchaseseti}\pricej\allocij$.
    Now suppose that
    agent $i$ keeps her reported value $\val\doubleprimed = \val\primed$ the same, but
    increases her reported budget by $\epsilon$
    for sufficiently small and positive $\epsilon < 
    \min\{\truewealth_i - \wealth_i\primed,
    \min_{j\in \purchaseseti}
    \val_i\doubleprimed \ctrij - \price_j
    \}
    $,
    i.e., $\wealth_i\doubleprimed = \wealth_i\primed + \epsilon < \truewealth_i$.
    Let $\allocs\doubleprimed,\prices\doubleprimed$ be 
    the allocation and per-unit price in the new induced FPPE.
    We have 
    \begin{align*}
        \sum_{j\in \purchaseseti}\price_j\doubleprimed \overset{(a)}{\leq} 
        \epsilon + \sum_{j\in \purchaseseti}\price_j
    \end{align*}
    where inequality~(a) holds due to the construction of per-unit price in FPPE (\Cref{lem:fppe increasing budget}).
    In this new induced FPPE, the utility $\util_i\doubleprimed$ of agent $i$ is 
    \begin{align*}
    \util_i\doubleprimed
    &\overset{(a)}{=}
        \valuefunc_i\left(
        \left(\max_{j\in[m]}
        \frac{\ctrij}{\price_j\doubleprimed}
        \right)
        \cdot 
        \sum_{j\in[m]}
            \price_j\doubleprimed
            \allocij\doubleprimed
        \right) 
        - \moneycost_i\left(
            \sum_{j\in[m]}
            \price_j\doubleprimed
            \allocij\doubleprimed
        \right)
        \\
        &\geq 
        \valuefunc_i\left(
        \frac{\sum_{j\in \purchaseseti}\ctrij}
        {\sum_{j\in \purchaseseti}
        \price_j\doubleprimed}
        \cdot 
        \sum_{j\in[m]}
            \price_j\doubleprimed
            \allocij\doubleprimed
        \right) 
        - \moneycost_i\left(
            \sum_{j\in[m]}
            \price_j\doubleprimed
            \allocij\doubleprimed
        \right)
        \\
        &\overset{(b)}{=} 
        \valuefunc_i\left(
        \frac{\sum_{j\in \purchaseseti}\ctrij}
        {\sum_{j\in \purchaseseti}
        \price_j\doubleprimed}
        \cdot 
        \wealth\doubleprimed
        \right) 
        - \moneycost_i\left(
            \wealth\doubleprimed
        \right)
        \\
        &\geq  
        \valuefunc_i\left(
        \frac{\sum_{j\in \purchaseseti}\ctrij}
        {\epsilon+ \sum_{j\in \purchaseseti}
        \price_j}
        \cdot 
        \left(
        \wealth\primed
        +
        \epsilon
        \right)
        \right) 
        - \moneycost_i\left(
            \wealth\primed
            +
            \epsilon
        \right)
        \\
        &\overset{(c)}{=}  
        \valuefunc_i\left(
        % \frac{1}{\frac{\epsilon}{\sum_{j\in\purchaseseti}\price_j}+1}
        \frac{\sum_{j\in\purchaseseti}\price_j}
        {\epsilon+\sum_{j\in\purchaseseti}\price_j}
        \frac{
        \wealth\primed
        +
        \epsilon
        }{\Delta}
        \right) 
        - \moneycost_i\left(
            \wealth\primed
            +
            \epsilon
        \right)
    \end{align*}
    where 
    equality~(a) holds by 
    the construction of FPPE;
    equality~(b) holds due to 
    the unnecessary pacing constraint implied 
    by the construction of $\val_i\doubleprimed$ and $\epsilon$;
    and equality~(c) holds 
    since $\frac{\price_j}{\ctrij} = \Delta$
    for every $j\in \purchaseseti$.
    With a similar argument, the utility $\util_i$
    of agent $i$ in the original FPPE induced by equilibrium $\eqlb$
    is 
    \begin{align*}
    \util_i
    &=
        \valuefunc_i\left(
        \left(\max_{j\in[m]}
        \frac{\ctrij}{\price_j}
        \right)
        \cdot 
        \sum_{j\in[m]}
            \price_j
            \allocij
        \right) 
        - \moneycost_i\left(
            \sum_{j\in[m]}
            \price_j
            \allocij
        \right)
        \\
        &= 
        \valuefunc_i\left(
        \frac{\sum_{j\in \purchaseseti}\ctrij}
        {\sum_{j\in \purchaseseti}
        \price_j}
        \cdot 
        \sum_{j\in[m]}
            \price_j
            \allocij
        \right) 
        - \moneycost_i\left(
            \sum_{j\in[m]}
            \price_j
            \allocij
        \right)
        \\
        &= 
        \valuefunc_i\left(
        \frac{\sum_{j\in \purchaseseti}\ctrij}
        {\sum_{j\in \purchaseseti}
        \price_j}
        \cdot 
        \wealth\primed
        \right) 
        - \moneycost_i\left(
            \wealth\primed
        \right)
        \\
        &=  
        \valuefunc_i\left(
        \frac{
        \wealth\primed}
        {\Delta}
        \right) 
        - \moneycost_i\left(
            \wealth\primed
        \right)
    \end{align*}
    Note that $\util_i - \util_i\doubleprimed \geq 0$ 
    since the former is the utility in the equilibrium, and the later
    is the utility after the deviation.
    Furthermore, we have 
    \begin{align*}
        \util_i - \util_i\doubleprimed
        &\leq \valuefunc_i\left(
        \frac{\wealth\primed}
        {\Delta}
        \right) 
        - \moneycost_i\left(
            \wealth\primed
        \right)
        - 
        \left(
        \valuefunc_i\left(
        \frac{\sum_{j\in\purchaseseti}\price_j}
        {\epsilon+\sum_{j\in\purchaseseti}\price_j}
        \frac{
        \wealth\primed
        +
        \epsilon
        }{\Delta}
        \right) 
        - \moneycost_i\left(
            \wealth\primed
            +
            \epsilon
        \right)
        \right)
        \\
        &= 
        \moneycost_i(\wealth_i\primed + \epsilon)
        - 
        \moneycost_i(\wealth_i\primed)
        -
         \left(
         \valuefunc_i\left(
        \frac{\sum_{j\in\purchaseseti}\price_j}
        {\epsilon+\sum_{j\in\purchaseseti}\price_j}
        \frac{
        \wealth\primed
        +
        \epsilon
        }{\Delta}
        \right) 
        -
        \valuefunc_i\left(
        \frac{
        \wealth\primed
        }{\Delta}
        \right) 
         \right)
        \\
        &\overset{(a)}{\leq}
        \epsilon
        \cdot 
        \moneycostderivative_i(\wealth\primed + \epsilon)
        -
        \left(
        \frac{\sum_{j\in\purchaseseti}\price_j}
        {\epsilon+\sum_{j\in\purchaseseti}\price_j}
        \frac{
        \wealth\primed
        +
        \epsilon
        }{\Delta}
        -
        \frac{
        \wealth\primed
        }{\Delta}
        \right)
        \cdot 
         \valuefuncderivative_i
         \left(
         \frac{\sum_{j\in\purchaseseti}\price_j}
        {\epsilon+\sum_{j\in\purchaseseti}\price_j}
        \frac{
        \wealth\primed
        +
        \epsilon
        }{\Delta}
        \right)
         \\
         &\overset{}{=}
         \epsilon
        \cdot 
        \moneycostderivative_i(\wealth\primed + \epsilon)
        -
        \frac{\epsilon}{\Delta}
        \cdot 
        \frac{\sum_{j\in\purchaseseti}\pricej -
        \wealth_i\primed}{\sum_{j\in\purchaseseti}\price_j + \epsilon}
        \cdot 
         \valuefuncderivative_i
         \left(
         \frac{\sum_{j\in\purchaseseti}\price_j}
        {\epsilon+\sum_{j\in\purchaseseti}\price_j}
        \frac{
        \wealth\primed
        +
        \epsilon
        }{\Delta}
        \right)
         \\
         &\overset{(b)}{=}
         \epsilon
        \cdot 
        \moneycostderivative_i(\wealth\primed + \epsilon)
        -
        \epsilon
        \cdot 
        \frac{\sum_{j\in\purchaseseti}(1-\allocij)\ctrij
        }
        {\sum_{j\in\purchaseseti}\price_j + \epsilon}
        \cdot 
         \valuefuncderivative_i
         \left(
         \frac{\sum_{j\in\purchaseseti}\price_j}
        {\epsilon+\sum_{j\in\purchaseseti}\price_j}
        \frac{
        \wealth\primed
        +
        \epsilon
        }{\Delta}
        \right)
    \end{align*}
    where inequality~(a) holds since $\alloci\doubleprimed > \alloci$, valuation function $\valuefunc_i$
    is concave and differentiable,
    and 
    disutility of money $\moneycost_i$
    is convex and differentiable up to $\truewealth_i$;
    and equality~(b) holds since $\frac{\price_j}{\ctrij} = \Delta$
    for every $j\in \purchaseseti$, and thus $\frac{1}{\Delta}(\sum_{j\in\purchaseseti}\pricej - \wealth_i\primed) =
    \frac{1}{\Delta}(\sum_{j\in\purchaseseti}\pricej - \sum_{j\in\purchaseseti}\pricej\allocij) = 
    \sum_{j\in\purchaseseti}(1-\allocij)\ctrij$.
    After rearranging the terms,
    we have 
    \begin{align*}
           \frac
    {\valuefuncderivative_i
         \left(
         \frac{\sum_{j\in\purchaseseti}\price_j}
        {\epsilon+\sum_{j\in\purchaseseti}\price_j}
        \frac{
        \wealth\primed
        +
        \epsilon
        }{\Delta}
        \right)}
{\moneycostderivative_i(\wealth\primed + \epsilon)}
    \leq 
    \frac{\sum_{j\in \purchaseseti}\price_j + \epsilon}{\sum_{j\in \purchaseseti}(1-\allocij)\ctrij}
    \end{align*}
    for all positive $\epsilon$ that is sufficiently small.
    Finally, letting $\epsilon$ go to zero, 
    the lemma statement is obtained as
    \begin{align*}
    &\lim_{\epsilon\rightarrow 0}
    \moneycostderivative_i(\wealth\primed + \epsilon)
    \overset{(a)}{=}
    \moneycostderivative_i(\wealth\primed)
    =
    \moneycostderivative_i\left(\sum_{j\in [m]}\pricej\allocij\right)
    \\
        &\lim_{\epsilon\rightarrow 0}
        \valuefuncderivative_i
         \left(
         \frac{\sum_{j\in\purchaseseti}\price_j}
        {\epsilon+\sum_{j\in\purchaseseti}\price_j}
        \frac{
        \wealth\primed
        +
        \epsilon
        }{\Delta}
        \right)
        \overset{(b)}{=}
        \valuefuncderivative_i
         \left(
        \frac{
        \wealth\primed
        }{\Delta}
        \right)
    %     =
    %     \valuefuncderivative_i
    % \left(\frac{\sum_{j\in[m]}\pricej\allocij}{\Delta}\right)
        \overset{(c)}{=}
    \valuefuncderivative_i
    \left(\sum_{j\in[m]}\ctrij\allocij\right)
    \end{align*}
    where 
    equalities~(a) (b) hold since $\moneycost_i$
    is differentiable at $\wealth\primed + \epsilon < \truewealth_i$ 
    and $\valuefunc_i$ is differentiable everywhere;
    and equality~(c) holds due to the construction 
    of $\wealth_i\primed$ and the fact that $\frac{\price_j}{\ctrij} = \Delta$
    for every $j\in \purchaseseti$ and $\allocij = 0$ for every $j\notin\purchaseseti$.
\end{proof}

Now we are ready to prove \Cref{thm:multi item concave value convex budget pure}.

\begin{proof}[Proof of \Cref{thm:multi item concave value convex budget pure}]
    Fix an arbitrary Nash equilibrium $\eqlb$.
    Suppose $\allocs,\prices$ are the allocation and per-unit price in the induced FPPE. 
    Let  
    $\mathbf\optalloc$ be the allocation in the optimal transferable welfare.
    We introduce the following partition $A_1\bigsqcup A_2\bigsqcup A_3$
    of agents based on $\allocs$, $\prices$, and $\mathbf\optalloc$:
    \begin{align*}
        A_1 &\triangleq 
        \left\{i\in[n]: \sum_{j\in[m]}\pricej\allocij = \truewealth_i\right\}
        \\
        A_2 &\triangleq
        \left\{i\in[n]: i \not\in A_1
        \land 
        \sum_{j\in[m]} \ctrij\optalloc_{ij} \leq 
        \sum_{j\in[m]} \ctrij\allocij
        \right\}
        \\
        A_3 &\triangleq
        \left\{i\in[n]: i \not\in A_1
        \land 
        \sum_{j\in[m]} \ctrij\optalloc_{ij} > 
        \sum_{j\in[m]} \ctrij\allocij
        \right\}
    \end{align*}
    In words, $A_1$ corresponds to every agent $i$ who exhausts her true budget $\truewealth_i$ in the equilibrium;
    and $A_2$, $A_3$ correspond to the remaining agents.
% 
    % For every agent $i\in A_4$, her allocation $\alloc_i$
    % is the equilibrium is at least 
    % \begin{align*}
    %     \alloci 
    %     % \overset{(a)}{\geq}
    %     % 1 - \frac{\price}{\valuefuncderivative_i(\alloci)}
    %     \overset{(a)}{\geq} 
    %     1 - \frac{\price}{\valuefuncderivative_i(\alloc_i)}
    %     \moneycostderivative_i(\price\alloci)
    %     \overset{(b)}{\geq}
    %     1 - \frac{1}{\pricethreshold}
    %     = 
    %     \frac{\pricethreshold - 1}{\pricethreshold}
    % \end{align*}
    % where inequality~(a) is guaranteed due to \Cref{lem:alloc lower bound single item concave value hard budget};
    % % inequality~(b) holds since $\optalloc_i > \alloci$
    % % and the concavity of valuation function $\valuefunc_i$;
    % and inequality~(b) is guaranteed since $\valuefuncderivative_i(\alloc_i) > \pricethreshold\cdot \price\moneycostderivative_i(\price\alloci)$.
% 
    Next, we compare the transferable welfare contribution from $A_1, A_2, A_3$ separately.

    \smallskip
    For every agent $i\in A_1$, note that 
    \begin{align*}
        \wtp_i(\optalloc_i) 
        \overset{(a)}{\leq} \truewealth_i
        \overset{(b)}{=}
        \wtp_i(\alloci)
    \end{align*}
    where the inequality holds due to the definition of $\wtp_i$;
    and the equality holds due to the definition of $A_1$.
    
    For every agent $i\in A_2$, note that 
    \begin{align*}
        \wtp_i(\optalloc_i) \leq \wtp_i(\alloci)
    \end{align*}
    where the inequality holds since 
    $\sum_{j\in[m]} \ctrij\optalloc_{ij} \leq 
        \sum_{j\in[m]} \ctrij\allocij$
        implied by the definition of $A_2$.

    For every agent $i\in A_3$, 
    let $\purchaseseti \triangleq \{j\in[m]:\allocij > 0\}$
    be the subset of items allocated to agent $i$,
    and $\Delta \triangleq \frac{\sum_{j\in \purchaseseti}\price_j}{\sum_{j\in \purchaseseti}\ctrij}$.
Due to the definition of FPPE, 
$\frac{\price_j}{\ctrij} \geq \Delta$ for every item $j\in[m]$,
and it becomes equality when $j\in \purchaseseti$.
    Note that 
    \begin{align*}
        \wtp_i(\optalloc_i) 
        &\overset{(a)}{\leq} 
        \wtp_i(\alloci) + 
        \frac{
        \valuefunc_i\left(\sum_{j\in[m]} \ctrij\optalloc_{ij}  
        \right) - 
        \valuefunc_i\left(
        \sum_{j\in[m]} \ctrij\allocij
        \right)
        }{
        \moneycostderivative_i(\wtp_i(\alloci))
        }
        \\
        &\overset{(b)}{\leq} 
         \wtp_i(\alloci) + 
        \frac{
        \valuefunc_i\left(\sum_{j\in[m]} \ctrij\optalloc_{ij}  
        \right) - 
        \valuefunc_i\left(
        \sum_{j\in[m]} \ctrij\allocij
        \right)
        }{
        \moneycostderivative_i\left(
        \sum_{j\in[m]} \pricej\allocij\right)
        }
        \\
        &\overset{(c)}{\leq} 
         \wtp_i(\alloci) 
         + 
         \left(
         \sum_{j\in[m]} (\optalloc_{ij} -\allocij)\ctrij
         \right)
         \cdot \frac{
        \valuefuncderivative_i\left(
        \sum_{j\in[m]} \ctrij\allocij
        \right)
         }{
        \moneycostderivative_i\left(
        \sum_{j\in[m]} \pricej\allocij\right)
         }
         \\
        &\overset{(d)}{\leq}
        \wtp_i(\alloci) + 
       \left(
         \sum_{j\in[m]} (\optalloc_{ij} -\allocij)\ctrij
         \right)
         \cdot 
    \frac{\sum_{j\in \purchaseseti}\price_j}{\sum_{j\in \purchaseseti}(1-\allocij)\ctrij}
    \\
        &\overset{(e)}{\leq}
        \wtp_i(\alloci) + 
       \left(
         \sum_{j\in[m]} \optalloc_{ij}\ctrij
         \right)
         \cdot 
    \frac{\sum_{j\in \purchaseseti}\price_j}{\sum_{j\in \purchaseseti}\ctrij}
    \\
        &\overset{(g)}{=}
        \wtp_i(\alloci) + 
       \left(
         \sum_{j\in[m]} \optalloc_{ij}\ctrij
         \right)
         \cdot \Delta
        \\
        &\overset{(f)}{\leq}
        \wtp_i(\alloci) + 
        \sum_{j\in[m]} \optalloc_{ij}\pricej
    \end{align*}
    where inequality~(a) holds due to the definition of $\wtp_i$ and the convexity of $\moneycost_i$;
    inequality~(b) holds since 
    $\moneycostderivative_i$ is weakly increasing implied by
    the convexity of 
    $\moneycost_i$,
    and 
    $\wtp_i(\alloci) \geq \sum_{j\in[m]}\pricej\allocij$ which is implied by the definition of $\wtp_i$ and 
    the fact that 
    agent $i$'s utility is non-negative in the equilibrium allocation $\allocs$ and per-unit prices $\prices$;
    inequality~(c) holds due to the concavity of valuation function $\valuefunc_i$;
    inequality~(d) holds due to \Cref{lem:budget lower bound multi item concave value hard budget};
    and inequality~(e) holds 
    since $\frac{\sum_{j\in[m](\optalloc_{ij}-\allocij)\ctrij}}{\sum_{j\in[m]}(1-\allocij)\ctrij} 
    \leq \frac{\sum_{j\in[m]\optalloc_{ij}\ctrij}}{\sum_{j\in[m]}\ctrij}$ 
    by algebra;
    equality~(f) holds by the definition of $\Delta$;
    and inequality~(g) holds since
    $\frac{\price_j}{\ctrij} \geq \Delta$ for every item $j\in[m]$.

    \smallskip
    Putting all pieces together, we have the following upper bound of
    the optimal transferable welfare $\wtp(\mathbf\optalloc)$,
    \begin{align*}
    % \label{eq:welfare upper bound single item concave value hard budget}
    \begin{split}
        \wtp(\mathbf\optalloc) 
        &= 
        \sum_{i\in[n]} \wtp_i(\optalloc_i)
        % \\
        \leq \sum_{i\in A_3}\sum_{j\in[m]} \optalloc_{ij}\pricej
        +
        \sum_{i\in A_1\sqcup A_2 \sqcup A_3}
        \wtp_i(\alloci)
        \\
        &
        \overset{(a)}{\leq} 
        \sum_{j\in[m]}\pricej
        +
        \sum_{i\in A_1\sqcup A_2 \sqcup A_3}
        \wtp_i(\alloci)
        % \\
        \overset{(b)}{\leq} 
        2\wtp(\allocs)
        \end{split}
    \end{align*}
    where inequality~(a) holds since $\sum_{i\in A_3}\optalloc_{ij} \leq 1$
    for every item $j\in[m]$;
    and inequality~(b) holds since 
    $\sum_{j\in[m]}\pricej \leq \wtp(\allocs)$
    since all agents receive non-negative utility in the equilibrium allocation $\allocs$ and per-unit prices $\prices$.
\end{proof}

\subsection{A $4$-approximation Analysis for Mixed Nash}

In this subsection, we present a $4$-approximation PoA (\Cref{thm:multi item concave value convex budget mixed})
for mixed Nash.
% The analysis is inspired by \citet{CST-15b}.

\begin{theorem}
\label{thm:multi item concave value convex budget mixed}
    In the multi-item environment,
    for agents with (differentiable) {concave} valuation functions 
 $\{\valuefunc_i\}$ and 
 (differentiable) convex disutilities of money $\{\moneycost_i\}$
 up to heterogeneous budgets $\{\truewealth_i\}$,
    the mixed Nash PoA of transferable welfare 
    is at most $4$.
\end{theorem}

% \newcommand{\tildePj}{\tildeP_j}
% \newcommand{\optallocij}{\optalloc_{ij}}

\begin{proof}
   Fix an arbitrary mixed Nash equilibrium $\eqlb$.
    Suppose $\allocs,\prices$ are the randomized allocation and per-unit prices in the induced FPPE. 
    Let  
    $\mathbf\optalloc$ be the allocation in the optimal transferable welfare.    

    For each agent $i$, we present the following upper bound 
    of its contribution $\wtp_i(\optalloc_i)$ in the optimal transferable welfare allocation,
    \begin{align}
    \label{eq:multi item mixed wtp bound}
        \frac{1}{2}\wtp_i(\optalloc_i) \leq 
        \moneycost_i^{-1}(\util_i) + 
        \sum_{j\in[m]}\optalloc_{ij} \expect{\pricej}
    \end{align}
    where $\util_i$ is the expected utility of agent $i$ in the equilibrium $\eqlb$.
    Note that inequality~\eqref{eq:multi item mixed wtp bound}
    immediately implies the lemma statement since
    \begin{align*}
        \wtp(\mathbf\optalloc) 
        = \sum_{i\in[n]}
        \wtp_i(\optalloc_i)
        \leq 
        2
        \left(
        \sum_{i\in[n]} 
        \moneycost_i^{-1}(\util_i)
        +
        \optalloc_i \expect{\price}
        \right)
        \leq 
        4\wtp(\allocs)
    \end{align*}
    where the last inequality holds since $\moneycost_i^{-1}(\util_i) \leq 
    \moneycost_i^{-1}
    \left(
    \expect{\val_i
    \left(
    \sum_{j\in[m]}\allocij\ctrij
    \right)
    }
    \right)
    \equiv
    \wtp_i(\alloci)$;
    $\sum_{j\in[m]}\expect{\pricej} \leq  \wtp(\allocs)$;
    and $\sum_{i\in[n]}\optalloc_{ij} = 1$
    for every item $j\in[m]$.

    \smallskip
    Below we proof inequality~\eqref{eq:single item mixed wtp bound}
    by considering a specific deviation strategy for agent $i$.
    Let $\prices\doubleprimed$ be the randomized per-unit prices induced by the FPPE where agent $i$ is not participated, or equivalently, reporting $\wealth_i\doubleprimed = 0$.
    As a sanity check randomized price $\pricej\doubleprimed$ is first order stochastically dominated by randomized price $\pricej$ for every item $j\in[m]$.
    
    Let $\tildePj\doubleprimed \triangleq \expect{\pricej\doubleprimed}$
    for every item $j\in[m]$.
    Now consider the following deviating strategy for agent $i$
    where agent $i$ deterministically reports 
    \begin{align*}
        \val_i\primed = \infty,\quad 
        \wealth_i\primed = 
        \sum_{j\in[m]}
        \optalloc_{ij}  
        \tildePj\doubleprimed
    \end{align*}
    Let $\allocs\primed,\prices\primed$ be the randomized allocation and per-unit prices in the induced FPPE after this deviation of agent $i$.
    Since agent $i$ reports $\val_i\primed = \infty$, 
    she always exhausts her reported budget$~\wealth_i\primed$.
    
    In the remaining analysis,
    we couple the report profiles of all other agents except agent~$i$ in the FPPE inducing randomized per-unit prices $\prices\doubleprimed$, and the FPPE inducing randomized 
    allocation~$\allocs\primed$ and per-unit prices $\prices\primed$.
    As a sanity check, 
    it is straightforward to verify that 
    \begin{align*}
        \pricej\doubleprimed \leq \pricej\primed
        \text{ for every $j\in[m]$, and }
        \sum_{j\in[m]}\pricej\primed \leq 
        \sum_{j\in[m]}\pricej\doubleprimed + \wealth_i\primed
    \end{align*}
    for every realization of agents' reports.
    % Let $\tildePj\primed = \expect{\pricej\primed}$.
    % By definition, $\sum_{j\in[m]}\tildePj\primed - \tildePj\doubleprimed\leq \wealth\primed$.

    Define auxiliary random variable 
    $\gamma \triangleq 
    \frac{\wealth_i\primed}
    {\sum_{j\in[m]}
    \optallocij\pricej\doubleprimed} \geq 0$.
    By definition, $\expect{\frac{1}{\gamma}} = 1$.
    The expected utility $\util_i$
    of agent $i$ is at least her expected utility under this deviation,
    i.e., 
    \begin{align*}
        \util_i 
        &\overset{(a)}{\geq} 
        \expect
        [\prices\primed]
        {
        \valuefunc_i\left(
        \left(
        \max_{j\in[m]}
        \frac{\ctrij}{\pricej\primed}
        \right)
        \wealth_i\primed
        \right)
        -
        \moneycost_i\left(\wealth_i\primed\right)}
        \\
        &\overset{(b)}{\geq} 
        \expect
        [\prices\primed]
        {
        \valuefunc_i\left(
        \left(
        \max_{j\in[m]}
        \frac{\ctrij}{\pricej\primed}
        \right)
        \left(
        \sum_{j\in[m]}
        \frac{1}{\gamma + 1}
        \gamma\optallocij\pricej\doubleprimed
        +
        \frac{\gamma}{\gamma+1}
        \left(\pricej\primed - \pricej\doubleprimed\right)
        \right)
        \right)}
        -
        \moneycost_i\left(
        \sum_{j\in[m]}
        \optalloc_{ij}  
        \tildePj\doubleprimed
        \right)
        \\
        &\overset{(c)}{\geq} 
        \expect
        [\prices\primed]
        {
        \valuefunc_i\left(
        \left(
        \max_{j\in[m]}
        \frac{\ctrij}{\pricej\primed}
        \right)
        \left(
        \sum_{j\in[m]}
        \frac{\gamma}{\gamma + 1}
        \optallocij
        \pricej\primed
        \right)
        \right)}
        -
        \moneycost_i\left(
        \sum_{j\in[m]}
        \optalloc_{ij}  
        \tildePj\doubleprimed
        \right)
        \\
        &\overset{(d)}{\geq} 
        \expect
        [\prices\primed]
        {
        \valuefunc_i\left(
        \sum_{j\in[m]}
        \frac{\gamma}{\gamma + 1}
        \frac{\ctrij}{\pricej\primed}
        \optallocij
        \pricej\primed
        \right)}
        -
        \moneycost_i\left(
        \sum_{j\in[m]}
        \optalloc_{ij}  
        \tildePj\doubleprimed\right)
        \\
        &\overset{(e)}{\geq} 
        \expect
        [\gamma]
        {
        \frac{\gamma}{\gamma + 1}
        \valuefunc_i\left(
        \sum_{j\in[m]}
        {\ctrij}
        \optallocij
        \right)}
        -
        \moneycost_i\left(
        \sum_{j\in[m]}
        \optalloc_{ij}  
        \tildePj\doubleprimed\right)
        \\
        &\overset{(f)}{\geq} 
        {
        \frac{1}
        {\expect{\frac{1}{\gamma}}
        +1 }
        \valuefunc_i\left(
        \sum_{j\in[m]}
        {\ctrij}
        \optallocij
        \right)}
        -
        \moneycost_i\left(
        \sum_{j\in[m]}
        \optalloc_{ij}  
        \tildePj\doubleprimed\right)
        \\
        &\overset{(g)}{=} 
        \frac{1}{2}
        \valuefunc_i\left(
        \sum_{j\in[m]}
        {\ctrij}
        \optallocij
        \right)
        -
        \moneycost_i\left(
        \sum_{j\in[m]}
        \optalloc_{ij}  
        \tildePj\doubleprimed\right)
    \end{align*}
    where inequality~(a) holds due to the construction of FPPE;
    inequality~(b) holds since $\wealth_i\primed = \gamma\sum_{j\in[m]}\optallocij\pricej\doubleprimed$
    and $\wealth_i\primed \geq \sum_{j\in[m]}\pricej\primed - \pricej\doubleprimed$ for every realization of 
    $\pricej\primed,\pricej\doubleprimed,\gamma$;
     inequality~(c) holds since $\optallocij \leq 1$;
     inequality~(d) holds by algebra;
     {inequality~(e) holds due to the concavity of 
     valuation function $\valuefunc_i$ and $\valuefunc_i(0) = 0$};
     inequality~(f) holds due to Jensen's inequality;
     and equality~(g) holds since $\expect{\frac{1}{\gamma}} = 1$
     by definition.

    Finally, applying concave function 
    $\moneycost_i^{-1}$ 
    to both side,
        we obtain
    \begin{align*}
        \frac{1}{2}\wtp_i(\optalloc_i) 
        &\leq 
        \moneycost_i^{-1}\left(
        \frac{1}{2}
        \valuefunc_i\left(
        \sum_{j\in[m]}
        {\ctrij}
        \optallocij
        \right)
        \right)
        \leq 
        \moneycost_i^{-1}\left(
        \util_i + 
        \moneycost_i\left(\sum_{j\in[m]}
        \optalloc_{ij}  
        \tildePj\doubleprimed\right)
        \right)
        \\
        &\leq 
        \moneycost_i^{-1}\left(
        \util_i  \right)
        +
        \sum_{j\in[m]}
        \optalloc_{ij}  
        \tildePj\doubleprimed
        \leq 
        \moneycost_i^{-1}\left(
        \util_i  \right)
        +
        \sum_{j\in[m]}
        \optalloc_{ij}  
        \expect{\pricej}
    \end{align*}
    where the first and third inequality hold
    due to the convexity of $\moneycost_i$;
    the second inequality holds due to the monotonicity of $\moneycost_i$;
    and the last inequality holds since $\pricej$
    first order stochastically dominates $\pricej\doubleprimed$ and thus $\expect{\pricej}
    \geq \expect{\pricej\doubleprimed} \equiv \tildePj\doubleprimed$
    for every item $j\in[m]$.
\end{proof}


==> Notes/multi-item-poa.tex <==




\section{Metagame with Multiple Items and Non-quasilinear Agents}
\label{sec:metagame fpa}

There are $m$ divisible items (aka impressions) 
and $n$ agents (aka advertisers).
Each agent $i$ has valuation profile $\vali = (\val_{i1}, \dots, \val_{im})$
where $\valij$ is the value for item $j$.
Each agent $i$ also has an outside option value for money, described by a function $\moneycost_i: \reals_+ \rightarrow \reals_+\cup\{\infty\}$, which is strictly increasing and weakly convex. 
For ease of presentation, we assume that $\moneycost_i$
is differentiable, and write
 $\moneycostderivative_i(\price_i)$ for the derivative of
 $\moneycost_i$ at $\price_i$.
 Without loss of generality, we assume that $\moneycostderivative_i(0) = 1$ for every agent $i$.
Given allocation profile $\alloci = (\alloc_{i1}, \dots, \alloc_{im})$ and payment $\price_i$,
agent $i$ has utility $
    \util_i(\alloc_i, \price_i) = 
    % \val_i(\alloc) -
    \sum_{j}\valij \cdot \allocij -
    \moneycost_i(\price_i)$.\footnote{This model is 
    similar to the model considered in \citet{BCHNL-21}.}

    
\paragraph{Transferable welfare.}
Given allocation profile $\allocbf = (\alloc_1, \dots, \alloc_n)$, the \emph{transferable welfare}
is $\twelfare(\allocbf) = \sum_i \wtp_i(\alloc_i)$
where $\wtp_i(\alloc_i) = \moneycost^{-1}(\sum_j\valij\cdot\allocij)$ 
is agent $i$'s \emph{willingness to pay} for allocation $\alloc_i$.
Recall that $\moneycost_i$ is convex and its derivative
$\moneycostderivative_i(0) = 1$.
Hence, $\wtp_i(\alloc_i) \leq \val_i \cdot \alloc_i$
and thus transferable welfare is upperbounded by welfare.

\paragraph{Metagame.}

All agents compete 
in the first-price pacing game. 
In particular, 
each agent reports a hard budget $\wealth_i$ and 
the seller implements the allocation and payment profile 
induced by the first-price pacing equilibrium \citep{CKPSSSW-22}
assuming each agent $i$ has valuation profile $\val_i$ and budget $\wealth_i$.
In this section, we focus in the \emph{pure} Nash equilibrium of reported budget profile $(\wealth_1,\dots,\wealth_n)$.

\begin{definition}[\citealp{CKPSSSW-22}]
A set of \emph{budget-feasible first price pacing multiplier (BFPM)}
is a tuple $(\pacescalar, \allocs)$ of pacing multipliers $\pacescalar_i\in[0,1]$
for each agent $i$, and fractional allocation $\allocij\in[0,1]$ for each 
agent $i$ and item $j$, that satisfies the following properties
\begin{itemize}
    \item (Price) Per-unit price $\price_j = \max_{i} \pacescalar_i \valij$
    \item (Highest bid wins) 
    If $\allocij > 0$, then $\pacescalar_i \valij = \price_j$
    \item (Budget feasible) $\sum_j \allocij\price_j \leq \wealth_i$
    \item (Demanded goods sold completely)
    If $\price_j > 0$, then $\sum_{i}\alloc_{ij} = 1$
    \item (No overselling) $\sum_{i}\alloc_{ij}  \leq 1$ for each item $j$
    \end{itemize}
    A 
\emph{first price pacing equilibrium (FPPE)} 
is a BFPM which additionally satisfies
    \begin{itemize}
    \item (No unnecessary pacing) If $\sum_{j}\alloc_{ij}\price_j < \wealth_i$,
    then $\pacescalar_i = 1$.
\end{itemize}
\end{definition}

\begin{lemma}[\citealp{CKPSSSW-22}]
\label{lem:fppe existence}
For any problem instance, an FPPE
is guaranteed to exist and is essentially unique (i.e., the pacing multipliers are unique).
Furthermore, FPPEs Pareto-dominate all BFPMs (in pacing multipliers, per-unit prices, revenue).
\end{lemma}

\begin{lemma}[\citealp{CKPSSSW-22}]
\label{lem:fppe adding item}
\label{lem:fppe adding agent}
    In an FPPE, adding an item (agent) weakly increases revenue.
\end{lemma}

\begin{lemma}
\label{lem:fppe increasing budget}
\label{lem:fppe change budget}
In an FPPE, increasing an arbitrary agent $i$'s budget from $\wealth_i$
to $\wealth_i\primed$,
the per-unit price $\price_j$ for every item $j$ weakly increases.
Moreover, the increment of the revenue is at most $\wealth_i\primed$.
\end{lemma}
\begin{proof}
    Let $(\pacescalar, \allocs)$/$(\pacescalar\primed, \allocs\primed)$ 
    be the FPPE before/after
    agent $i$'s budget increasing.
    Let $\prices$/$\prices\primed$
    be their induced per-unit prices respectively.
    It can be verified that $(\pacescalar, \allocs)$
    is still a valid BFPM after budget increasing.
    By \Cref{lem:fppe existence}, $\pacescalar\primed_\ell\geq \pacescalar_\ell$
    for every agent $\ell$,
    and thus per-unit price $\price_j\primed \geq \price_j$ for every item $j$.

    Now consider an instance $\instance\doubleprimed$ where we exclude agent $i$
    while holding all other parameters fixed.
    By \Cref{lem:fppe adding agent},
    the revenue of FPPE in this instance $\instance\doubleprimed$ 
    is at most 
    the revenue of FPPE in the original instance where agent $i$ has budget $\wealth_i$,
    i.e., at most $\sum_j \price_j$.
    It is sufficient to show the revenue of FPPE in $\instance\doubleprimed$ is 
    at least $\sum_j \price_j\primed - \wealth_i\primed$.
    To see this, consider the following pacing multipliers $\pacescalar\doubleprimed\triangleq \pacescalar\primed_{-i}$ and 
    allocations $\allocs\doubleprimed \triangleq \allocs\primed_{-i}$.
    The tuple $(\pacescalar\doubleprimed, \allocs\doubleprimed)$ satisfies all
    constraints of BFPM for instance $\instance\doubleprimed$ except 
    (demand goods sold completely).
    Note that we can further decompose every items into smaller pieces and discard 
    pieces with no allocation under $\allocs\doubleprimed$.
    In this way, $(\pacescalar\doubleprimed, \allocs\doubleprimed)$ becomes a valid
    BFPM after removing those (fractional) items,
    and its revenue is at least $\sum_j \price_j\primed - \wealth_i\primed$.
    Invoking \Cref{lem:fppe existence} and \Cref{lem:fppe adding item} finishes the proof.
\end{proof}


\subsection{Market Clearing Allocations for Non-quasilinear Agents}
As a key intermediate step for PoA analysis in the metagame, 
we first consider the market clearing prices / allocations and 
present two lemmas to characterize its transferable welfare.



\begin{definition}
    For non-quasilinear agents,
    the \emph{market clearing price $\marketclearings$} and 
    \emph{market clearing allocation ${\marketclearingallocs}$}
    satisfies
    \begin{itemize}
        \item for every agent $i$, 
        % his market clearing allocation profile $\marketclearingalloc_i$
        % satisfies
        $\marketclearingalloc_{i} 
        \in \argmax_{\alloci\geq 0} 
        \sum_j \valij\cdot \allocij - 
        \moneycost_i\left(\sum_j   \marketclearing_j\cdot \allocij\right)
        $
        \item for each agent $i$ and each item $j$, $0\leq \marketclearingalloc_{ij} \leq 1$
        \item for each item $j$, $\sum_i \marketclearingalloc_{ij} = 1$
    \end{itemize}
\end{definition}
\begin{lemma}
    For non-quasilinear agents,
    the market clearing price $\marketclearings$ exists and 
    is unique. 
\end{lemma}


% Given the \mcptext~$\mcps$
% and any \mcatext~$\mcas$,
% let $\mcr_i \triangleq 
% \moneycostderivative_i(\sum_j \mcp_j \cdot \mca_{ij})$
% for each agent $i$.

\begin{lemma}
\label{lem:mc foc}
    For non-quasilinear agents,
    the market clearing price $\marketclearings$
    and \mcatext~$\mcas$,
    for each agent $i$ and each item $j$,
    \begin{align*}
        \valij &\leq 
        \mcp_j\cdot \moneycostderivative_i(t)\quad 
        \forall t\in\left[0, \sum_{j}\mcp_j \cdot \mca_{ij}\right)
        \\
        \valij &\geq 
        \mcp_j\cdot \moneycostderivative_i(t)\quad 
        \forall t\in\left(\sum_{j}\mcp_j \cdot \mca_{ij},\infty\right)
    \end{align*}
    where the equality holds only if 
\end{lemma}
\begin{proof}
    This is the first order condition of $\marketclearingalloc_{i} 
        \in \argmax_{\alloci\geq 0} 
        \sum_j \valij\cdot \allocij - 
        \moneycost_i\left(\sum_j   \marketclearing_j\cdot \allocij\right)$.
\end{proof}

The following two lemmas characterizes the \twelfaretext\ in 
any
\mcatext~$\mcas$.

\begin{lemma}
\label{lem:mc 2 approx}
  For non-quasilinear agents,
the transferable welfare of any
    market clearing allocation ${\marketclearingallocs}$
    is a 2-approximation
of the optimal transferable welfare.
\end{lemma}
\begin{proof}
Let  
$\optalloc_i$ be the allocation for each 
agent $i$ in the optimal transferable welfare. Note that
\begin{align*}
    2\cdot 
    % \sum_{i\in[n]}
    \wtp(\marketclearingallocs)
    -
    % \sum_{i\in[n]}
    \wtp(\mathbf{\optalloc})
    % \\
    \overset{(a)}{\geq}&
    \sum_{j\in[m]}\marketclearing_j
    + \sum_{i\in[n]}
    \wtp_i(\marketclearingalloc_i)
    -
    \sum_{i\in[n]}\wtp_i(\optalloc_i)
    \\
    \overset{(b)}{\geq}&
    \sum_{j\in[m]}\marketclearing_j
    -
    \sum_{i\in[n]}
    \frac{\plus{\sum_{j\in[m]}
    \valij\cdot \optalloc_{ij} - 
    \valij\cdot \mca_{ij}
    }
    }{
    \moneycostderivative^{-}\left(\sum_{j\in[m]}\valij\cdot\mca_{ij} \right)
    }
    \\
    \overset{(c)}{\geq}&
    \sum_{j\in[m]}\marketclearing_j
    -
    \sum_{i\in[n]}\sum_{j\in[m]}
    \frac{\valij\cdot \plus{
    \optalloc_{ij} -\mca_{ij}
    }
    }{
    \moneycostderivative^-\left(\sum_{j\in[m]}\mcp_j\cdot\mca_{ij} \right)
    }
    \\
    \overset{(d)}{\geq}&
    \sum_{j\in[m]}\marketclearing_j
    -
    \sum_{i\in[n]}\sum_{j\in[m]}
    \mcp_j\cdot \plus{
    \optalloc_{ij} -\mca_{ij}
    }
    \\
    \overset{}{\geq}& 
    ~0
\end{align*}
where
inequality~(a) uses the fact that transferable welfare $\sum_{i}\wtp_i(\marketclearingalloc_i)$ is lowerbounded by the revenue $\sum_{j\in[m]}\marketclearing_j$;
inequalities~(b) (c) use the 
definition of $\wtp_i$
and the
monotonicity of $\moneycostderivative_i$;
and inequality~(d) uses \Cref{lem:mc foc}.
\end{proof}

\begin{lemma}  
\label{lem:mc decompose}
  For non-quasilinear agents,
  for any \mcatext~$\mcas$,
  for each agent $i\in[n]$ 
  and any partition $\hitems\sqcup\litems \subseteq[m]$
  of items, 
  \begin{align*}
      \wtp_i(\mca_i) \leq 
      2\sum_{j\in \hitems}
      \mcp_j\cdot \mca_{ij}
      +
      \moneycost_i^{-1}\left(
      \sum_{j\in \litems}
      \valij\cdot \mca_{ij}
      \right)
  \end{align*}
\end{lemma}
\begin{proof}
    By definition,
    \begin{align*}
         \wtp_i(\mca_i) = 
         \moneycost_i^{-1}\left(
      \sum_{j\in[m]}
      \valij\cdot \mca_{ij}
      \right)
      \leq 
      \moneycost_i^{-1}\left(
      \sum_{j\in \hitems}
      \valij\cdot \mca_{ij}\right)
      +
      \moneycost_i^{-1}\left(
      \sum_{j\in \litems}
      \valij\cdot \mca_{ij}\right)
    \end{align*}
    where the inequality holds since $\hitems, \litems$
    is a partition of $[m]$ and $\moneycost_i$
    is convex and increasing.

    Let $\marketclearingwtp_i^{\hitems} \triangleq \moneycost_i^{-1}(
      \sum_{j\in \hitems}
      \valij\cdot \mca_{ij})$.
      Note that the lemma statement is satisfied trivially if $\marketclearingwtp_i^{\hitems} 
      \leq \sum_{j\in\hitems}\mcp_j\cdot \mca_{ij}$.
      Thus,
      from now on, we assume that 
      $\marketclearingwtp_i^{\hitems} > \sum_{j\in\hitems}\mcp_j\cdot \mca_{ij}$.
      By definition,
      \begin{align*}
      \displaystyle\int_0^{\marketclearingwtp_i^{\hitems}}
      \moneycostderivative_i(t)\,dt = 
      \sum_{j\in \hitems}
      \valij\cdot \mca_{ij}
      \end{align*}
      Below we lowerbound (upperbound) the left-hand (right-hand) side, respectively.
      Observe that 
      \begin{align*}
           \displaystyle\int_0^{\marketclearingwtp_i^{\hitems}}
      \moneycostderivative_i(t)\,dt
      \geq 
       \displaystyle\int_{\sum_{j\in\hitems}\mcp_j\cdot \mca_{ij}}^{\marketclearingwtp_i^{\hitems}}
      \moneycostderivative_i(t)\,dt
      \geq 
      \left(
      \marketclearingwtp_i^{\hitems}
      -
      \sum_{j\in\hitems}\mcp_j\cdot \mca_{ij}
      \right)
      \cdot
      \moneycostderivative_i^+\left(\sum_{j\in\hitems}\mcp_j\cdot \mca_{ij}\right)
      \end{align*}
      where the second inequality holds due to the monotonicity of $\moneycostderivative_i$.
      Furthermore, by \Cref{lem:mc foc},
      \begin{align*}
      \sum_{j\in \hitems}
      \valij\cdot \mca_{ij}
      \leq  
      \sum_{j\in\hitems}\mcp_j\cdot \mca_{ij}
      \cdot
      \moneycostderivative_i^-\left(\sum_{j\in\hitems}\mcp_j\cdot \mca_{ij}\right)
      \end{align*}
      Combining both sides, we obtain
      \begin{align*}
          \marketclearingwtp_i^{\hitems} 
          \leq 
           2\sum_{j\in \hitems}
      \mcp_j\cdot \mca_{ij}
      \end{align*}
      as desired.
\end{proof}

\subsection{Price of Anarchy in the Metagame}

In this section, we analyze the PoA in the metagame.

\begin{theorem}
\label{thm:poa multi-item}
    For non-quasilinear agents 
    with differentiable
    $\{\moneycost_i\}_{i\in[n]}$, the
    PoA of transferable welfare 
    (over pure Nash) is at most
    $23.09$.
\end{theorem}
\begin{proof}
    Fix an arbitrary equilibrium $\eqlb = (\wealth_1, \dots, \wealth_n)$
    in the metagame.
    Denote $\prices$ and $\allocs$ by the per-unit price and allocation in the induced FPPE, respectively.
    Fix an arbitrary \mcatext~$\mcas$.
    By \Cref{lem:mc 2 approx},
    the \twelfaretext\ $\wtp(\mcas)$ 
    in \mcatext~$\mcas$
    is a 2-approximation to the optimal \twelfaretext.
    Thus, it is sufficient for us to upperbound  the \twelfaretext\ $\wtp(\mcas)$  
    in \mcatext~$\mcas$
    with the \twelfaretext\ $\wtp(\allocs)$ in equilibrium $\eqlb$.
    
    Let $\pricethreshold\in (0, 1)$ be a parameter which will be specified
    in the end of the proof.
    Consider the partition of $m$ items as follows,
    \begin{align*}
        \hitems \triangleq \{j\in[m]: \price_j \geq \pricethreshold\cdot \mcp_j\} \\
        \litems \triangleq \{j\in[m]: \price_j < \pricethreshold\cdot \mcp_j\}
    \end{align*}
    By \Cref{lem:mc decompose},
    the \twelfaretext\ in \mcatext~$\mcas$
    can be upperbounded as 
    \begin{align*}
    \wtp(\mcas) = 
      \sum_{i\in[n]}\wtp_i(\mca_i) \leq 
      \sum_{i\in[n]}
      \sum_{j\in \hitems}
      2\mcp_j\cdot \mca_{ij}
      +
      \sum_{i\in[n]}
      \moneycost_i^{-1}\left(
      \sum_{j\in \litems}
      \valij\cdot \mca_{ij}
      \right)
    \end{align*}
    Below we upperbound the first term with $\hitems$
    and the second term with $\litems$ separately.
    
    \smallskip
    First, we focus on $\hitems$.
    Note that 
    \begin{align}
    \label{eq:high items bound pure}
        \wtp(\allocs) 
        \overset{(a)}{\geq}
        \sum_{j\in[m]}\price_j
        \geq 
        \sum_{j\in\hitems}
        \left(
        \price_j
        \cdot
        \sum_{i\in[n]}
        \mca_{ij}
        \right)
        \overset{(b)}{\geq}
        \sum_{i\in[n]}
        \sum_{j\in\hitems}
        \pricethreshold\cdot \mcp_j
        \cdot \mca_{ij}
    \end{align}
    where inequality~(a) holds since the \twelfaretext\ is 
    lowerbounded by the revenue;
    and inequality~(b) holds 
    since $\price_j \geq \pricethreshold\cdot \mcp_j$ for each item $j\in \hitems$.

    \smallskip
    Next, we focus on $\litems$.
    Fix an arbitrary agent $i\in[n]$.
    We start with the following claim
    that the utility $\util_i(\alloci, \prices)$ of agent $i$
    in equilibrium $\eqlb$ can be lowerbounded as
    \begin{align}
    \label{eq:util lower bound pure}
        \util_i(\alloci, \prices)
        \geq
        \left(1-\sqrt{\pricethreshold}\right)^2 \cdot \sum_{j\in \litems}
        \valij\cdot \mca_{ij}
    \end{align}
    Note that inequality~\eqref{eq:util lower bound pure}
    immediately implies 
    \begin{align}
    \begin{split}
    \label{eq:low items bound pure}
        \wtp_i(\alloci)
        &\geq 
        \moneycost^{-1}_i(\util_i(\alloc_i, \prices)) \\
        &\geq 
        \moneycost^{-1}_i\left(
        \left(1-\sqrt{\pricethreshold}\right)^2 \cdot \sum_{j\in \litems}
        \valij\cdot \mca_{ij}\right) \\
        &\geq 
        \left(1-\sqrt{\pricethreshold}\right)^2 \cdot 
        \moneycost^{-1}_i\left(
        \sum_{j\in \litems}
        \valij\cdot \mca_{ij}
        \right)
        \end{split}
    \end{align}
    where the last inequality holds due to the convexity of $\moneycost_i$.

    Now we show inequality~\eqref{eq:util lower bound pure}.
    Let $\meaningfulitems_i = \{j\in\litems:\valij \geq \mcp_j\}$.
    Without loss of generality, 
    we assume that
    subset $\meaningfulitems_i$
    is not empty, i.e., $|\meaningfulitems_i| > 0$.
    % that there exists an item $j\in \litems$ such that 
    % $\valij \geq \mcp_j$.
    Otherwise, $\mca_{ij} = 0$ for all items $j\in \litems$ and inequality~\eqref{eq:util lower bound pure}
    holds trivially.
    Let $\budgetscalar = \sqrt{\pricethreshold} - \pricethreshold$.
    Suppose agent $i$ deviates from reporting budget $\wealth_i$
    to budget $\deviatewealth_i$
    defined as follows
    \begin{align*}
       \deviatewealth_i \triangleq \budgetscalar\cdot \sum_{j\in\meaningfulitems_i} \mcp_j\cdot \mca_{ij}
    \end{align*}
    Denote $\deviateprices$ and $\deviateallocs$ by the per-unit price and allocation 
    in the induced FPPE after agent $i$'s deviation.
    We first argue that there exists an item $k\in \meaningfulitems_i$
    such that $\deviateprice_k \leq (\pricethreshold + \budgetscalar)\cdot \mcp_k$.
    By \Cref{lem:fppe increasing budget}, 
    it holds trivially if $\deviatewealth_i \leq \wealth_i$.
    % by contradiction.
    If $\deviatewealth_i > \wealth_i$, note that 
    \begin{align*}
        \sum_{j\in\meaningfulitems_i}\deviateprice_j
        &=
        \sum_{j\in[m]}\deviateprice_j
        -
        \sum_{j\not\in\meaningfulitems_i}\deviateprice_j
        % \\
        % &
        \overset{(a)}{\leq}
        \sum_{j\in[m]}\price_j
        +
        \deviatewealth_i
        -
        \sum_{j\not\in\meaningfulitems_i}\deviateprice_j
        \overset{(b)}{\leq}
        \sum_{j\in\meaningfulitems_i}
        \price_j
        +
        \deviatewealth_i
        \overset{(c)}{\leq}
        \left(\pricethreshold + \budgetscalar\right)
        \cdot
        \sum_{j\in\meaningfulitems_i} \mcp_j
    \end{align*}
    where inequality~(a) holds due to \Cref{lem:fppe change budget};
    inequality~(b) holds due to \Cref{lem:fppe increasing budget};
    and inequality~(c) holds 
    due to the definition of $\meaningfulitems_i$ and $\deviatewealth_i$.
    Now
    we can lowerbound 
    $\sum_{j\in[m]}\valij\cdot \allocij\primed$
    as follows,
    \begin{align*}
    \sum_{j\in[m]}\valij\cdot \deviatealloc_{ij}
    &\overset{(a)}{\geq} 
    \left(\max_{\ell\in[m]}\frac{\val_{i\ell}}{\deviateprice_\ell}\right)
    \cdot 
    \sum_{j\in[m]}\deviateprice_j\cdot \deviatealloc_{ij}
    \geq
    \frac{\val_{ik}}{\deviateprice_k}
    \cdot 
    \sum_{j\in[m]}\deviateprice_j\cdot \deviatealloc_{ij}
    \\
    &\overset{(b)}{\geq} 
    \frac
    {
    \moneycostderivative_i^+\left(
    \sum_{j\in[m]}\mcp_j\cdot \mca_{ij}
    \right)
    \cdot \mcp_k
    }{
    (\pricethreshold + \budgetscalar)\cdot \mcp_k}
    \cdot 
    \sum_{j\in[m]}\deviateprice_j\cdot \deviatealloc_{ij}
    \overset{(c)}{=}
    \frac{\moneycostderivative_i^+\left(
    \sum_{j\in[m]}\mcp_j\cdot \mca_{ij}
    \right)
    }{
    \pricethreshold + \budgetscalar}
    \cdot \deviatewealth_i
    \\
    &\overset{(d)}{=}
    \frac{\budgetscalar}{\pricethreshold + \budgetscalar}
    \cdot 
    \sum_{j\in\meaningfulitems_i}
    \mcp_j\cdot \moneycostderivative_i^+\left(
    \sum_{j\in[m]}\mcp_j\cdot \mca_{ij}
    \right)
    \cdot \mca_{ij}
    \overset{(e)}{\geq}
    \frac{\budgetscalar}{\pricethreshold + \budgetscalar}
    \cdot 
    \sum_{j\in\meaningfulitems_i}
    \val_{ij} 
    \cdot \mca_{ij}
    \\
    &=
    \frac{\budgetscalar}{\pricethreshold + \budgetscalar}
    \cdot 
    \sum_{j\in\litems}
    \val_{ij} 
    \cdot \mca_{ij}
    \end{align*}
    where equality~(a) holds due to the definition of FPPE;
    inequalities~(b) (e) holds due to \Cref{lem:mc foc};
    equality~(c) holds due to the existence of item $k$;
    and
    equality~(d) holds due to the definition of $\deviatewealth_i$.
    Now we are ready to show inequality~\eqref{eq:util lower bound pure} as follows,
    \begin{align*}
        \util_i(\alloci, \prices)
        &\geq
        \util_i(\deviatealloc_i, \deviateprices)
        =
        \sum_{j\in[m]}\valij\cdot \deviatealloc_{ij}
        -
        \moneycost_i\left(\sum_{j\in[m]}\deviateprice_j\cdot \deviatealloc_{ij}\right)
        \\
        &\overset{(a)}{=}
        \sum_{j\in[m]}\valij\cdot \deviatealloc_{ij}
        -
        \moneycost_i\left(\deviatewealth_i\right)
        \geq 
        \frac{\budgetscalar}{\pricethreshold+\budgetscalar}\cdot \sum_{j\in\meaningfulitems_i} \valij\cdot \mca_{ij}
        -
        \moneycost_i\left(\budgetscalar\cdot \sum_{j\in\meaningfulitems_i} \mcp_j\cdot \mca_{ij}\right)
        \\
        &=
        \left(\frac{\budgetscalar}{\pricethreshold+\budgetscalar} - \budgetscalar\right)
        \cdot \sum_{j\in\meaningfulitems_i} \valij\cdot \mca_{ij}
        +
        \budgetscalar \cdot \sum_{j\in\meaningfulitems_i} \valij\cdot \mca_{ij}
        -
        \moneycost_i\left(\budgetscalar\cdot \sum_{j\in\meaningfulitems_i} \mcp_j\cdot \mca_{ij}\right)
        \\
        &\overset{(b)}{\geq}
        \left(\frac{\budgetscalar}{\pricethreshold+\budgetscalar} - \budgetscalar\right)
        \cdot \sum_{j\in\meaningfulitems_i} \valij\cdot \mca_{ij}
        +
        \budgetscalar \cdot 
        \left(\sum_{j\in\meaningfulitems_i} \valij\cdot \mca_{ij}
        -
        \moneycost_i\left(\sum_{j\in\meaningfulitems_i} \mcp_j\cdot \mca_{ij}\right)
        \right)
        \\
        &\geq 
        \left(\frac{\budgetscalar}{\pricethreshold+\budgetscalar} - \budgetscalar\right)
        \cdot \sum_{j\in\meaningfulitems_i} \valij\cdot \mca_{ij}
    \end{align*}
    where equality~(a) holds due to 
    the existence of item $k$;
    and inequality~(b) holds due to 
    the convexity of $\moneycost_i$.

    Combining inequalities~\eqref{eq:high items bound pure}
    and \eqref{eq:low items bound pure}, we have
    \begin{align*}
        \left(\frac{4}{\pricethreshold} + \frac{2}{\left(1-\sqrt{\pricethreshold}\right)^2}
        \right)
        \cdot \wtp(\allocs)
        \geq
      \sum_{i\in[n]}
      \sum_{j\in \hitems}
      4\mcp_j\cdot \mca_{ij}
      +
      \sum_{i\in[n]}
      2\moneycost_i^{-1}\left(
      \sum_{j\in \litems}
      2\valij\cdot \mca_{ij}
      \right)
      \geq 
      2\wtp(\mcas)
      \geq
      \wtp(\allocs^*)
    \end{align*}
    Finally, optimizing $\pricethreshold\approx 0.310814$ and
    thus $\frac{4}{\pricethreshold} + \frac{2}{\left(1-\sqrt{\pricethreshold}\right)^2}\approx 23.09$
    as desired.
\end{proof}

\subsection{An Alternative Proof of \Cref{thm:poa multi-item}}
\begin{proof}[Alternative proof of \Cref{thm:poa multi-item}]
    Fix an arbitrary equilibrium $\eqlb = (\wealth_1, \dots, \wealth_n)$
    in the metagame.
    Denote $\prices$ and $\allocs$ by the per-unit price and allocation in the induced FPPE, respectively.
    Fix an arbitrary \mcatext~$\mcas$.
    By \Cref{lem:mc 2 approx},
    the \twelfaretext\ $\wtp(\mcas)$ 
    in \mcatext~$\mcas$
    is a 2-approximation to the optimal \twelfaretext.
    Thus, it is sufficient for us to upperbound  the \twelfaretext\ $\wtp(\mcas)$  
    in \mcatext~$\mcas$
    with the \twelfaretext\ $\wtp(\allocs)$ in equilibrium $\eqlb$.
    
    Let $\pricethreshold\in (0, 1)$ be a parameter which will be specified
    in the end of the proof.
    Consider the partition of $m$ items as follows,
    \begin{align*}
        \hitems \triangleq \{j\in[m]: \price_j \geq \pricethreshold\cdot \mcp_j\} \\
        \litems \triangleq \{j\in[m]: \price_j < \pricethreshold\cdot \mcp_j\}
    \end{align*}
    By \Cref{lem:mc decompose},
    the \twelfaretext\ in \mcatext~$\mcas$
    can be upperbounded as 
    \begin{align*}
    \wtp(\mcas) = 
      \sum_{i\in[n]}\wtp_i(\mca_i) \leq 
      \sum_{i\in[n]}
      \sum_{j\in \hitems}
      2\mcp_j\cdot \mca_{ij}
      +
      \sum_{i\in[n]}
      \moneycost_i^{-1}\left(
      \sum_{j\in \litems}
      \valij\cdot \mca_{ij}
      \right)
    \end{align*}
    Below we upperbound the first term with $\hitems$
    and the second term with $\litems$ separately.
    
    \smallskip
    First, we focus on $\hitems$.
    Note that 
    \begin{align}
    \label{eq:high items bound}
        \wtp(\allocs) 
        \overset{(a)}{\geq}
        \sum_{j\in[m]}\price_j
        \geq 
        \sum_{j\in\hitems}
        \left(
        \price_j
        \cdot
        \sum_{i\in[n]}
        \mca_{ij}
        \right)
        \overset{(b)}{\geq}
        \sum_{i\in[n]}
        \sum_{j\in\hitems}
        \pricethreshold\cdot \mcp_j
        \cdot \mca_{ij}
    \end{align}
    where inequality~(a) holds since the \twelfaretext\ is 
    lowerbounded by the revenue;
    and inequality~(b) holds 
    since $\price_j \geq \pricethreshold\cdot \mcp_j$ for each item $j\in \hitems$.

    \smallskip
    Next, we focus on $\litems$.
    Fix an arbitrary agent $i\in[n]$.
    We start with the following claim
    that the utility $\util_i(\alloci, \prices)$ of agent $i$
    in equilibrium $\eqlb$ can be lowerbounded as
    \begin{align}
    \label{eq:util lower bound}
        \util_i(\alloci, \prices)
        \geq
        \left(1-\sqrt{\pricethreshold}\right)^2 \cdot \sum_{j\in \litems}
        \valij\cdot \mca_{ij}
    \end{align}
    Note that inequality~\eqref{eq:util lower bound}
    immediately implies 
    \begin{align}
    \begin{split}
    \label{eq:low items bound}
        \wtp_i(\alloci)
        &\geq 
        \moneycost^{-1}_i(\util_i(\alloc_i, \prices)) \\
        &\geq 
        \moneycost^{-1}_i\left(
        \left(1-\sqrt{\pricethreshold}\right)^2 \cdot \sum_{j\in \litems}
        \valij\cdot \mca_{ij}\right) \\
        &\geq 
        \left(1-\sqrt{\pricethreshold}\right)^2 \cdot 
        \moneycost^{-1}_i\left(
        \sum_{j\in \litems}
        \valij\cdot \mca_{ij}
        \right)
        \end{split}
    \end{align}
    where the last inequality holds due to the convexity of $\moneycost_i$.

\newcommand{\wealths}{\mathbf{\wealth}}

{\color{red}
    Now we show inequality~\eqref{eq:util lower bound}.
    First, consider a budget profile $\wealths'$
    where agent $i$ reports $\wealth_i' = 0$.
    Let $\prices'$ be the per-unit price in the 
    induced FPPE under $\wealths'$.
    Let $\litems' = \{j\in[m]: \price_j' < \pricethreshold\cdot \marketclearing_j\}$.
    By \Cref{lem:fppe increasing budget},
    $\price_j' \leq \price_j$ for every $j$,
    and thus $\litems \subseteq \litems'$.
    
    Let $\meaningfulitems_i = \{j\in\litems':\valij \geq \mcp_j\}$.
    Without loss of generality, 
    we assume that
    subset $\meaningfulitems_i$
    is not empty, i.e., $|\meaningfulitems_i| > 0$.
    % that there exists an item $j\in \litems$ such that 
    % $\valij \geq \mcp_j$.
    Otherwise, $\mca_{ij} = 0$ for all items $j\in \litems$ and inequality~\eqref{eq:util lower bound}
    holds trivially.
    Let $\budgetscalar = \sqrt{\pricethreshold} - \pricethreshold$.
    Suppose agent $i$ deviates from reporting budget $\wealth_i'=0$
    to budget $\deviatewealth_i$
    defined as follows
    \begin{align*}
       \deviatewealth_i \triangleq \budgetscalar\cdot \sum_{j\in\meaningfulitems_i} \mcp_j\cdot \mca_{ij}
    \end{align*}
    Denote $\deviateprices$ and $\deviateallocs$ by the per-unit price and allocation 
    in the induced FPPE after agent $i$'s deviation.
    We first argue that there exists an item $k\in \meaningfulitems_i$
    such that $\deviateprice_k \leq (\pricethreshold + \budgetscalar)\cdot \mcp_k$.
    % by contradiction.
    Note that 
    \begin{align*}
        \sum_{j\in\meaningfulitems_i}\deviateprice_j
        &=
        \sum_{j\in[m]}\deviateprice_j
        -
        \sum_{j\not\in\meaningfulitems_i}\deviateprice_j
        % \\
        % &
        \overset{(a)}{\leq}
        \sum_{j\in[m]}\price_j
        +
        \deviatewealth_i
        -
        \sum_{j\not\in\meaningfulitems_i}\deviateprice_j
        \overset{(b)}{\leq}
        \sum_{j\in\meaningfulitems_i}
        \price_j
        +
        \deviatewealth_i
        \overset{(c)}{\leq}
        \left(\pricethreshold + \budgetscalar\right)
        \cdot
        \sum_{j\in\meaningfulitems_i} \mcp_j
    \end{align*}
    where inequality~(a) holds due to \Cref{lem:fppe change budget};
    inequality~(b) holds due to \Cref{lem:fppe increasing budget};
    and inequality~(c) holds 
    due to the definition of $\meaningfulitems_i$ and $\deviatewealth_i$.
    Now
    we can lowerbound 
    $\sum_{j\in[m]}\valij\cdot \allocij\primed$
    as follows,
    \begin{align*}
    \sum_{j\in[m]}\valij\cdot \deviatealloc_{ij}
    &\overset{(a)}{\geq} 
    \left(\max_{\ell\in[m]}\frac{\val_{i\ell}}{\deviateprice_\ell}\right)
    \cdot 
    \sum_{j\in[m]}\deviateprice_j\cdot \deviatealloc_{ij}
    \geq
    \frac{\val_{ik}}{\deviateprice_k}
    \cdot 
    \sum_{j\in[m]}\deviateprice_j\cdot \deviatealloc_{ij}
    \\
    &\overset{(b)}{\geq} 
    \frac
    {
    \moneycostderivative_i^+\left(
    \sum_{j\in[m]}\mcp_j\cdot \mca_{ij}
    \right)
    \cdot \mcp_k
    }{
    (\pricethreshold + \budgetscalar)\cdot \mcp_k}
    \cdot 
    \sum_{j\in[m]}\deviateprice_j\cdot \deviatealloc_{ij}
    \overset{(c)}{=}
    \frac{\moneycostderivative_i^+\left(
    \sum_{j\in[m]}\mcp_j\cdot \mca_{ij}
    \right)
    }{
    \pricethreshold + \budgetscalar}
    \cdot \deviatewealth_i
    \\
    &\overset{(d)}{=}
    \frac{\budgetscalar}{\pricethreshold + \budgetscalar}
    \cdot 
    \sum_{j\in\meaningfulitems_i}
    \mcp_j\cdot \moneycostderivative_i^+\left(
    \sum_{j\in[m]}\mcp_j\cdot \mca_{ij}
    \right)
    \cdot \mca_{ij}
    \overset{(e)}{\geq}
    \frac{\budgetscalar}{\pricethreshold + \budgetscalar}
    \cdot 
    \sum_{j\in\meaningfulitems_i}
    \val_{ij} 
    \cdot \mca_{ij}
    \\
    &=
    \frac{\budgetscalar}{\pricethreshold + \budgetscalar}
    \cdot 
    \sum_{j\in\litems}
    \val_{ij} 
    \cdot \mca_{ij}
    \end{align*}
    where equality~(a) holds due to the definition of FPPE;
    inequalities~(b) (e) holds due to \Cref{lem:mc foc};
    equality~(c) holds due to the existence of item $k$;
    and
    equality~(d) holds due to the definition of $\deviatewealth_i$.
    Now we are ready to show inequality~\eqref{eq:util lower bound} as follows,
    \begin{align*}
        \util_i(\alloci, \prices)
        &\geq
        \util_i(\deviatealloc_i, \deviateprices)
        =
        \sum_{j\in[m]}\valij\cdot \deviatealloc_{ij}
        -
        \moneycost_i\left(\sum_{j\in[m]}\deviateprice_j\cdot \deviatealloc_{ij}\right)
        \\
        &\overset{(a)}{=}
        \sum_{j\in[m]}\valij\cdot \deviatealloc_{ij}
        -
        \moneycost_i\left(\deviatewealth_i\right)
        \geq 
        \frac{\budgetscalar}{\pricethreshold+\budgetscalar}\cdot \sum_{j\in\meaningfulitems_i} \valij\cdot \mca_{ij}
        -
        \moneycost_i\left(\budgetscalar\cdot \sum_{j\in\meaningfulitems_i} \mcp_j\cdot \mca_{ij}\right)
        \\
        &=
        \left(\frac{\budgetscalar}{\pricethreshold+\budgetscalar} - \budgetscalar\right)
        \cdot \sum_{j\in\meaningfulitems_i} \valij\cdot \mca_{ij}
        +
        \budgetscalar \cdot \sum_{j\in\meaningfulitems_i} \valij\cdot \mca_{ij}
        -
        \moneycost_i\left(\budgetscalar\cdot \sum_{j\in\meaningfulitems_i} \mcp_j\cdot \mca_{ij}\right)
        \\
        &\overset{(b)}{\geq}
        \left(\frac{\budgetscalar}{\pricethreshold+\budgetscalar} - \budgetscalar\right)
        \cdot \sum_{j\in\meaningfulitems_i} \valij\cdot \mca_{ij}
        +
        \budgetscalar \cdot 
        \left(\sum_{j\in\meaningfulitems_i} \valij\cdot \mca_{ij}
        -
        \moneycost_i\left(\sum_{j\in\meaningfulitems_i} \mcp_j\cdot \mca_{ij}\right)
        \right)
        \\
        &\geq 
        \left(\frac{\budgetscalar}{\pricethreshold+\budgetscalar} - \budgetscalar\right)
        \cdot \sum_{j\in\meaningfulitems_i} \valij\cdot \mca_{ij}
    \end{align*}
    where equality~(a) holds due to 
    the existence of item $k$;
    and inequality~(b) holds due to 
    the convexity of $\moneycost_i$.

    Combining inequalities~\eqref{eq:high items bound}
    and \eqref{eq:low items bound}, we have
    \begin{align*}
        \left(\frac{4}{\pricethreshold} + \frac{2}{\left(1-\sqrt{\pricethreshold}\right)^2}
        \right)
        \cdot \wtp(\allocs)
        \geq
      \sum_{i\in[n]}
      \sum_{j\in \hitems}
      4\mcp_j\cdot \mca_{ij}
      +
      \sum_{i\in[n]}
      2\moneycost_i^{-1}\left(
      \sum_{j\in \litems}
      2\valij\cdot \mca_{ij}
      \right)
      \geq 
      2\wtp(\mcas)
      \geq
      \wtp(\allocs^*)
    \end{align*}
    Finally, optimizing $\pricethreshold\approx 0.310814$ and
    thus $\frac{4}{\pricethreshold} + \frac{2}{\left(1-\sqrt{\pricethreshold}\right)^2}\approx 23.09$
    as desired.
    }
\end{proof}

\newpage

\subsection{Price of Anarchy over Mixed Nash}
\newcommand{\probthreshold}{\gamma}
\newcommand{\goodmeaningfulitems}{\hat{\meaningfulitems}}
\newcommand{\bpbthreshold}{\theta}
\newcommand{\CDF}{F}
\newcommand{\CDFHat}{\hat{\CDF}}

In this section, we analyze the PoA over mixed Nash
in the metagame.
\begin{theorem}
\label{thm:poa multi-item mixed nash}
    For non-quasilinear agents 
    with differentiable
    $\{\moneycost_i\}_{i\in[n]}$, the
    PoA of transferable welfare 
    (over mixed Nash) is at most
    $313.47$.
\end{theorem}
\begin{proof}
    Fix an arbitrary mixed equilibrium $\eqlb$
    in the metagame.
    Denote $\prices$ and $\allocs$ by the 
    randomized per-unit price and allocation in the induced FPPE, respectively.
    Note that $\prices$ and $\allocs$ could be correlated.
    Fix an arbitrary \mcatext~$\mcas$.
    By \Cref{lem:mc 2 approx},
    the \twelfaretext\ $\wtp(\mcas)$ 
    in \mcatext~$\mcas$
    is a 2-approximation to the optimal \twelfaretext.
    Thus, it is sufficient for us to upperbound  the \twelfaretext\ $\wtp(\mcas)$  
    in \mcatext~$\mcas$
    with the \twelfaretext\ $\wtp(\allocs)$ in mixed equilibrium $\eqlb$.
    
    Let $\pricethreshold=\frac{1}{4},\probthreshold=\frac{2}{27}$.
    Consider the partition of $m$ items as follows,
    \begin{align*}
        \hitems \triangleq \left\{j\in[m]: 
        \prob{\price_j \geq \pricethreshold\cdot \mcp_j\} \geq \probthreshold}
        \right\} \\
        \litems \triangleq \left\{j\in[m]: 
        \prob{\price_j \geq \pricethreshold\cdot \mcp_j\} \leq \probthreshold}
        \right\} 
    \end{align*}
    By \Cref{lem:mc decompose},
    the \twelfaretext\ in \mcatext~$\mcas$
    can be upperbounded as 
    \begin{align*}
    \wtp(\mcas) = 
      \sum_{i\in[n]}\wtp_i(\mca_i) \leq 
      \sum_{i\in[n]}
      \sum_{j\in \hitems}
      2\mcp_j\cdot \mca_{ij}
      +
      \sum_{i\in[n]}
      \moneycost_i^{-1}\left(
      \sum_{j\in \litems}
      \valij\cdot \mca_{ij}
      \right)
    \end{align*}
    Below we upperbound the first term with $\hitems$
    and the second term with $\litems$ separately.
    
    \smallskip
    First, we focus on $\hitems$.
    Note that 
    \begin{align}
    \label{eq:high items bound mixed nash}
        \wtp(\allocs) 
        \overset{(a)}{\geq}
        \expect{\sum_{j\in[m]}\price_j}
        \geq 
        \sum_{j\in\hitems}
        \left(
        \expect{\price_j}
        \cdot
        \sum_{i\in[n]}
        \mca_{ij}
        \right)
        \overset{(b)}{\geq}
        \sum_{i\in[n]}
        \sum_{j\in\hitems}
        \pricethreshold\probthreshold\cdot \mcp_j
        \cdot \mca_{ij}
    \end{align}
    where inequality~(a) holds since the \twelfaretext\ is 
    lowerbounded by the revenue;
    and inequality~(b) holds 
    since $\prob{\price_j \geq \pricethreshold\cdot \mcp_j}\geq \probthreshold$ 
    for each item $j\in \hitems$.

    \smallskip
    Next, we focus on $\litems$.
    Fix an arbitrary agent $i\in[n]$.
    We start with the following claim
    that the expected utility $\util_i(\alloci, \prices)$ of agent $i$
    in equilibrium $\eqlb$ can be lowerbounded as
    \begin{align}
    \label{eq:util lower bound mixed nash}
        \util_i(\alloci, \prices)
        \geq
        0.08208 \budgetscalar \cdot \sum_{j\in \litems}
        \valij\cdot \mca_{ij}
    \end{align}
    Note that inequality~\eqref{eq:util lower bound}
    immediately implies 
    \begin{align}
    \begin{split}
    \label{eq:low items bound mixed nash}
        \wtp_i(\alloci)
        &\geq 
        \moneycost^{-1}_i(\util_i(\alloc_i, \prices)) \\
        &\geq 
        \moneycost^{-1}_i\left(
        0.08208 \budgetscalar \cdot \sum_{j\in \litems}
        \valij\cdot \mca_{ij}\right) \\
        &\geq 
        0.08208 \budgetscalar \cdot 
        \moneycost^{-1}_i\left(
        \sum_{j\in \litems}
        \valij\cdot \mca_{ij}
        \right)
        \end{split}
    \end{align}
    where the last inequality holds due to the convexity of $\moneycost_i$.

    Now we show inequality~\eqref{eq:util lower bound}.
    Let $\meaningfulitems_i = \{j\in\litems:\valij \geq \mcp_j\}$.
    Without loss of generality, 
    we assume that
    subset $\meaningfulitems_i$
    is not empty, i.e., $|\meaningfulitems_i| > 0$.
    % that there exists an item $j\in \litems$ such that 
    % $\valij \geq \mcp_j$.
    Otherwise, $\mca_{ij} = 0$ for all items $j\in \litems$ and inequality~\eqref{eq:util lower bound}
    holds trivially.
    Let $\budgetscalar = \frac{1}{4}$.
    Suppose agent $i$ deviates from reporting 
    (possibly randomized) budget $\wealth_i$
    to deterministic budget $\deviatewealth_i$
    defined as follows
    \begin{align*}
       \deviatewealth_i \triangleq \budgetscalar\cdot \sum_{j\in\meaningfulitems_i} \mcp_j\cdot \mca_{ij}
    \end{align*}
    Denote $\deviateprices$ and $\deviateallocs$ by the (possibly) randomized correlated
    per-unit price and allocation 
    in the induced FPPE after agent $i$'s deviation.
    Define random subset $\goodmeaningfulitems_i \triangleq
    \{j\in \meaningfulitems: \price_j \leq \pricethreshold\cdot \mcp_j\}$.
    Denote $\event_i(\bpbthreshold)$
    as the event that 
    \begin{align*}
        \sum_{j\in \goodmeaningfulitems_i}\price_j + \deviatewealth_j \leq 
        \bpbthreshold\cdot \sum_{j\in\goodmeaningfulitems_i}\price_j
    \end{align*}
    and $\CDF_i(\bpbthreshold)$ as the probability of event $\event_i(\bpbthreshold)$.
    By \Cref{lem:prob bound}, 
    for every $\bpbthreshold \geq \pricethreshold$,
    we hav
    \begin{align*}
        \CDF_i(\bpbthreshold) \geq 
        1 - \frac{\pricethreshold(1-\probthreshold) + \bpbthreshold \probthreshold}{\bpbthreshold - \budgetscalar}
    \end{align*}
    Define $\eventHat_i(\bpbthreshold)$
    as the event that 
    \begin{align*}
        \exists k \in \goodmeaningfulitems_i
        \;\;\mbox{s.t.}\;\;
        \deviateprice_k \leq \bpbthreshold\cdot \mcp_k
    \end{align*}
    and $\CDFHat_i(\bpbthreshold)$
    as the probability of event $\eventHat_i(\bpbthreshold)$.
    We claim that event $\event_i(\bpbthreshold)$ implies $\eventHat_i(\bpbthreshold)$,
    and thus $\CDFHat_i(\bpbthreshold) \geq \CDF_i\bpbthreshold)$.
    To see this, we consider two cases separately.
    \begin{enumerate}
        \item For every realization of FPPE conditioning on $\wealth_i\geq\deviatewealth_i$
        and event $\event_i(\bpbthreshold)$, we have
        \begin{align*}
            \sum_{j\in\goodmeaningfulitems_i}\deviateprice_j
            \overset{(a)}{\leq}
            \sum_{j\in\goodmeaningfulitems_i}\price_j
            \leq 
        \sum_{j\in\goodmeaningfulitems_i}
        \price_j
        +
        \deviatewealth_i
            \overset{(b)}{\leq}
            \bpbthreshold\cdot \sum_{j\in\goodmeaningfulitems_i}\mcp_j
        \end{align*}
        where inequality~(a) holds due to \Cref{lem:fppe increasing budget};
        and inequality~(b) holds due to event $\eventHat_i(\bpbthreshold)$.
        Since all $\deviateprice_j$ are non-negative,
        event $\eventHat_i(\bpbthreshold)$
        happens.
        \item For every realization of FPPE conditioning on $\wealth_i\leq\deviatewealth_i$
        and event $\event_i(\bpbthreshold)$, we have
        \begin{align*}
            \sum_{j\in\goodmeaningfulitems_i}\deviateprice_j
        &=
        \sum_{j\in[m]}\deviateprice_j
        -
        \sum_{j\not\in\goodmeaningfulitems_i}\deviateprice_j
        \overset{(a)}{\leq}
        \sum_{j\in[m]}\price_j
        +
        \deviatewealth_i
        -
        \sum_{j\not\in\goodmeaningfulitems_i}\deviateprice_j
        \\
        &\overset{(b)}{\leq}
        \sum_{j\in\goodmeaningfulitems_i}
        \price_j
        +
        \deviatewealth_i
        \overset{(c)}{\leq}
            \bpbthreshold\cdot \sum_{j\in\goodmeaningfulitems_i}\mcp_j
        \end{align*}
    where inequality~(a) holds due to \Cref{lem:fppe change budget};
    inequality~(b) holds due to \Cref{lem:fppe increasing budget};
    and inequality~(c) holds 
    due to event $\event_i(\bpbthreshold)$.
        Since all $\deviateprice_j$ are non-negative,
        event $\eventHat_i(\bpbthreshold)$
        happens.
    \end{enumerate}
    For every $\bpbthreshold\in[0,\infty)$,
    for every realization of FPPE
    conditioning on event $\eventHat_i(\bpbthreshold)$,
    we can lowerbound 
    $\sum_{j\in[m]}\valij\cdot \allocij\primed$
    as follows,
    \begin{align}
    \begin{split}
    \label{eq:value lower bound mixed nash}
    \sum_{j\in[m]}\valij\cdot \deviatealloc_{ij}
    &\overset{(a)}{\geq} 
    \left(\max_{\ell\in[m]}\frac{\val_{i\ell}}{\deviateprice_\ell}\right)
    \cdot 
    \sum_{j\in[m]}\deviateprice_j\cdot \deviatealloc_{ij}
    \geq
    \frac{\val_{ik}}{\deviateprice_k}
    \cdot 
    \sum_{j\in[m]}\deviateprice_j\cdot \deviatealloc_{ij}
    \\
    &\overset{(b)}{\geq} 
    \frac
    {
    \moneycostderivative_i^+\left(
    \sum_{j\in[m]}\mcp_j\cdot \mca_{ij}
    \right)
    \cdot \mcp_k
    }{
    \bpbthreshold\cdot \mcp_k}
    \cdot 
    \sum_{j\in[m]}\deviateprice_j\cdot \deviatealloc_{ij}
    \\
    &\overset{}{=}
    \frac{1
    }{
    \bpbthreshold
    }
    \cdot \moneycostderivative_i^+\left(
    \sum_{j\in[m]}\mcp_j\cdot \mca_{ij}
    \right)
    \cdot 
    \sum_{j\in[m]}\deviateprice_j\cdot \deviatealloc_{ij}
    \end{split}
    \end{align}
    where equality~(a) holds due to the definition of FPPE;
    and inequality~(b) holds due to \Cref{lem:mc foc}
    and event $\eventHat_i(\bpbthreshold)$.
    % Furthermore, for every $\bpbthreshold\in[0, 1]$,
    % for every realization of FPPE conditioning on 
    % event $\eventHat_i(\bpbthreshold)$,
    % agent $i$ exhausts her budget, i.e., 
    % \begin{align*}
    % \sum_{j\in[m]}\deviateprice_j\cdot \deviatealloc_{ij}
    % = \deviatewealth_i
    % \end{align*}
    Now we are ready to show inequality~\eqref{eq:util lower bound mixed nash} as follows,
    \begin{align*}
        &~~~~\util_i(\alloci, \prices)
        \geq
        \util_i(\deviatealloc_i, \deviateprices)
        =
        \expect{\sum_{j\in[m]}\valij\cdot \deviatealloc_{ij}}
        -
        \moneycost_i\left(
        \expect{\sum_{j\in[m]}\deviateprice_j\cdot \deviatealloc_{ij}}\right)
        \\
        &\overset{(a)}{\geq} 
        \displaystyle
        \int_0^\infty
        \frac{1}{\bpbthreshold}
        \cdot 
        \moneycostderivative_i^+\left(
    \sum_{j\in[m]}\mcp_j\cdot \mca_{ij}
    \right)
    \cdot 
    \expect{
    \sum_{j\in[m]}\deviateprice_j\cdot \deviatealloc_{ij}
    \condition \eventHat_i(\bpbthreshold)}
    \,d\CDFHat_i(\bpbthreshold)
    \\
    &\qquad\qquad
    -
        \moneycost_i\left(
        \displaystyle
        \int_0^\infty
        \expect{\sum_{j\in[m]}\deviateprice_j\cdot \deviatealloc_{ij}
        \condition \eventHat_i(\bpbthreshold)
        }
        \,d\CDFHat_i(\bpbthreshold)
        \right)
        \\
&\overset{}{=} 
        \displaystyle
        \int_0^1
        \frac{1}{\bpbthreshold}
        \cdot 
        \moneycostderivative_i^+\left(
    \sum_{j\in[m]}\mcp_j\cdot \mca_{ij}
    \right)
    \cdot 
    \expect{
    \sum_{j\in[m]}\deviateprice_j\cdot \deviatealloc_{ij}
    \condition \eventHat_i(\bpbthreshold)}
    \,d\CDFHat_i(\bpbthreshold)
    \\
    &\qquad\qquad 
    + 
        \displaystyle
        \int_1^\infty
        \frac{1}{\bpbthreshold}
        \cdot 
        \moneycostderivative_i^+\left(
    \sum_{j\in[m]}\mcp_j\cdot \mca_{ij}
    \right)
    \cdot 
    \expect{
    \sum_{j\in[m]}\deviateprice_j\cdot \deviatealloc_{ij}
    \condition \eventHat_i(\bpbthreshold)}
    \,d\CDFHat_i(\bpbthreshold)
    \\
    &\qquad\qquad
    -
        \moneycost_i\left(
        \displaystyle
        \int_0^1
        \expect{\sum_{j\in[m]}\deviateprice_j\cdot \deviatealloc_{ij}
        \condition \eventHat_i(\bpbthreshold)
        }
        \,d\CDFHat_i(\bpbthreshold)
        +
        \displaystyle
        \int_1^\infty
        \expect{\sum_{j\in[m]}\deviateprice_j\cdot \deviatealloc_{ij}
        \condition \eventHat_i(\bpbthreshold)
        }
        \,d\CDFHat_i(\bpbthreshold)
        \right)
        \\
                &\overset{(b)}{=} 
        \displaystyle
        \int_0^1
        \frac{1}{\bpbthreshold}
        \cdot 
        \moneycostderivative_i^+\left(
    \sum_{j\in[m]}\mcp_j\cdot \mca_{ij}
    \right)
    \cdot 
    \deviatewealth_i
    \,d\CDFHat_i(\bpbthreshold)
    \\
    &\qquad\qquad 
    + 
        \displaystyle
        \int_1^\infty
        \frac{1}{\bpbthreshold}
        \cdot 
        \moneycostderivative_i^+\left(
    \sum_{j\in[m]}\mcp_j\cdot \mca_{ij}
    \right)
    \cdot 
    \expect{
    \sum_{j\in[m]}\deviateprice_j\cdot \deviatealloc_{ij}
    \condition \eventHat_i(\bpbthreshold)}
    \,d\CDFHat_i(\bpbthreshold)
    \\
    &\qquad\qquad
    -
        \moneycost_i\left(
        \displaystyle
        \int_0^1
        \deviatewealth_i
        \,d\CDFHat_i(\bpbthreshold)
        +
        \displaystyle
        \int_1^\infty
        \expect{\sum_{j\in[m]}\deviateprice_j\cdot \deviatealloc_{ij}
        \condition \eventHat_i(\bpbthreshold)
        }
        \,d\CDFHat_i(\bpbthreshold)
        \right)
        \\
&\overset{(c)}{\geq} 
        \displaystyle
        \int_0^1
        \frac{1}{\bpbthreshold}
        \cdot 
        \moneycostderivative_i^+\left(
    \sum_{j\in[m]}\mcp_j\cdot \mca_{ij}
    \right)
    \cdot 
    \deviatewealth_i
    \,d\CDFHat_i(\bpbthreshold)
    \\
    &\qquad\qquad 
    + 
        \displaystyle
        \int_1^\infty
        \frac{1}{\bpbthreshold}
        \cdot 
        \moneycostderivative_i^+\left(
    \sum_{j\in[m]}\mcp_j\cdot \mca_{ij}
    \right)
    \cdot 
    \deviatewealth_i
    \,d\CDFHat_i(\bpbthreshold)
    % \\
    % &\qquad\qquad
    -
        \moneycost_i\left(
        \displaystyle
        \int_0^1
        \deviatewealth_i
        \,d\CDFHat_i(\bpbthreshold)
        +
        \displaystyle
        \int_1^\infty
        \deviatewealth_i
        \,d\CDFHat_i(\bpbthreshold)
        \right)
        \\
&\overset{(d)}{=}
\displaystyle
        \int_0^\infty
        \frac{\budgetscalar}{\bpbthreshold}
        \cdot 
        \moneycostderivative_i^+\left(
    \sum_{j\in[m]}\mcp_j\cdot \mca_{ij}
    \right)
    \cdot 
    \sum_{j\in\meaningfulitems_i}\mcp_j\cdot \mca_{ij}
    \,d\CDFHat_i(\bpbthreshold)
    -
        \moneycost_i\left(
        \displaystyle
        \int_0^\infty
        \budgetscalar\cdot 
        \sum_{j\in\meaningfulitems_i}\mcp_j\cdot \mca_{ij}
        \,d\CDFHat_i(\bpbthreshold)
        \right)
        \\
&\overset{(e)}{\geq}
\displaystyle
        \int_0^\infty
        \frac{\budgetscalar}{\bpbthreshold}
        \cdot 
    \sum_{j\in\meaningfulitems_i}\valij\cdot \mca_{ij}
    \,d\CDFHat_i(\bpbthreshold)
    -
        \moneycost_i\left(
        \displaystyle
        \int_0^\infty
        \budgetscalar\cdot 
        \sum_{j\in\meaningfulitems_i}\mcp_j\cdot \mca_{ij}
        \,d\CDFHat_i(\bpbthreshold)
        \right)
        \\
&\overset{}{\geq}
\left(
\displaystyle
        \int_{\frac{\pricethreshold(1-\probthreshold)+\budgetscalar}{1-\probthreshold}}^\infty
        \frac{\budgetscalar}{\bpbthreshold}
        \,d\left(
         1 - \frac{\pricethreshold(1-\probthreshold) + \bpbthreshold \probthreshold}{\bpbthreshold - \budgetscalar}
        \right)
        \right)
        \cdot 
    \sum_{j\in\meaningfulitems_i}\valij\cdot \mca_{ij}
    -
        \moneycost_i\left(
        \displaystyle
        \budgetscalar\cdot 
        \sum_{j\in\meaningfulitems_i}\mcp_j\cdot \mca_{ij}
        \right)
        \\
        &\overset{(f)}{\geq} 
        1.08208 \budgetscalar\cdot 
        \sum_{j\in\meaningfulitems_i}\valij\cdot \mca_{ij}
        -
        \moneycost_i\left(
        \budgetscalar\cdot 
        \displaystyle
        \sum_{j\in\meaningfulitems_i}\mcp_j\cdot \mca_{ij}
        \right)
        \\
        &\overset{(g)}{\geq} 
        0.08208 \budgetscalar\cdot 
        \sum_{j\in\meaningfulitems_i}\valij\cdot \mca_{ij}
        +
        \budgetscalar\cdot 
        \left(
        \sum_{j\in\meaningfulitems_i}\valij\cdot \mca_{ij}
        -
        \moneycost_i\left(
        \displaystyle
        \sum_{j\in\meaningfulitems_i}\mcp_j\cdot \mca_{ij}
        \right)
        \right)
        \\
        &\geq  
        0.08208 \budgetscalar\cdot 
        \sum_{j\in\meaningfulitems_i}\valij\cdot \mca_{ij}
    \end{align*}
    where equality~(a) holds due to inequality~\eqref{eq:value lower bound mixed nash};
    equality~(b) holds since 
    agent $i$ exhausts her budget conditioning on 
    event $\eventHat_i(\bpbthreshold)$
    for every $\bpbthreshold\in[0, 1]$;
    inequality~(c) holds due to the convexity of 
    $\moneycost_i$ and $\bpbthreshold \geq 1$,
    $\pricethreshold = \frac{1}{4}$,
    $\probthreshold = \frac{2}{27}$,
    $\budgetscalar = \frac{1}{4}$;\footnote{
    More specifically, 
    $
        \int_1^\infty
        \frac{1}{\bpbthreshold}
        \cdot 
        \moneycostderivative_i^+(
    \sum_{j\in[m]}\mcp_j\cdot \mca_{ij}
    )
    \cdot 
    z_{\bpbthreshold}
    \,d\CDFHat_i(\bpbthreshold)
    -
        \moneycost_i(
        \int_0^1
        \deviatewealth_i
        \,d\CDFHat_i(\bpbthreshold)
        +
        \int_1^\infty
        z_{\bpbthreshold}
        \,d\CDFHat_i(\bpbthreshold)
        )$
        is a concave function for every 
        variable $z_{\bpbthreshold}\in[0, \deviatewealth_i]$.
        Thus, it attains its minimum at the 
        boundary, i.e., $z_{\bpbthreshold} = 0$
        or $z_{\bpbthreshold} = \deviatewealth_i$.
        Given pre-specified parameters 
        $\pricethreshold = \frac{1}{4}$,
    $\probthreshold = \frac{2}{27}$,
    $\budgetscalar = \frac{1}{4}$,
    it can be verified that the minimum is 
    attained at $z_{\bpbthreshold} = \deviatewealth_i$
    for every $\bpbthreshold \geq 1$.
    }
    equality~(d) holds due to the definition of 
    $\deviatewealth_i$;
    inequality~(e) holds due to \Cref{lem:mc foc};
    inequality~(f) holds where we evaluate
    the integral term at our pre-specified parameters
    $\pricethreshold = \frac{1}{4}$,
    $\probthreshold = \frac{2}{27}$,
    $\budgetscalar = \frac{1}{4}$;
    and inequality~(g) holds due to the convexity of $\moneycost_i$.

    Combining inequalities~\eqref{eq:high items bound mixed nash}
    and \eqref{eq:low items bound mixed nash}, we have
    \begin{align*}
        \left(\frac{4}{\pricethreshold\probthreshold} + 
        \frac{2}{0.08208 \budgetscalar}
        \right)
        \cdot \wtp(\allocs)
        &\geq
      \sum_{i\in[n]}
      \sum_{j\in \hitems}
      4\mcp_j\cdot \mca_{ij}
      +
      \sum_{i\in[n]}
      2\moneycost_i^{-1}\left(
      \sum_{j\in \litems}
      2\valij\cdot \mca_{ij}
      \right)
      \\
      &\geq 
      2\wtp(\mcas)
      \geq
      \wtp(\allocs^*)
    \end{align*}
    where $\frac{4}{\pricethreshold\probthreshold} + 
        \frac{2}{0.08208 \budgetscalar}
        \approx 313.47.
        $
\end{proof}

\begin{lemma}
\label{lem:prob bound}
    Given any $m\in\naturals$, $\pricethreshold \in [0, 1]$,
    $\probthreshold\in[0, 1]$,
    $\budgetscalar\in[0, 1]$,
    non-negative constants $\mcp_1, \dots, \mcp_m\in\reals_+$,
    and non-negative (possibly correlated) random variables 
    $\price_1, \dots, \price_m$ such that 
    $\prob{\price_j \geq \pricethreshold\cdot \mcp_j} \leq 
        \probthreshold$
    for every $j\in[m]$,
    define random subset $\goodmeaningfulitems \triangleq \{j\in[m]:\price_j\leq \mcp_j\}$.
    Then,
    for every $\bpbthreshold\geq \pricethreshold$:
    \begin{align*}
        \prob{
        \sum_{j\in \goodmeaningfulitems}\price_j
        +
        \budgetscalar\cdot 
        \sum_{j\in[m]} \mcp_j
        \leq 
        \bpbthreshold\cdot 
        \sum_{j\in \goodmeaningfulitems}
        \mcp_j
        }
        \geq 1 - \frac{\pricethreshold(1-\probthreshold) + \bpbthreshold \probthreshold}{\bpbthreshold - \budgetscalar}
    \end{align*}
\end{lemma}
\begin{proof}
Note that 
\begin{align*}
        &~~\prob{
        \sum_{j\in \goodmeaningfulitems}\price_j
        +
        \budgetscalar\cdot 
        \sum_{j\in[m]} \mcp_j
        \leq 
        \bpbthreshold\cdot 
        \sum_{j\in \goodmeaningfulitems}
        \mcp_j
        }
        =
        \prob{
        \sum_{j\in \goodmeaningfulitems}\price_j
        +
        \bpbthreshold\cdot \sum_{j\not\in \goodmeaningfulitems}\mcp_j
        \leq 
        \left(\bpbthreshold-\budgetscalar\right)\cdot 
        \sum_{j\in [m]}
        \mcp_j
        }
        \\
        &\overset{(a)}{\geq} 
        1 - \frac{\expect{
        \displaystyle\sum_{j\in \goodmeaningfulitems}\price_j
        +
        \bpbthreshold\cdot \sum_{j\not\in \goodmeaningfulitems}\mcp_j
        }}{
        \left(\bpbthreshold-\budgetscalar\right)\cdot 
        \displaystyle\sum_{j\in [m]}
        \mcp_j
        }
        % \\
        \overset{}{\geq} 
        1 - \frac{
        \displaystyle\sum_{j\in [m]}\pricethreshold(1-\probthreshold)\cdot \mcp_j
        +
        \bpbthreshold\cdot \sum_{j\in[m]}\probthreshold\cdot\mcp_j
        }{
        \left(\bpbthreshold-\budgetscalar\right)\cdot 
        \displaystyle\sum_{j\in [m]}
        \mcp_j
        }
        \\
        &=
        1 - \frac{\pricethreshold(1-\probthreshold) + \bpbthreshold \probthreshold}{\bpbthreshold - \budgetscalar}
\end{align*}
where inequality~(a) holds due to Markov's inequality.
\end{proof}

    

==> Notes/single-agent-pacing.tex <==
\section{Pacing Equilibrium in Single-agent Environment With Reserve}

In this section, we discuss the pacing equilibrium 
for both first/second-price auction with 
reserve when there is only a single agent.

\subsection{Model}
There is a single agent and $m$ items.
The agent has budget $\wealth$ and $\val_j$ for each item~$j\in[m]$.
The seller is allowed to select an \emph{item-anonymous} reserve price $\reserve$.

\subsection{Pacing Equilibrium}
Motivated by first price pacing equilibrium when there is no reserve price \citep{CKPSSSW-22,CKSS-22},
we extend it to the equilibrium 
under reserve price.
Without loss of generality, we assume $\val_1 \geq \val_2
\geq \dots \geq \val_m > 0$.

\paragraph{First price pacing equilibrium.} We first consider 
pacing equilibrium under first-price semantic.

\begin{definition}
Given reserve price $\reserve\geq 0$,
a \emph{first price pacing equilibrium (best response)}
is a scalar $\pacescalar\in[0, 1]$ such that 
there exists allocation profile $\mathbf\alloc\in[0,1]^m$,
\begin{align*}
\begin{array}{rl}
\text{(budget feasibility)}&
~ 
    \sum_{j\in[m]:\pacescalar\cdot \val_j \geq \reserve} 
    \alloc_j\cdot 
    \pacescalar\cdot \val_j \leq \wealth 
    \\
\text{(demanded good sold completely)}&
~
\forall j\in[m], \pacescalar\cdot \val_j > \reserve:
    \alloc_j = 1  
    \\
\text{(no unnecessary pacing)}&
~
    \text{if } 
    \sum_{j\in[m]:\pacescalar\cdot \val_j \geq \reserve} 
    \alloc_j\cdot 
    \pacescalar\cdot \val_j < \wealth,
    \text{then }
\alpha = 1
    \end{array}
\end{align*}
\end{definition}

\begin{claim}
For any reserve price $\reserve$, there exists unique first price pacing 
equilibrium $\pacescalar$.
Furthermore, the pacing multiplier $\pacescalar$ is weakly increasing in 
reserve price $\reserve$.
\end{claim}


\begin{claim}
Among first-price pacing equilibrium for all possible $\reserve$,
the revenue is maximized when there is no reserve, i.e., $\reserve = 0$.
\end{claim}
\begin{proof}
Suppose $\sum_{j\in[m]}\val_j \leq \wealth$.
No unnecessary pacing property implies that $\alpha = 1$ 
when reserve price $\reserve = 0$. Thus, the revenue (without reserve) is
 $\sum_{j\in[m]}\val_j \leq \wealth$, which is maximized.
 
Suppose $\sum_{j\in[m]}\val_j > \wealth$.
When reserve price $\reserve = 0$,
the pacing multiplier $\pacescalar < 1$ and thus
the revenue is
 $\wealth$, which is maximized.
\end{proof}


\paragraph{Second price pacing equilibrium.}
Here we consider pacing equilibrium under second-price semantic.

\begin{definition}
Given reserve price $\reserve\geq 0$,
a \emph{second price pacing equilibrium (best response)}
is a scalar $\pacescalar\in[0, 1]$ such that 
there exists allocation profile $\mathbf\alloc\in[0,1]^m$,
\begin{align*}
\begin{array}{rl}
\text{(budget feasibility)}&
~ 
    \sum_{j\in[m]:\pacescalar\cdot \val_j \geq \reserve} 
    \alloc_j\cdot 
    \reserve \leq \wealth 
    \\
\text{(demanded good sold completely)}&
~
\forall j\in[m], \pacescalar\cdot \val_j > \reserve:
    \alloc_j = 1  
    \\
\text{(no unnecessary pacing)}&
~
    \text{if } 
    \sum_{j\in[m]:\pacescalar\cdot \val_j \geq \reserve} 
    \alloc_j\cdot 
   \reserve < \wealth,
    \text{then }
\alpha = 1
    \end{array}
\end{align*}
\end{definition}

\begin{claim}
For any reserve price $\reserve$, there exists second price pacing  equilibrium $\pacescalar$.
Furthermore, the pacing multiplier $\pacescalar$ is 
\emph{non-monotone} in 
reserve price $\reserve$.
\end{claim}

Fixing any reserve price $\reserve$, let $D(\reserve) \triangleq \frac{\wealth}{\reserve}$ be the total demand under budget $\wealth$ and per-unit price $\reserve$;
and $S(\reserve) \triangleq |\{j\in[m]:\val_j \geq \reserve\}|$ be the number of items whose value is above $\reserve$. Note that 
\begin{itemize}
\item 
both functions $D(\cdot)$ and $S(\cdot)$ is monotone decreasing
\item $D(0) = \infty > S(0) = m$, and 
$D(\val_1 + \epsilon) > 0 = S(\val_1 + \epsilon)$.
Recall item 1 has the highest value.
\item If $D(\reserve) \geq S(\reserve)$, the pacing multiplier $\alpha = 1$, i.e., no pacing.
Otherwise, the pacing multiplier $\alpha\in (0, 1)$ is selected 
so that budget feasibility property is binding.
\item If function $D(\cdot)$ and function $S(\cdot)$
cross multiple time, then pacing multiplier $\alpha$
is not monotone in $\reserve$.
\end{itemize}

\newpage

==> Notes/single-item-new-analysis-old.tex <==
\section{New Analysis for Single Item}

In this section, we consider the metagame 
for a single item. 
We focus on the PoA of pure Nash equilibrium.
We assume  
that agents have concave valuation functions $\{\valuefunc_i\}$
and convex disutilities of money $\{\moneycost_i\}$.
In the metagame, the agents report both their values and budgets 
to the inner game.



\subsection{A $\frac{3 + \sqrt{5}}{2}$-approximation Analysis for Pure Nash}

In this subsection, we assume that 
agents have (differentiable) concave valuation functions 
 $\{\valuefunc_i\}$ and 
 (differentiable) convex disutilities of money $\{\moneycost_i\}$
 up to heterogeneous budgets $\{\truewealth_i\}$.
Recall that $\valuefuncderivative_i(\alloci)$
is the derivative of valuation function $\valuefunc_i$
at allocation $\alloci$,
and $\moneycostderivative_i(\price_i)$
is the derivative of disutility of money $\moneycost$ 
at payment $\price_i$.
The PoA guarantee is as follows.
 
\begin{theorem}
\label{thm:single item concave value hard budget}
    In the single-item environment,
    for agents with (differentiable) concave valuation functions 
 $\{\valuefunc_i\}$ and 
 (differentiable) convex disutilities of money $\{\moneycost_i\}$
 up to heterogeneous budgets $\{\truewealth_i\}$,
    the pure Nash PoA of transferable welfare 
    is at most $\frac{3 + \sqrt{5}}{2}\approx 2.618$.
\end{theorem}

Before the proof of \Cref{thm:single item concave value hard budget},
we first establish a lowerbound on 
the allocation in an arbitrary pure Nash equilibrium
for every agent $i$ whose true budget $\truewealth_i$ is not exhausted.

\begin{lemma}
\label{lem:alloc lower bound single item concave value hard budget}
    In the single-item environment,
    for agents with (differentiable) concave valuation functions 
 $\{\valuefunc_i\}$ and 
 (differentiable) convex disutilities of money $\{\moneycost_i\}$
 up to heterogeneous budgets $\{\truewealth_i\}$,
and every pure Nash equilibrium $\eqlb$,
suppose $\xbf, \price$
are the allocation and per-unit price in the induced FPPE.
For every agent $i$ who does not exhaust her true budget $\truewealth_i$,
i.e., $\alloci\cdot \price < \truewealth_i$,
her allocation $\alloci$ is at least 
\begin{align*}
    \alloci \geq 1 - \frac{\price}{\valuefuncderivative_i(\alloci)}
    \moneycostderivative_i(\price\alloci)
\end{align*}
\end{lemma}
\begin{proof}
    Fix an arbitrary Nash equilibrium $\eqlb$.
    Suppose $\allocs,\price$ are the allocation and per-unit price in the induced FPPE.
    Fix an arbitrary agent $i$ who does not exhaust her true budget $\truewealth_i$,
i.e., $\alloci\cdot \price < \truewealth_i$.
Furthermore, we assume that $\valuefuncderivative_i(\alloc_i) > \price$;
otherwise, $1 - \frac{\price}{\valuefuncderivative_i(\alloc_i)}
\moneycostderivative_i(\price\alloci)
\leq 0$ and thus the lemma statement holds trivially.



    Firstly note that the same FPPE and thus the same utility for every agent are induced
    if 
    we hold all other agents' reports fixed and let 
    agent $i$ report
    $\val_i\primed = \valuefuncderivative_i(\alloci)$ and $\wealth_i\primed = \alloc_i \cdot \price$.
    Next consider agent $i$ increases her reported budget by $\epsilon$
    for sufficiently small and positive $\epsilon < \min\{\truewealth_i - \wealth_i\primed,
    \valuefuncderivative_i(\alloci) 
    -
    \price
    \}$,
    i.e., $\wealth_i\doubleprimed = \wealth_i\primed + \epsilon < \truewealth_i$.
    Let $\allocs\doubleprimed,\price\doubleprimed$ be 
    the allocation and per-unit price in the new induced FPPE.
    We have 
    \begin{align*}
        \price\doubleprimed \overset{(a)}{\leq} \price + \epsilon
        \qquad\qquad
        \alloc_i\doubleprimed \overset{(b)}{=}
        \frac{\wealth_i\doubleprimed}{\price\doubleprimed} 
        \geq 
        \frac{\wealth_i\primed + \epsilon}{\price + \epsilon}
        =
        \frac{\alloci \cdot \price + \epsilon}{\price + \epsilon}
    \end{align*}
    where inequality~(a) holds due to the construction of per-unit price in FPPE;
    equality~(b) holds due to the unnecessary pacing constraint implied 
    by the construction $\val_i\doubleprimed = \infty$.
    In this new induced FPPE, the utility $\util_i\doubleprimed$ of agent $i$ is 
    \begin{align*}
    \util_i\doubleprimed
    =
        \valuefunc_i(\alloc_i\doubleprimed) 
        - \moneycost_i(\wealth_i\doubleprimed)
    \end{align*}
    where the first equality holds due to the 
    the unnecessary pacing constraint implied 
    by the construction $\val_i\doubleprimed = \valuefuncderivative_i(\alloci) > \price + \epsilon \geq \price\primed$.
    With a similar argument, the utility $\util_i$
    of agent $i$ in the original FPPE induced by equilibrium $\eqlb$
    is 
    \begin{align*}
        \util_i
    =
        \valuefunc_i(\alloc_i) 
        - \moneycost_i(\wealth_i\primed)
    \end{align*}
    Note that $\util_i - \util_i\doubleprimed \geq 0$ 
    since the former is the utility in the equilibrium, and the later
    is the utility after the deviation.
    Furthermore, we have 
    \begin{align*}
        \valuefunc_i(\alloc_i) - \moneycost_i(\wealth_i\primed) - 
        \left(
        \valuefunc_i(\alloci\doubleprimed) - \moneycost_i(\wealth_i\doubleprimed)
        \right)
        &= 
        \moneycost_i(\wealth_i\doubleprimed)
        - 
        \moneycost_i(\wealth_i\primed)
        -
         \left(
         \valuefunc_i(\alloci\doubleprimed) - \valuefunc_i(\alloci)
         \right)
        \\
        &\overset{(a)}{\leq}
        \left(
        \wealth_i\doubleprimed - \wealth_i\primed
        \right)
        \cdot 
        \moneycostderivative_i(\wealth\doubleprimed)
        -
        \left(\alloci\doubleprimed - \alloci\right)
        \cdot 
         \valuefuncderivative_i(\alloci\doubleprimed)
         \\
         &\overset{}{\leq}
         \epsilon
         \cdot 
         \moneycostderivative_i(\price\alloc_i + \epsilon)
         - 
         \left(
         \frac{\alloci\cdot \price + \epsilon}{\price + \epsilon}
         -
         \alloci
         \right)
        \cdot 
         \valuefuncderivative_i(\alloci\doubleprimed)
         \\
         &=
         \epsilon
         \cdot 
         \moneycostderivative_i(\price\alloc_i + \epsilon)
         - 
         \epsilon\cdot
         \frac{1-\alloci}{\price + \epsilon}
        \cdot 
         \valuefuncderivative_i(\alloci\doubleprimed)
    \end{align*}
    where inequality~(a) holds since $\alloci\doubleprimed > \alloci$, valuation function $\valuefunc_i$
    is concave and differentiable,
    $\truewealth_i > \wealth_i\doubleprimed > \wealth_i\primed$,
    and 
    disutility of money $\moneycost_i$
    is convex and differentiable up to $\truewealth_i$.
    Combining with $\util_i - \util_i\doubleprimed \geq 0$,
    we have 
    \begin{align*}
        \alloc_i \geq 1 - \frac{\price + \epsilon}{\valuefuncderivative_i(\alloci\doubleprimed)}
        \moneycostderivative_i(\price\alloci+\epsilon)
    \end{align*}
    for all positive $\epsilon$ that is sufficiently small.
    Finally, letting $\epsilon$ go to zero
    finishes the proof.
\end{proof}

Now we are ready to prove \Cref{thm:single item concave value hard budget}.

\begin{proof}[Proof of \Cref{thm:single item concave value hard budget}]
    Fix an arbitrary Nash equilibrium $\eqlb$.
    Suppose $\allocs,\price$ are the allocation and per-unit price in the induced FPPE. 
    Let  
    $\mathbf\optalloc$ be the allocation in the optimal transferable welfare.
    We introduce the following partition $A_1\bigsqcup A_2\bigsqcup A_3\bigsqcup A_4$
    of agents based on $\allocs$, $\price$, and $\mathbf\optalloc$:
    \begin{align*}
        A_1 &\triangleq 
        \{i\in[n]: \alloci \cdot \price = \truewealth_i\}
        \\
        % A_2 &\triangleq
        % \{i\in[n]: i \not\in A_1
        % \land \valuefuncderivative_i(\optalloc_i) \leq \pricethreshold\cdot \price
        % \}
        A_2 &\triangleq
        \{i\in[n]: i \not\in A_1
        \land \optalloc_i \leq \alloci
        \}
        \\
        % A_3 &\triangleq
        % \{i\in[n]: i \not\in A_1
        % \land \valuefuncderivative_i(\optalloc_i) > \pricethreshold\cdot \price
        % \land \optalloc_i \leq \alloci
        % \}
        A_3 &\triangleq
        \{i\in[n]: i \not\in A_1
        \land \optalloc_i > \alloci
        \land \valuefuncderivative_i(\alloc_i) \leq \pricethreshold\cdot \price
        \moneycostderivative_i(\price\alloci)
        \}
        \\
        A_4 &\triangleq
        \{i\in[n]: i \not\in A_1
        \land \optalloc_i > \alloci
        \land \valuefuncderivative_i(\alloc_i) > \pricethreshold\cdot \price
        \moneycostderivative_i(\price\alloci)
        \}
    \end{align*}
    where $\pricethreshold = \frac{1+\sqrt{5}}{2}\approx 1.618$ 
    is the golden ratio.
    In words, $A_1$ corresponds to every agent $i$ who exhausts her true budget $\truewealth_i$ in the equilibrium;
    and $A_2$, $A_3$, $A_4$ correspond to remaining agents.

    For every agent $i\in A_4$, her allocation $\alloc_i$
    is the equilibrium is at least 
    \begin{align*}
        \alloci 
        % \overset{(a)}{\geq}
        % 1 - \frac{\price}{\valuefuncderivative_i(\alloci)}
        \overset{(a)}{\geq} 
        1 - \frac{\price}{\valuefuncderivative_i(\alloc_i)}
        \moneycostderivative_i(\price\alloci)
        \overset{(b)}{\geq}
        1 - \frac{1}{\pricethreshold}
        = 
        \frac{\pricethreshold - 1}{\pricethreshold}
    \end{align*}
    where inequality~(a) is guaranteed due to \Cref{lem:alloc lower bound single item concave value hard budget};
    % inequality~(b) holds since $\optalloc_i > \alloci$
    % and the concavity of valuation function $\valuefunc_i$;
    and inequality~(b) is guaranteed since $\valuefuncderivative_i(\alloc_i) > \pricethreshold\cdot \price\moneycostderivative_i(\price\alloci)$.

    Next, we compare the transferable welfare contribution from $A_1, A_2, A_3, A_4$ separately.

    \smallskip
    For every agent $i\in A_1$, note that 
    \begin{align*}
        \wtp_i(\optalloc_i) 
        \overset{(a)}{\leq} \truewealth_i
        \overset{(b)}{=}
        \wtp_i(\alloci)
    \end{align*}
    where the inequality holds due to the definition of $\wtp_i$;
    and the equality holds due to the definition of $A_1$.
    
    For every agent $i\in A_2$, note that 
    \begin{align*}
        \wtp_i(\optalloc_i) \leq \wtp_i(\alloci)
    \end{align*}
    where the inequality holds since $\optalloc_i \leq \alloci$ implied by the definition of $A_2$.

    For every agent $i\in A_3$, note that 
    \begin{align*}
        \wtp_i(\optalloc_i) 
        &\overset{(a)}{\leq} 
        \wtp_i(\alloci) + 
        \frac{
        \valuefunc_i(\optalloc_i) - \valuefunc_i(\alloci)
        }{
        \moneycostderivative_i(\wtp_i(\alloci))
        }
        \\
        &\overset{(b)}{\leq} 
         \wtp_i(\alloci) + 
        \frac{
        \valuefunc_i(\optalloc_i) - \valuefunc_i(\alloci)
        }{
        \moneycostderivative_i(\price\alloci)
        }
        \\
        &\overset{(c)}{\leq} 
         \wtp_i(\alloci) + (\optalloc_i - \alloci)
         \cdot \frac{\valuefuncderivative_i(\alloc_i)}{
         \moneycostderivative_i(\price\alloci)
         }
         \\
        &\overset{(c)}{\leq}
        \wtp_i(\alloci) + \optalloc_i\cdot \pricethreshold\cdot \price
    \end{align*}
    where inequality~(a) holds due to the definition of $\wtp_i$ and the convexity of $\moneycost_i$;
    inequality~(b) holds since 
    $\moneycostderivative_i$ is weakly increasing implied by
    the convexity of 
    $\moneycost_i$,
    and 
    $\wtp_i(\alloci) \geq \price\alloci$ which is implied by the definition of $\wtp_i$ and 
    the fact that 
    agent $i$'s utility is non-negative in the equilibrium;
    inequality~(c) holds due to the concavity of valuation function $\valuefunc_i$;
    and inequality~(d) holds due since $\valuefuncderivative_i(\alloci) \leq \pricethreshold\cdot 
    \price\moneycostderivative_i(\price\alloci)$ implied by the definition of $A_3$.

    For every agent $i\in A_4$, note that 
    \begin{align*}
        \wtp_i(\optalloc_i) =
        \wtp_i\left(\alloci \cdot \frac{\optalloc_i}{\alloci}\right)
        \overset{(a)}{\leq}
        \frac{\optalloc_i}{\alloci}
        \cdot \wtp_i(\alloci)
        \overset{(b)}{\leq}
        \frac{\pricethreshold\optalloc_i}{\pricethreshold - 1}
        \cdot \wtp_i(\alloci)
    \end{align*}
    where inequality~(a) holds due to the concavity of $\wtp_i$;
    and inequality~(b) holds due to the lowerbound of $\alloci$ established above.

    \smallskip
    Putting all pieces together, we have the following upper bound of
    the optimal transferable welfare $\wtp(\mathbf\optalloc)$,
    \begin{align}
    \label{eq:welfare upper bound single item concave value hard budget}
    \begin{split}
        \wtp(\mathbf\optalloc) 
        &= 
        \sum_{i\in[n]} \wtp_i(\optalloc_i)
        \\
        &\leq 
        \left(\sum_{i\in A_3} \optalloc_i
        \right)\cdot \pricethreshold \price 
        +
        \sum_{i\in A_1\sqcup A_2 \sqcup A_3}
        \wtp_i(\alloci)
        +
        \sum_{i\in A_4}
        \frac{\pricethreshold\optalloc_i}{\pricethreshold - 1}
        \cdot \wtp_i(\alloci)
        \\
        &\leq 
        \left(1 - \sum_{i\in A_4} \optalloc_i
        \right)\cdot \pricethreshold \price 
        +
        \sum_{i\in A_1\sqcup A_2 \sqcup A_3}
        \wtp_i(\alloci)
        +
        \sum_{i\in A_4}
        \frac{\pricethreshold\optalloc_i}{\pricethreshold - 1}
        \cdot \wtp_i(\alloci)
        \\
        &\leq 
        \left(1 - \sum_{i\in A_4} \optalloc_i
        \right)\cdot \pricethreshold \wtp(\allocs)
        +
        \sum_{i\in A_1\sqcup A_2 \sqcup A_3}
        \wtp_i(\alloci)
        +
        \sum_{i\in A_4}
        \frac{\pricethreshold\optalloc_i}{\pricethreshold - 1}
        \cdot \wtp_i(\alloci)
        \end{split}
    \end{align}
    To further simplify upper bound~\eqref{eq:welfare upper bound single item concave value hard budget}, 
    we analyze two cases separately. 

    Firstly, suppose $A_4$ is empty. In this case,
    \begin{align*}
        \text{Right-hand side of \eqref{eq:welfare upper bound single item concave value hard budget}}
        =
        \pricethreshold \wtp(\allocs) + \wtp(\allocs) 
        =
        \frac{3+\sqrt{5}}{2}\wtp(\allocs)
    \end{align*}

    Next, suppose $A_4$ is not empty. 
    In this case, 
    let $X \triangleq \sum_{i\in A_4} \optalloc_i$.
    By the definition of $A_4$ and the fact that 
    $\alloci \geq \frac{\pricethreshold  -1}{\pricethreshold}$
    for every $i\in A_4$,
    we have
    $X \geq \sum_{i\in A_4} \alloci \geq \frac{\pricethreshold  -1}{\pricethreshold}$.
    Finally, by algebra we have\footnote{To see this, consider an optimization program where variables are $\{\optalloc_i\}_{i\in A_4}$;
    the constraints are $\optalloc_i \geq 0$ for every $i\in A_4$,
    and $\sum_{i\in A_4} \optalloc_i = X$;
    and the objective is the right-hand side of \eqref{eq:welfare upper bound single item concave value hard budget}.
    In this optimization program,
    the optimal solution finds $k \triangleq \argmax_{i\in A_4}\wtp_i(\alloci)$,
    and set $\optalloc_i = X \cdot \indicator{i = k}$
    for every $i\in A_4$.}
    \begin{align*}
        \text{Right-hand side of \eqref{eq:welfare upper bound single item concave value hard budget}}
        &\leq 
        \left(1 - X\right) \cdot \pricethreshold \wtp(\allocs) 
        +
        \frac{\pricethreshold X}{\pricethreshold - 1}\wtp(\allocs)
        \\
        &=
        \left(\pricethreshold + \frac{2\pricethreshold -\pricethreshold^2}{\pricethreshold - 1} X\right)
        \wtp(\allocs)
        \\
        &\leq 
        \left(\pricethreshold + \frac{2\pricethreshold -\pricethreshold^2}{\pricethreshold - 1}\right)
        \wtp(\allocs)
        \\
        &=\frac{\pricethreshold}{\pricethreshold - 1}
        \wtp(\allocs)
        =
        \frac{3+\sqrt{5}}{2}
        \wtp(\allocs)
    \end{align*}
    where the last inequality holds since $\frac{2\pricethreshold -\pricethreshold^2}{\pricethreshold - 1} > 0$ and $X \leq 1$.
\end{proof}

\begin{remark}
    The same PoA bound and analysis hold if we consider 
    the variant model where the agents have linear valuation function, and can only report budgets in the metagame.
\end{remark}

\subsection{A $4$-approximation Analysis for Pure Nash}

\begin{theorem}
    In the single-item environment,
    for agents with concave valuation functions
    $\{\valuefunc_i\}$
and convex disutilities of money $\{\moneycost_i\}$,
    the PoA of transferable welfare 
    is at most 4.
\end{theorem}

\begin{lemma}
    For every agent $i$,
    every other agents' report $(\val_{-i},\wealth_{-i})$ in the metagame, 
    and
    every payment constraint $\tilde\price \in \reals_+$,
    we have
    \begin{align*}
        (\infty, \tilde\price)
        \in
        \argmax_{(\val_i, \wealth_i)}
        ~
        \alloc_i(\val_i, \wealth_i, \val_{-i}, \wealth_{-i})
        \quad
        \text{s.t.}
        \quad 
        \price_i(\val_i, \wealth_i, \val_{-i}, \wealth_{-i}) = \tilde\price
    \end{align*}
\end{lemma}

Inspired by the lemma above, we define auxiliary functions
$\alloc_i^{(\val_{-i}, \wealth_{-i})}(\cdot)$,
$\price_i^{(\val_{-i}, \wealth_{-i})}(\cdot)$,
and 
$\price^{(\val_{-i}, \wealth_{-i})}(\cdot)$
as follows
\begin{align*}
    \alloc_i^{(\val_{-i}, \wealth_{-i})}(\price)
    &\triangleq 
    \alloc_i(\infty, \price, \val_{-i}, \wealth_{-i})
    \\
    \price_i^{(\val_{-i}, \wealth_{-i})}(\alloc)
    &\triangleq
    \min \{\price:
    \alloc_i^{(\val_{-i}, \wealth_{-i})}(\price) = \alloc
    \}
    \\
    \price^{(\val_{-i}, \wealth_{-i})}(\alloc)
    &\triangleq
    \frac{\price_i^{(\val_{-i}, \wealth_{-i})}(\alloc)}{\alloc}
\end{align*}


\begin{lemma}
For every agent $i$, for every allocation $\alloc\primed,\alloc\doubleprimed \in (0, 1)$,
\begin{align*}
    \price^{(\val_{-i}, \wealth_{-i})}(\alloc\primed)
    \leq 
    \frac{1}{1 - \alloc\primed}
    {\price^{(\val_{-i}, \wealth_{-i})}(\alloc\doubleprimed)}
\end{align*}
\end{lemma}

\begin{lemma}
    For every agent $i$, $\alloc_i^{(\val_{-i}, \wealth_{-i})}(\price)$
is concave in $\price$.
Furthermore, 
if agent $i$ has concave valuation function
    $\valuefunc_i$,
    then $\valuefunc_i(\alloc_i^{(\val_{-i}, \wealth_{-i})}(\price))$
    is also concave in $\price$.
\end{lemma}

\begin{lemma}
    Fix an arbitrary pure Nash equilibrium $\eqlb$,
    suppose $\allocs\primed,\price\primed$
    are the allocation and per-unit price 
    in the induced FPPE.
    For every agent $i$, we have
    \begin{align*}
        \price^{(\val_{-i}, \wealth_{-i})}(\alloc_i\primed) 
        \leq 
         \price\primed
    \end{align*}
\end{lemma}


==> Notes/single-item-new-analysis.tex <==
\section{New Analysis for Single Item}

In this section, we consider the metagame 
for a single item. 
We focus on the PoA of pure Nash equilibrium.
We assume  
that agents have concave valuation functions $\{\valuefunc_i\}$
and convex disutilities of money $\{\moneycost_i\}$.
In the metagame, the agents report both their values and budgets 
to the inner game.



\subsection{A $2$-approximation Analysis for Pure Nash}

In this subsection, we assume that 
agents have (differentiable) concave valuation functions 
 $\{\valuefunc_i\}$ and 
 (differentiable) convex disutilities of money $\{\moneycost_i\}$
 up to heterogeneous budgets $\{\truewealth_i\}$.
Recall that $\valuefuncderivative_i(\alloci)$
is the derivative of valuation function $\valuefunc_i$
at allocation $\alloci$,
and $\moneycostderivative_i(\price_i)$
is the derivative of disutility of money $\moneycost$ 
at payment $\price_i$.
The PoA guarantee is as follows.
 
\begin{theorem}
\label{thm:single item concave value convex budget pure}
    In the single-item environment,
    for agents with (differentiable) concave valuation functions 
 $\{\valuefunc_i\}$ and 
 (differentiable) convex disutilities of money $\{\moneycost_i\}$
 up to heterogeneous budgets $\{\truewealth_i\}$,
    the pure Nash PoA of transferable welfare 
    is at most $2$.
\end{theorem}

Before the proof of \Cref{thm:single item concave value convex budget pure},
we first establish a lowerbound on 
the allocation in an arbitrary pure Nash equilibrium
for every agent $i$ whose true budget $\truewealth_i$ is not exhausted.

\begin{lemma}
\label{lem:alloc lower bound single item concave value hard budget}
    In the single-item environment,
    for agents with (differentiable) concave valuation functions 
 $\{\valuefunc_i\}$ and 
 (differentiable) convex disutilities of money $\{\moneycost_i\}$
 up to heterogeneous budgets $\{\truewealth_i\}$,
and every pure Nash equilibrium $\eqlb$,
suppose $\xbf, \price$
are the allocation and per-unit price in the induced FPPE.
For every agent $i$ who does not exhaust her true budget $\truewealth_i$,
i.e., $\alloci\cdot \price < \truewealth_i$,
her allocation $\alloci$ is at least 
\begin{align*}
    \alloci \geq 1 - \frac{\price}{\valuefuncderivative_i(\alloci)}
    \moneycostderivative_i(\price\alloci)
\end{align*}
\end{lemma}
\begin{proof}
    Fix an arbitrary Nash equilibrium $\eqlb$.
    Suppose $\allocs,\price$ are the allocation and per-unit price in the induced FPPE.
    Fix an arbitrary agent $i$ who does not exhaust her true budget $\truewealth_i$,
i.e., $\alloci\cdot \price < \truewealth_i$.
Furthermore, we assume that $\valuefuncderivative_i(\alloc_i) > \price$;
otherwise, $1 - \frac{\price}{\valuefuncderivative_i(\alloc_i)}
\moneycostderivative_i(\price\alloci)
\leq 0$ and thus the lemma statement holds trivially.



    Firstly note that the same FPPE and thus the same utility for every agent are induced
    if 
    we hold all other agents' reports fixed and let 
    agent $i$ report
    $\val_i\primed = \valuefuncderivative_i(\alloci)$ and $\wealth_i\primed = \alloc_i \cdot \price$.
    Next consider agent $i$ increases her reported budget by $\epsilon$
    for sufficiently small and positive $\epsilon < \min\{\truewealth_i - \wealth_i\primed,
    \valuefuncderivative_i(\alloci) 
    -
    \price
    \}$,
    i.e., $\wealth_i\doubleprimed = \wealth_i\primed + \epsilon < \truewealth_i$.
    Let $\allocs\doubleprimed,\price\doubleprimed$ be 
    the allocation and per-unit price in the new induced FPPE.
    We have 
    \begin{align*}
        \price\doubleprimed \overset{(a)}{\leq} \price + \epsilon
        \qquad\qquad
        \alloc_i\doubleprimed \overset{(b)}{=}
        \frac{\wealth_i\doubleprimed}{\price\doubleprimed} 
        \geq 
        \frac{\wealth_i\primed + \epsilon}{\price + \epsilon}
        =
        \frac{\alloci \cdot \price + \epsilon}{\price + \epsilon}
    \end{align*}
    where inequality~(a) holds due to the construction of per-unit price in FPPE;
    equality~(b) holds due to the unnecessary pacing constraint implied 
    by the construction $\val_i\doubleprimed = \infty$.
    In this new induced FPPE, the utility $\util_i\doubleprimed$ of agent $i$ is 
    \begin{align*}
    \util_i\doubleprimed
    =
        \valuefunc_i(\alloc_i\doubleprimed) 
        - \moneycost_i(\wealth_i\doubleprimed)
    \end{align*}
    where the first equality holds due to the 
    the unnecessary pacing constraint implied 
    by the construction $\val_i\doubleprimed = \valuefuncderivative_i(\alloci) > \price + \epsilon \geq \price\primed$.
    With a similar argument, the utility $\util_i$
    of agent $i$ in the original FPPE induced by equilibrium $\eqlb$
    is 
    \begin{align*}
        \util_i
    =
        \valuefunc_i(\alloc_i) 
        - \moneycost_i(\wealth_i\primed)
    \end{align*}
    Note that $\util_i - \util_i\doubleprimed \geq 0$ 
    since the former is the utility in the equilibrium, and the later
    is the utility after the deviation.
    Furthermore, we have 
    \begin{align*}
        \valuefunc_i(\alloc_i) - \moneycost_i(\wealth_i\primed) - 
        \left(
        \valuefunc_i(\alloci\doubleprimed) - \moneycost_i(\wealth_i\doubleprimed)
        \right)
        &= 
        \moneycost_i(\wealth_i\doubleprimed)
        - 
        \moneycost_i(\wealth_i\primed)
        -
         \left(
         \valuefunc_i(\alloci\doubleprimed) - \valuefunc_i(\alloci)
         \right)
        \\
        &\overset{(a)}{\leq}
        \left(
        \wealth_i\doubleprimed - \wealth_i\primed
        \right)
        \cdot 
        \moneycostderivative_i(\wealth\doubleprimed)
        -
        \left(\alloci\doubleprimed - \alloci\right)
        \cdot 
         \valuefuncderivative_i(\alloci\doubleprimed)
         \\
         &\overset{}{\leq}
         \epsilon
         \cdot 
         \moneycostderivative_i(\price\alloc_i + \epsilon)
         - 
         \left(
         \frac{\alloci\cdot \price + \epsilon}{\price + \epsilon}
         -
         \alloci
         \right)
        \cdot 
         \valuefuncderivative_i(\alloci\doubleprimed)
         \\
         &=
         \epsilon
         \cdot 
         \moneycostderivative_i(\price\alloc_i + \epsilon)
         - 
         \epsilon\cdot
         \frac{1-\alloci}{\price + \epsilon}
        \cdot 
         \valuefuncderivative_i(\alloci\doubleprimed)
    \end{align*}
    where inequality~(a) holds since $\alloci\doubleprimed > \alloci$, valuation function $\valuefunc_i$
    is concave and differentiable,
    $\truewealth_i > \wealth_i\doubleprimed > \wealth_i\primed$,
    and 
    disutility of money $\moneycost_i$
    is convex and differentiable up to $\truewealth_i$.
    Combining with $\util_i - \util_i\doubleprimed \geq 0$,
    we have 
    \begin{align*}
        \alloc_i \geq 1 - \frac{\price + \epsilon}{\valuefuncderivative_i(\alloci\doubleprimed)}
        \moneycostderivative_i(\price\alloci+\epsilon)
    \end{align*}
    for all positive $\epsilon$ that is sufficiently small.
    Finally, letting $\epsilon$ go to zero
    finishes the proof.
\end{proof}

Now we are ready to prove \Cref{thm:single item concave value convex budget pure}.

\begin{proof}[Proof of \Cref{thm:single item concave value convex budget pure}]
    Fix an arbitrary Nash equilibrium $\eqlb$.
    Suppose $\allocs,\price$ are the allocation and per-unit price in the induced FPPE. 
    Let  
    $\mathbf\optalloc$ be the allocation in the optimal transferable welfare.
    We introduce the following partition $A_1\bigsqcup A_2\bigsqcup A_3$
    of agents based on $\allocs$, $\price$, and $\mathbf\optalloc$:
    \begin{align*}
        A_1 &\triangleq 
        \{i\in[n]: \alloci \cdot \price = \truewealth_i\}
        \\
        % A_2 &\triangleq
        % \{i\in[n]: i \not\in A_1
        % \land \valuefuncderivative_i(\optalloc_i) \leq \pricethreshold\cdot \price
        % \}
        A_2 &\triangleq
        \{i\in[n]: i \not\in A_1
        \land \optalloc_i \leq \alloci
        \}
        \\
        % A_3 &\triangleq
        % \{i\in[n]: i \not\in A_1
        % \land \valuefuncderivative_i(\optalloc_i) > \pricethreshold\cdot \price
        % \land \optalloc_i \leq \alloci
        % \}
        A_3 &\triangleq
        \{i\in[n]: i \not\in A_1
        \land \optalloc_i > \alloci
        \}
    \end{align*}
    In words, $A_1$ corresponds to every agent $i$ who exhausts her true budget $\truewealth_i$ in the equilibrium;
    and $A_2$, $A_3$ correspond to the remaining agents.
% 
    % For every agent $i\in A_4$, her allocation $\alloc_i$
    % is the equilibrium is at least 
    % \begin{align*}
    %     \alloci 
    %     % \overset{(a)}{\geq}
    %     % 1 - \frac{\price}{\valuefuncderivative_i(\alloci)}
    %     \overset{(a)}{\geq} 
    %     1 - \frac{\price}{\valuefuncderivative_i(\alloc_i)}
    %     \moneycostderivative_i(\price\alloci)
    %     \overset{(b)}{\geq}
    %     1 - \frac{1}{\pricethreshold}
    %     = 
    %     \frac{\pricethreshold - 1}{\pricethreshold}
    % \end{align*}
    % where inequality~(a) is guaranteed due to \Cref{lem:alloc lower bound single item concave value hard budget};
    % % inequality~(b) holds since $\optalloc_i > \alloci$
    % % and the concavity of valuation function $\valuefunc_i$;
    % and inequality~(b) is guaranteed since $\valuefuncderivative_i(\alloc_i) > \pricethreshold\cdot \price\moneycostderivative_i(\price\alloci)$.
% 
    Next, we compare the transferable welfare contribution from $A_1, A_2, A_3$ separately.

    \smallskip
    For every agent $i\in A_1$, note that 
    \begin{align*}
        \wtp_i(\optalloc_i) 
        \overset{(a)}{\leq} \truewealth_i
        \overset{(b)}{=}
        \wtp_i(\alloci)
    \end{align*}
    where the inequality holds due to the definition of $\wtp_i$;
    and the equality holds due to the definition of $A_1$.
    
    For every agent $i\in A_2$, note that 
    \begin{align*}
        \wtp_i(\optalloc_i) \leq \wtp_i(\alloci)
    \end{align*}
    where the inequality holds since $\optalloc_i \leq \alloci$ implied by the definition of $A_2$.

    For every agent $i\in A_3$, note that 
    \begin{align*}
        \wtp_i(\optalloc_i) 
        &\overset{(a)}{\leq} 
        \wtp_i(\alloci) + 
        \frac{
        \valuefunc_i(\optalloc_i) - \valuefunc_i(\alloci)
        }{
        \moneycostderivative_i(\wtp_i(\alloci))
        }
        \\
        &\overset{(b)}{\leq} 
         \wtp_i(\alloci) + 
        \frac{
        \valuefunc_i(\optalloc_i) - \valuefunc_i(\alloci)
        }{
        \moneycostderivative_i(\price\alloci)
        }
        \\
        &\overset{(c)}{\leq} 
         \wtp_i(\alloci) 
         + 
         (\optalloc_i - \alloci)
         \cdot \frac{\valuefuncderivative_i(\alloc_i)}{
         \moneycostderivative_i(\price\alloci)
         }
         \\
        &\overset{(d)}{\leq}
        \wtp_i(\alloci) + 
        (\optalloc_i - \alloci)
        \cdot 
        \frac{\price}{1-\alloci}
        \\
        &\overset{(e)}{\leq}
        \wtp_i(\alloci) + 
        \optalloc_i\price
    \end{align*}
    where inequality~(a) holds due to the definition of $\wtp_i$ and the convexity of $\moneycost_i$;
    inequality~(b) holds since 
    $\moneycostderivative_i$ is weakly increasing implied by
    the convexity of 
    $\moneycost_i$,
    and 
    $\wtp_i(\alloci) \geq \price\alloci$ which is implied by the definition of $\wtp_i$ and 
    the fact that 
    agent $i$'s utility is non-negative in the equilibrium allocation $\allocs$ and per-unit price $\price$;
    inequality~(c) holds due to the concavity of valuation function $\valuefunc_i$;
    inequality~(d) holds due to \Cref{lem:alloc lower bound single item concave value hard budget};
    and inequality~(e) holds 
    since $\frac{\optalloc_i - \alloci}{1-\alloci} \leq 
    \frac{\optalloc_i - \optalloc_i\alloci}{1-\alloci} = 
    \optalloc_i$.

    \smallskip
    Putting all pieces together, we have the following upper bound of
    the optimal transferable welfare $\wtp(\mathbf\optalloc)$,
    \begin{align*}
    % \label{eq:welfare upper bound single item concave value hard budget}
    \begin{split}
        \wtp(\mathbf\optalloc) 
        &= 
        \sum_{i\in[n]} \wtp_i(\optalloc_i)
        % \\
        \leq 
        \left(\sum_{i\in A_3} \optalloc_i
        \right)\cdot  \price 
        +
        \sum_{i\in A_1\sqcup A_2 \sqcup A_3}
        \wtp_i(\alloci)
        % \\
        \overset{(a)}{\leq} 
        \price 
        +
        \sum_{i\in A_1\sqcup A_2 \sqcup A_3}
        \wtp_i(\alloci)
        % \\
        \overset{(b)}{\leq} 
        2\wtp(\allocs)
        \end{split}
    \end{align*}
    where inequality~(a) holds since $\sum_{i\in A_3}\optalloc_i \leq 1$;
    and inequality~(b) holds since 
    $\price \leq \wtp(\allocs)$
    since all agents receive non-negative utility in the equilibrium allocation $\allocs$ and per-unit price $\price$.
\end{proof}

\begin{example}[Tightness of \Cref{thm:single item concave value convex budget pure}]
    Consider two exogenously-budgeted agents
    with linear valuation as follows:
    \begin{align*}
        \val_1 = K,
        \qquad 
        \truewealth_1 = 1,
        \qquad
        \val_2 = 1,
        \qquad
        \truewealth_2 = \infty
    \end{align*}
    where $K$ is a sufficiently large constant.
    The optimal transferable welfare is $(2 - 1/K)$
    by allocating agent $1$ with $\frac{1}{K}$-fraction 
    and allocating agent $2$ with $\frac{K-1}{K}$-fraction.
    Suppose both agents truthfully report
    their values and budgets, 
    the induced FPPE allocates the whole item to agent 1 with per-unit price 1,
    and thus achieves the transferable welfare of $1$.
    Finally, it can be straightforwardly verified that truthfully reporting forms a valid equilibrium in the metagame.
\end{example}


\begin{remark}
    The same PoA bound and analysis hold if we consider 
    the variant model where the agents have linear valuation function, and can only report budgets in the metagame.
\end{remark}

\begin{remark}
\label{remark:tight poa single item pure}
    In the single-item environment,
    our metagame is similar to the 
    classic \emph{Kelly mechanism}.\footnote{In Kelly mechanism, each agent submits a single bid $\wealth_i$, receives a fraction of the item
    proportional to her bid, 
    and pays her bids.}
    However, our metagame is not equivalent to the Kelly mechanism -- there exists 
    allocation and payment outcome in 
    the equilibrium of our metagame, which is not attainable in the equilibrium of the Kelly mechanism. 
    For example, consider two linear utility agents with values $10 > 1$, respectively.
    In our metagame, reporting 
    reporting $(\val_1 = 10, \wealth_1 = 1)$,
    $(\val_2 = 1, \wealth_2 = 1)$
    is a equilibrium with optimal (transferable) welfare. 
    In contrast, there exists no welfare-optimal equilibrium in the Kelly mechanism.
\end{remark}

\subsection{A $4$-approximation Analysis for Mixed Nash}

In this subsection, we present a $4$-approximation PoA guarantee 
for mixed Nash. 
% The analysis is inspired by \citet{CST-15b}.

\begin{theorem}
\label{thm:single item concave value convex budget mixed}
    In the single-item environment,
    for agents with (differentiable) concave valuation functions 
 $\{\valuefunc_i\}$ and 
 (differentiable) convex disutilities of money $\{\moneycost_i\}$
 up to heterogeneous budgets $\{\truewealth_i\}$,
    the mixed Nash PoA of transferable welfare 
    is at most $4$.
\end{theorem}

% \newcommand{\priceTilde}{\tilde\price}
% \newcommand{\tildeP}{\tilde P}

\begin{proof}
% [Proof of \Cref{thm:single item concave value convex budget mixed}]
   Fix an arbitrary mixed Nash equilibrium $\eqlb$.
    Suppose $\allocs,\price$ are the randomized allocation and per-unit price in the induced FPPE. 
    Let  
    $\mathbf\optalloc$ be the allocation in the optimal transferable welfare.    

    For each agent $i$, we present the following upper bound 
    of its contribution $\wtp_i(\optalloc_i)$ in the optimal transferable welfare allocation,
    \begin{align}
    \label{eq:single item mixed wtp bound}
        \frac{1}{2}\wtp_i(\optalloc_i) \leq 
        \moneycost_i^{-1}(\util_i) + 
        \optalloc_i \expect{\price}
    \end{align}
    where $\util_i$ is the expected utility of agent $i$ in the equilibrium $\eqlb$.
    Note that inequality~\eqref{eq:single item mixed wtp bound}
    immediately implies the lemma statement since
    \begin{align*}
        \wtp(\mathbf\optalloc) 
        = \sum_{i\in[n]}
        \wtp_i(\optalloc_i)
        \leq 
        2
        \left(
        \sum_{i\in[n]} 
        \moneycost_i^{-1}(\util_i)
        +
        \optalloc_i \expect{\price}
        \right)
        \leq 
        4\wtp(\allocs)
    \end{align*}
    where the last inequality holds since $\moneycost_i^{-1}(\util_i) \leq 
    \moneycost_i^{-1}(\expect{\val_i(\alloci)})
    \equiv
    \wtp_i(\alloci)$;
    $\expect{\price} \leq  \wtp(\allocs)$;
    and $\sum_{i\in[n]}\optalloc_i = 1$.

    Below we proof inequality~\eqref{eq:single item mixed wtp bound}
    by considering a specific deviation strategy for agent $i$.
    Let $\price\doubleprimed$ be the randomized per-unit price induced by the FPPE where agent $i$ is not participated, or equivalently, reporting $\wealth_i\doubleprimed = 0$.
    As a sanity check randomized price $\price\doubleprimed$ is first order stochastically dominated by randomized price $\price$.
    
    Let $\tildeP \triangleq \expect{\price\doubleprimed}$.
    % and $\event_2\triangleq \neg \event$ be its complement event.
    Now consider the following deviating strategy for agent $i$
    where agent $i$ deterministically reports 
    \begin{align*}
        \val_i\primed = \infty,\quad 
        \wealth_i\primed = 
        \optalloc_i \cdot 
        \tildeP
    \end{align*}
    Let $\allocs\primed,\price\primed$ be the randomized allocation and per-unit price in the induced FPPE after this deviation of agent $i$.
    Since agent $i$ reports $\val_i\primed = \infty$, 
    she always exhausts her reported budget $\wealth_i\primed$.
    
    In the remaining analysis,
    we couple the report profiles of all other agents except $i$ in the FPPE inducing randomized per-unit price $\price\doubleprimed$, and the FPPE inducing randomized 
    allocation~$\allocs\primed$ and per-unit price $\price\primed$.
    As a sanity check, 
    it is straightforward to verify that 
    \begin{align*}
        \price\doubleprimed \leq \price\primed
        \leq \price\doubleprimed + \wealth_i\primed
    \end{align*}
    and thus
    \begin{align*}
        \alloci\primed = 
        \frac{\wealth_i\primed}{\price\primed}
        \geq 
        \frac{\wealth_i\primed}{\price\doubleprimed + \wealth_i\primed}
    \end{align*}
    The expected utility $\util_i$
    of agent $i$ is at least her expected utility under this deviation,
    i.e., 
    \begin{align*}
        \util_i 
        &\geq 
        \expect
        [\alloci\primed]
        {
        \valuefunc_i\left(\alloci\primed\right)
        -
        \moneycost_i\left(\wealth_i\primed\right)}
        \\
        &\geq 
        \expect[\price\doubleprimed]{
        \valuefunc_i\left(
        \frac{\wealth_i\primed}{\priceTilde\doubleprimed
        +
        \wealth_i\primed
        }
        \right)}
        -
        \moneycost_i\left(\wealth_i\primed\right) 
        \\
        &= 
        \expect[\price\doubleprimed]{
        \valuefunc_i\left(
        \frac{\optalloc_i\tildeP}{\priceTilde\doubleprimed
        +
        \optalloc_i\tildeP
        }
        \right)}
        -
        \moneycost_i\left(\optalloc_i\tildeP\right) 
        \\
        &\overset{(a)}{\geq} 
        \expect[\price\doubleprimed]{
        \valuefunc_i\left(
        \frac{\optalloc_i\tildeP}{\price\doubleprimed
        +
        \tildeP
        }
        \right)}
        -
        \moneycost_i\left(\optalloc_i\tildeP\right) 
        \\
        &\overset{(b)}{\geq}
        \expect[\price\doubleprimed]{
        \frac{\tildeP}{\price\doubleprimed
        +
        \tildeP
        }
        \valuefunc_i\left(\optalloc_i
        \right)
        }
        -
        \moneycost_i\left(\optalloc_i\tildeP\right) 
        \\
        &\overset{(c)}{\geq} 
        \frac{\tildeP}{\expect[\price\doubleprimed]{\price
        \doubleprimed}
        +
        \tildeP
        }
        \valuefunc_i\left(\optalloc_i
        \right)
        -
        \moneycost_i\left(\optalloc_i\tildeP\right) 
        \\
        &= 
        \frac{1}{2}
        \valuefunc_i\left(\optalloc_i
        \right)
        -
        \moneycost_i\left(\optalloc_i\tildeP\right) 
    \end{align*}
    where inequality~(a) holds since $\optalloc_i \leq 1$;
    inequality~(b) holds due to the concavity of valuation function $\valuefunc_i$;
    and inequality~(c) holds since $\frac{\tildeP}{a + \tildeP}$ is convex in $a\geq 0$.

    Finally, applying concave function 
    $\moneycost_i^{-1}$ 
    to both side,
        we obtain
    \begin{align*}
        \frac{1}{2}\wtp_i(\optalloc_i) 
        &\leq 
        \moneycost_i^{-1}\left(\frac{1}{2}
        \valuefunc_i(\optalloc_i)\right)
        \leq 
        \moneycost_i^{-1}\left(
        \util_i + 
        \moneycost_i\left(\optalloc_i\tildeP\right)
        \right)
        \\
        &\leq 
        \moneycost_i^{-1}\left(
        \util_i  \right)
        +\optalloc_i\tildeP
        \leq 
        \moneycost_i^{-1}\left(
        \util_i  \right)
        +\optalloc_i\expect{\price}
    \end{align*}
    where the first and third inequality hold
    due to the convexity of $\moneycost_i$;
    the second inequality holds due to the monotonicity of $\moneycost_i$;
    and the last inequality holds since $\price$
    first order stochastically dominates $\price\doubleprimed$ and thus $\expect{\price}
    \geq \expect{\doubleprimed} \equiv \tildeP$.
\end{proof}

\begin{remark}
    The 4-approximation PoA analysis 
    can be extended to the setting where 
    agents have linear valuations, 
    and only reports budgets in the metagame.
    The main observation is that reporting value $\val_i = \infty$ weakly decreases 
    agent $i$'s utility compared with reporting $\val_i$.
\end{remark}

% We also present an improved PoA guarantee when agents 
% have concave valuations, and heterogeneous budgets.

% \begin{theorem}
% \label{thm:single item concave value hard budget mixed}
%     In the single-item environment,
%     for agents with (differentiable) concave valuation functions 
%  $\{\valuefunc_i\}$ and 
%   heterogeneous budgets $\{\truewealth_i\}$,
%     the mixed Nash PoA of transferable welfare 
%     is at most $\frac{\sqrt{5}+3}{2}\approx 2.618$.
% \end{theorem}

% Before the proof of \Cref{thm:single item concave value convex budget mixed} and \Cref{thm:single item concave value hard budget mixed},
% we first establish a lowerbound on 
% the transferable contribution
% for every agent $i$
% in an arbitrary mixed Nash equilibrium
% by constructing a specific deviation strategy.


==> Notes/summary.tex <==
\section{Summary of Prior Work and Results}

In this section, we summarize all 
results in prior work and results 
in this project.

\subsection{Single-item Environment}

\paragraph{Prior work on DSIC mechanisms}

\begin{theorem}[\citealp{abr-06,DP-14}]
    Linear-value, budgeted agents:
    the liquid welfare of 
    the market clearing price
    is a $2$-approximation.
\end{theorem}

\begin{theorem}[\citealp{DP-14}]
    Linear-value, budgeted agents:
    the liquid welfare of 
    the clinching auction
    is a $2$-approximation.
\end{theorem}


\begin{theorem}[\citealp{LX-15}]
    Linear-value, budgeted agents:
    the liquid welfare of 
    the random-sampling auction
    is at most $\frac{\sqrt{5}+1}{2}$-approximation.
\end{theorem}

\paragraph{Prior work on liquid welfare PoA}

\begin{theorem}[\citealp{CV-16,CST-15,CV-18}]
    Concave-value, budgeted agents:
    the mixed (resp.\ pure) 
    Nash PoA of 
    the Kelly mechanism is at most 2.618 (resp.\ 2).
\end{theorem}

\begin{theorem}[\citealp{CST-15}]
    Concave-value, budgeted agents:
    the Bayesian
    Nash PoA of 
    the Kelly mechanism is at most 2.618.
\end{theorem}

\begin{theorem}[\citealp{CV-18}]
    Concave-value, budgeted agents:
    for every resource allocation mechanism\footnote{A resource allocation mechanism is  
    a mapping from signals, aka., bids to 
    allocation and payment profiles.},
    there exists $n$ concave-value, budgeted agents such that 
    there exists pure Nash equilibrium whose 
    liquid welfare is at least a
    $2-\frac{1}{n}$-approximation.
\end{theorem}

\paragraph{Our new results}

\begin{theorem}[see~\Cref{thm:single item concave value convex budget pure} for the upper bound and \Cref{remark:tight poa single item pure} for the lower bound]
    Concave-value, convex-money-disutility 
    agents: the pure Nash PoA of
    the value-budget-reporting
    metagame
    is 2.
\end{theorem}

\begin{theorem}[see \Cref{thm:single item concave value convex budget mixed}]
    Concave-value, convex-money-disutility 
    agents: the mixed/Bayesian Nash PoA of
    the budget-reporting
    metagame
    is 4.
\end{theorem}

\Cref{thm:single item concave value convex budget pure} can be extended to $\epsilon$-Nash with an additional additive loss $O(nL\epsilon)$
where $L$ is the Lipschitz constant of $\valuefuncderivative$ and $\moneycostderivative$.
\Cref{thm:single item concave value convex budget mixed}
can be extended to $\epsilon$-Nash with an additional additive loss $O(n\epsilon)$
without dependence on $L$.


\begin{theorem}[see \Cref{lem:market clearing approx single item}]
    Convex-value, 
    convex-money-disutility
    agents:
    the transferable welfare of the market clearing price is a 2-approximation.
\end{theorem}

\begin{remark}
    There exists allocation profile induced by 
    the market clearing price that 
    cannot be induced in the metagame.
    For the simplest example, consider the single-agent instance.
\end{remark}

\subsection{Multi-item Environment}

\paragraph{Prior work on liquid welfare PoA}

\begin{theorem}[\citealp{CST-15}]
    Subadditive-value,\footnote{Additive-concave-value agents are the special case of subadditive-value agents.} quasi-linear agents:
    the mixed/Bayesian Nash PoA of the simultaneous Kelly mechanism is at most 2.
\end{theorem}

\begin{theorem}[\citealp{CST-15}]
    Subadditive-value, budgeted agents:
    the mixed Nash PoA of the simultaneous Kelly mechanism is at most 2.618.
\end{theorem}

\begin{theorem}[\citealp{AFGR-17}]
    Additive-linear-value, budgeted agents:
    the mixed Nash PoA of the 
    simultaneous first-price
    mechanism is at most 51.5 
    in the share model.\footnote{In the share model,
    each item is divided into sufficiently small pieces, and agents submit bid
    for each piece separately.}
\end{theorem}


\begin{theorem}[\citealp{AFGR-17}]
    Additive-linear-value, budgeted agents:
    the Bayesian Nash PoA of the 
    simultaneous first-price 
    mechanism 
    (resp.\ second-price with no over-bidding, no over-budgeting)
    is at most 51.5 
    in the share model.
\end{theorem}

\begin{theorem}[\citealp{AFGR-17}]
    Fractional-subadditive-value, budgeted agents:
    the pure Nash (with no over-bidding, no over-budgeting) PoA of the 
    simultaneous first-price
    mechanism with deterministic tie-breaking rule is at most 2
    in the inivisible-item model.
\end{theorem}

\begin{theorem}[\citealp{BCHNL-21}]
    Additive-linear-value, convex-money-disutility agents: 
    the ROI-optimal pure Nash PoA 
    of the simultaneous second-price auction
    is 2.
\end{theorem}

\paragraph{Our new results}

\begin{theorem}[see~\Cref{thm:multi item concave value convex budget pure} for the upper bound and \Cref{remark:tight poa single item pure} for the lower bound]
    Concave-value, convex-money-disutility 
    agents: the pure Nash PoA of
    the value-budget-reporting
    metagame
    is 2.
\end{theorem}

\begin{theorem}[see \Cref{thm:multi item concave value convex budget mixed}]
    Concave-value, convex-money-disutility 
    agents: the mixed/Bayesian Nash PoA of
    the budget-reporting
    metagame
    is 4.
\end{theorem}

\Cref{thm:multi item concave value convex budget pure} can be extended to $\epsilon$-Nash with an additional additive loss $O(nL\epsilon)$
where $L$ is the Lipschitz constant of $\valuefuncderivative$ and $\moneycostderivative$.
\Cref{thm:multi item concave value convex budget mixed}
can be extended to $\epsilon$-Nash with an additional additive loss $O(n\epsilon)$
without dependence on $L$.


\begin{theorem}[see \Cref{lem:mc 2 approx}]
    Additive-linear value, 
    convex-money-disutility
    agents:
    the transferable welfare of the market clearing price is a 2-approximation.
\end{theorem}

\subsection{Convergence to equilibrium}

\begin{theorem}[\citealp{NJR-11}]
    Concave-value, quasi-linear agents:
    the better response dynamics
    of the Kelly mechanism 
    converges to the equilibrium.
\end{theorem}

\begin{theorem}{\citealp{GPD-20}}
    Agents with monotone, Lipschitz smooth cost, and unconstrained action space: the optimistic gradient algorithm
    converges to the equilibrium.
\end{theorem}

In the single-item environment,
for the budget-reporting metagame
with linear value, Lipschitz smooth convex
money disutility agents,
we might be able to prove the assumptions 
required in \citet{GPD-20}.


\newpage

==> Notes/todo.tex <==
\section*{Todo}

==> Paper/PoA-results.tex <==
\label{sec:poa}

In this section, we present the main results of the paper: the price of anarchy (PoA) bound of our metagame. In \Cref{sec:poa pure}, we show the tight PoA bound under pure Nash equilibrium; while in \Cref{sec:poa mixed}, we present the PoA bound under mixed Nash equilibrium.


\subsection{Tight PoA Bound Under Pure Nash Equilibrium}
\label{sec:poa pure}
\input{Paper/PoA-pure}



\subsection{PoA Bound Under Mixed Nash Equilibrium}
\label{sec:poa mixed}
\input{Paper/PoA-mixed}

==> Paper/intro-OLD.tex <==
\label{sec:intro}


% Outline


In the ever-evolving landscape of digital advertising auctions, efficient and effective bidding strategies play a crucial role in optimizing the allocation of resources and maximizing returns on investments.  {Bid management is a complex and challenging task, with advertisers participating in many thousands of auctions that are strategically linked through a shared campaign budget.}  {To help alleviate this burden, nearly all advertising platforms now provide an \emph{autobidding} service that partially automates the bidding process.}
%, gaining significant attention due to its potential to automate the bidding process and improve campaign performance.
%By leveraging the power of algorithmic assistance and machine learning, a
An autobidder places bids on the advertisers' behalf, leveraging machine learning and other algorithmic techniques to tune bids in response to observed auction outcomes and other information from the platform such as  predictions of ad relevance and user intent. %values in real-time, taking into account various factors such as user behavior, ad relevance, and market dynamics.
Autobidding has had dramatic impact on the advertising industry: virtually all campaign spending now passes through some form of autobidder, and individual autobidding algorithms are in constant competition with each other to secure the most coveted ad placements.

The usual autobidding paradigm involves three distinct layers: advertisers, autobidders, and auctions for individual advertising events (e.g., impression, click, conversion, etc.).  See \Cref{fig:metagame} for an illustration.  Each advertiser has their own individual autobidding algorithm (often provided by the ad platform itself) %, which is a decentralized algorithm 
that bids on their behalf.
%advertiser's behalf.  
An advertiser provides their autobidder with instructions such as a specified budget and possibly a maximum bid, which is sometimes interpreted as a declared value per event.\footnote{\yfedit{In our model, the maximum bid constraint is equivalent to an aggregate return-of-investment (ROI) constraint, which is common in the autobidding literature.}}  These specifications serve as a mandate for the autobidder.
{The autobidder then participates in many individual auctions, %decentralized algorithms that bid on behalf of each advertiser, with the objective of
bidding to }
maximize the total value received (i.e., the total number of events) while adhering to the specified constraints.
%within the simultaneous auction.
The interplay between autobidders competing in the same auctions forms a budget-pacing game, where autobidders optimize their bidding strategies in response to competition. Recent research has made significant progress in studying this game,
%the budget-pacing game of autobidders,
establishing the existence of equilibria and characterizing their properties.

From the advertisers' perspective, the autobidder and
%simultaneous
per-event auction layers can be seen as a cohesive mechanism that the advertisers strategically interact with. The advertiser-specified constraints (e.g., budgets) define the mechanism's message space. While such message space is typically designed to be comprehensible and user-friendly, it does not necessarily capture the intricacies of advertiser preferences. Indeed, the latter may be much more complex than, e.g., maximizing a linear value for clicks or other events subject to a budget. (And even when the message space does capture advertisers' preferences, these mechanisms are, in general, not known to incentivize truth-telling.) In practice, advertisers frequently adjust these constraints, treating them simply as ``knobs" to be fine-tuned.

%However, it is crucial to acknowledge that these constraints may not always accurately reflect the true preferences of the advertisers. While a lack of incentive compatibility within the mechanism may be one factor, another significant driver stems from the advertisers themselves: the true preferences of advertisers may be much more complex than maximizing a linear value for clicks or other events subject to a budget.  Consequently, the message space of the mechanism is limited in its ability to fully capture the intricacies of advertiser preferences. This is evident as advertisers frequently adjust these specifications, suggesting that they are not primitive components of their preferences but instead are strategic knobs to be fine-tuned.

Thus, while the autobidders play a budget-pacing game amongst themselves, the advertisers play a game of constraint selection, henceforth called the \emph{metagame}. The actions in this metagame are the budgets and 
%maximum bids specified to the autobidders. (We also consider an extension with no maximum bid.) 
any other constraints specified to the autobidders.
These constraints in turn define a budget-pacing game,
%that the autobidders will play. The equilibrium of the inner game ultimately determines the advertisers' payoffs.
called the \emph{inner game}, where the autobidders compete with each other to maximize the total value (i.e., number of events obtained) subject to the specified constraints. The outcome of the inner game
ultimately determines the advertisers' payoffs. In this paper, we focus on the metagame played by the advertisers, explore its equilibrium outcomes, 
%we aim to explore the equilibrium outcomes of the metagame played by advertisers
and shed light on the efficiency of the overall market.


\begin{figure}
    \centering
    \input{figs/fig-metagame}
    \caption{The metagame of strategic budget selection.}
    \label{fig:metagame}
\end{figure}


%\subsection{Our Contributions.}
%To study the strategic behavior of advertisers in the autobidding paradigm, we
%%introduce a novel game-theoretic model --
%{consider} a \emph{metagame of strategic budget selection}.
%%\blcomment{I softened the language of the previous sentence, since the EC'23 paper also treats budget selection as strategic. But we should still highlight the novelty of our model with advertiser utilities being distinct from the mechanism message space, which is completely novel.}
%In this metagame, each advertiser \emph{strategically} declares a budget constraint (and possibly a maximum bid) to their autobidder. The chosen constraints define an ``inner'' budget-pacing game for the autobidders, who compete with each other to maximize the total value (i.e., number of events obtained) subject to the constraints. Advertiser payoffs in the original metagame are then determined by the equilibrium reached by the autobidders. Below we discuss and highlight a few details of our metagame.

\xhdr{Our model.}
First, we need to specify the outcome of the inner game. One challenge is the multiplicity of equilibria therein: indeed, advertisers' payoffs in the metagame are easily unspecified and possibly depend on the inner game dynamics. Fortunately, for the first-price auction, the equilibrium of the inner game is essentially unique, known as the \emph{first-price pacing equilibrium (FPPE)} \citep{CKPSSSW-22}, \bledit{and it is known that broad classes of simple learning dynamics will converge quickly to this equilibrium \citep{CJNKOM-07}}. Given that and the practical prevalence of the first-price auction in the digital advertising market, we will focus on first-price auctions and use FPPE as the unique outcome of the inner game.
\footnote{In contrast, for second-price auctions the equilibrium of the inner game
%it is known that the equilibrium of the budget-pacing game in the second-price auction
may not be unique \citep{CKSS-22}. Therefore,
extending our model to second-price auctions necessitates taking a stance on equilibrium selection,
%to extend our model from the first-price auction context to the second-price context, a stance on equilibrium selection of the inner game is necessary,
which we leave for future work.}



%\xhdr{First-price auction and inner game equilibrium uniqueness.}
%One potential challenge that arises is the possibility of non-uniqueness of equilibrium in the inner game.  When there are multiple equilibria in the inner budget-pacing game, the payoff of the advertisers in the metagame becomes underspecified. Fortunately, for first-price auctions the equilibrium of the budget-pacing game is essentially unique, and is known as the \emph{first-price pacing equilibrium (FPPE)} \citep{CKPSSSW-22}. Given the desired theoretical properties of FPPE and the practical prevalence of the first-price auction in the digital advertising market, we will focus on first-price auctions and use FPPE as the unique outcome of the autobidders to determine the payoff of the advertisers.\footnote{In contrast, it is known that the equilibrium of the budget-pacing game in the second-price auction may not be unique \citep{CKSS-22}. Therefore, to extend our model from the first-price auction context to the second-price context, a stance on equilibrium selection of the inner game is necessary, which we leave for future work.}
%See \Cref{fig:metagame}.
%%for a graphical illustration of our model.  %\blcomment{Not sure what figure is intended here.}

%\xhdr{Advertisers with general utility models.}
Our model encompasses a broad range of advertiser preferences.
We consider general \emph{separable} utility models
%that incorporates concave increasing
with a weakly concave (not necessarily linear) valuation for events (e.g., clicks) and weakly convex increasing disutility for spending money.
%This formulation includes the case of
This includes quasi-linear utility up to a hard budget constraint, but also allows
%. But it also allows
soft budget constraints, decreasing marginal value for clicks, etc.
We emphasize the mismatch in preferences: while the autobidders strive to maximize value given the specified constraints, the advertisers maximize utility given their more general preferences.

%We emphasize that while the advertiser utility model is general, they must declare a linear value (i.e., maximum bid) and a hard budget constraint to their autobidders, which may not perfectly capture their true preferences. Furthermore, while autobidders function as \emph{value-maximizers}, designed to maximize the total value received while adhering to the specified constraints, advertisers are \emph{utility-maximizers} based on their true preferences.

% \asmargincomment{moved here}
To measure the efficiency of the overall market, we focus on the \emph{liquid welfare}, which is the summation of each advertiser's willingness-to-pay given her own type and allocation. This general definition
%Our general definition of liquid welfare
encompasses the classic definition of welfare for linear agents and the original definition of liquid welfare for budgeted agents, respectively \citep{vic-61,DP-14}. Liquid welfare is also closely related to \emph{compensating variation} from economics \citep{hic-75}.%
\footnote{\label{footnote:compensating variation}Compensating variation is the transfer of money required, after some market change, to return agents to their original utility levels.  In our scenario, the ``change" is an allocation of resources, and the compensating variation is the maximum amount the agents would pay for their allocations; i.e., the liquid welfare.}
Given the advertisers' types, the liquid welfare is determined by the allocation; in our results, we compare to the optimal liquid welfare achieved by \emph{any} allocation, henceforth called the \OPT.

\xhdr{Our results: approximate efficiency in the metagame.}
In our baseline model, we consider a full-information environment where each advertiser's type (i.e., valuation and disutility for spending money) is fixed and publicly known. We consider both pure and mixed Nash equilibria: the advertisers simultaneously declare their constraints to their respective autobidders (deterministically for pure Nash or randomly for mixed Nash),
%each advertiser deterministically (for pure) or randomly (for mixed) declares constraints to their autobidder simultaneously,
then outcomes and payoffs are determined by the FPPE of the inner game.
%the inner FPPE of the autobidders.


As the main results of this paper, we show that at any pure Nash equilibrium (if one exists), the resulting liquid welfare is a 2-approximation to the
$\OPT$
%optimal liquid welfare
and this is tight.\footnote{We say that liquid welfare at equilibrium is an $\alpha$-approximation to the \OPT, for some approximation factor $\alpha\geq 1$, if the liquid welfare is at least $\OPT/\alpha$ for any vector of advertiser types.}
Moreover, at any mixed Nash equilibrium (which is guaranteed to exist), the resulting liquid welfare is at most a 4-approximation to the
\OPT.
%optimal liquid welfare.

We also consider an extension of our model to Bayesian environments, where each advertiser's type is independently drawn from a prior.
%type distribution independently.
We generalize our analysis for the mixed Nash equilibrium in the full information environments. Specifically, we show that at any Bayesian Nash equilibrium, the resulting liquid welfare is at most a 4-approximation to the expected \OPT.
%optimal liquid welfare.

\yfcomment{Placeholder: mention new pure Nash characterization for single-item instances.}

%At a high level, the intuition behind our approximation
\xhdr{Summary of Techniques.}
The intuition behind our liquid welfare approximation results is as follows.  At a pure Nash equilibrium, each advertiser will face a Pareto curve that represents the relationship between the value she receives and the budget constraint she declares to her autobidder. Increasing the declared budget allows the advertiser to win more, but at a potentially decreasing bang-per-buck.  %Ideally, we would like to show that this tradeoff is not too extreme, so each advertiser has a choice of budget that achieves high welfare without suffering too high a payment.  
The first step of our analysis is to analyze this tradeoff. 
%Roughly, we aim to show that 
%
{
To that end, we will employ a useful interpretation of FPPE due to~\citet{CKPSSSW-22}: the inner FPPE of autobidders corresponds to a market-clearing outcome that assigns a price to each impression, so that each autobidder obtains a preferred bundle under those prices.
}
%We would like to say that each advertiser can provide her autobidder with enough budget to obtain a high-welfare bundle.
Since increasing one autobidder's budget has downstream effects on how other autobidders will behave (even keeping the reports of other advertisers fixed), adjusting one's budget can cause the market-clearing prices to change.
%; see \Cref{lem:fppe increasing budget}.
{
This gives us the perspective we need to understand an advertiser's tradeoff when choosing a budget: the sensitivity of FPPE prices and market-clearing allocations to budget changes.
}

{
Unfortunately, this sensitivity can be unbounded in general: an advertiser might need to increase their spend by an arbitrary amount to secure a given increase in allocation.
}
%For example, consider two advertisers competing for a single item.  If the advertisers set infinitely high values but finite budgets, then at FPPE they will spend their budgets exactly and split the item in proportion to their declared budgets.  (See Section~\ref{sec:example} for examples and intuition for FPPE.)  This means that if the first advertiser sets a budget of $1$, the second advertiser would need 
But we show that this only occurs when an advertiser's allocation is already high.
As long as an advertiser is not winning an excessive share of the impressions, the market-clearing prices faced by her autobidder will not be overly sensitive to changes in her allocation.  This is our main technical lemma, Lemma~\ref{lem:poa pure allocation price relation}, which relates the rate of substitution between valuation utility and payment disutility of an advertiser at equilibrium to the FPPE prices and the share of each impression she obtains.  It implies that if an advertiser is obtaining significantly less value than she would in the optimal allocation, then either (a) the prices are low and her allocation is small, in which case by Lemma~\ref{lem:poa pure allocation price relation} she can improve her utility by increasing her budget (contradicting the equilibrium assumption), or (b) her autobidder must be facing high market-clearing prices. But in the latter case, we can employ a standard trick for bounding the price of anarchy: the lost welfare from the advertiser can be charged against revenue collected from the other advertisers who are paying these high prices. {Here we use the fact that since liquid welfare measures total willingness to pay, the revenue collected is always a lower bound on liquid welfare.}  Putting these pieces together yields our $2$-approximation result for pure Nash equilibrium.

{
The extension to mixed (and Bayesian) Nash equilibrium requires a slightly different approach.  Since the messages (and hence outcomes and prices) may be random, it is less straightforward to characterize each advertiser's tradeoff between allocation and spend.  So instead of quantifying that tradeoff precisely, we consider a specific budget-setting strategy that each agent will consider.  Namely, each advertiser considers the \emph{expected} FPPE market-clearing prices (over the reports of others) that would be obtained \emph{if she were not present in the market}.  She then calculates the expected cost of her expected optimal allocation under this price distribution; this will be the deviating budget she considers.  We show that if an advertiser is receiving low expected value at equilibrium and the FPPE prices are low in expectation, this deviation will be utility-improving, a contradiction.  A low-value advertiser must therefore be facing high expected prices, and we can once again charge any shortfall of liquid welfare to the revenue generated by those high prices.
}

\xhdr{Practical interpretations.} Our theoretical results highlight an important practical implication:
\begin{displayquote}
\emph{Simple instructions for autobidders are sufficient to achieve good market outcomes even when advertisers have much more complex preferences.}
\end{displayquote}
An interesting follow-up question arises: Can these instructions be further simplified? Specifically, are hard budget or maximum bid necessary constraints for the autobidder? To answer this question, we study variants of the metagame where advertisers exclusively declare budget constraints or maximum bid constraints, respectively.
%Our analysis for these variants demonstrates that the hard
We demonstrate that the budget constraints are crucial. If advertisers exclusively specify maximum bids but not budgets, the resulting approximation factor at equilibrium can be as bad as linear in the number of advertisers. On the other hand, all our approximation results extend to the variant of the metagame with no maximum bid.
%where advertisers exclusively declare hard budgets but not maximum bids.
Intuitively, the presence of budgets allows advertisers to hedge against unexpectedly high expenditures, which can have a potentially catastrophic impact on their utility. 

\xhdr{Organization.} We start by formalizing the model and providing necessary preliminaries and
notations in \Cref{sec:prelim}. In \Cref{sec:example} we study two simple examples and analyze their pure Nash equilibrium in the metagame. In \Cref{sec:poa pure,sec:poa mixed}, we present the approximation results of the liquid welfare at equilibrium. Finally, we study the extension of our model in the Bayesian environments in \Cref{sec:bayesian}, and several variants of our model under restrictive message space (i.e., advertisers can only exclusively declare hard budgets, or maximum bids) in \Cref{sec:value/budget reporting only}.
\yfcomment{Placeholder: mention new pure Nash characterization for single-item instances.}

\subsection{Related Work}

\paragraph{Autobidding in auctions.} There is a rapidly growing literature on autobidding. %One of the earliest works in this line is
An early work of
\citet{Borgs-www07} studied budget-management algorithms for first- and second-price auctions and showed convergence for the case of first-price auctions.  \citet{balseiro2019learning} analyze a budget-pacing method based on gradient descent for second-price auctions, leading to
%and this has opened a
rich literature on the design of autobidding algorithms for budget management with desirable regret and convergence properties~\citep{balseiro2017budget,balseiro2020dual,balseiro2023best,castiglioni2022unifying} and how a platform might design its auction rules or prices for such algorithms~\citep{balseiro2021robust,deng2021towards,golrezaei2023pricing}.  In contrast, we abstract away from the learning process and directly study the equilibria between autobidders in our inner budget-pacing game for a fixed auction format.
%
%A mathematical formulation for equilibrium obtained by autobidders is given in \citet{ABM-19}, who bounded the liquid welfare obtained at equilibrium under a general form of constraints.
In this sense, our model of autobidders is closest to the one in  \citet{CKPSSSW-22}. This paper introduces the first-price pacing equilibrium (FPPE), a solution concept for autobidders in the first-price auction whose goal is to maximize the total values received subject to the budget and maximum bid constraints. Crucially, FPPE is proved to be unique and polynomial-time computable. \citet{CKSS-22} introduce the second-price pacing equilibrium (SPPE), a similar concept for the second-price auctions. Unlike FPPE, SPPE is not unique and PPAD-Hard to compute in general \citep{CKSS-22,CKK-21}.  Nevertheless, \citet{ABM-19} show that any
SPPE
%equilibrium
will result in approximately optimal liquid welfare, under budget and/or return-on-investment constraints.
%a rich class of (possibly multiple) constraints including budget constraints.

A recent line of work has studied the incentives of value-maximizing advertisers to truthfully describe their preferences to their autobidders. \citet{MP-23} show that the advertisers may benefit by misreporting their preference to autobidders when the platform does not have commitment power and can change the auction rule. \citet{LT-22} conduct an empirical investigation using numerical examples, illustrating the potential advantages for advertisers when misreporting to autobidders in a second-price auction.  Conceptually closest to our work is \citet{AMP-23}, who introduce the concept of auto-bidding incentive compatibility (AIC)
%. They establish that the second-price auction, truthful auction, and first-price auction are not AIC, whereas
and show that first-price auction with uniform bidding satisfies AIC (while many other auction formats do not).
%It is important to emphasize the the significant distinctions between our work and \citet{AMP-23}.
Crucially, all of these works assume that both advertisers and their autobidders are value-maximizers with similar constraints, so the advertisers are able to declare their true preferences to their autobidders.  In contrast, in our model the advertisers are utility-maximizers and they can only give their autobidders simple constraints (hard budget, maximum bid) that may not be rich enough to capture their true complex preferences.  In particular, the induced mechanism is not direct-revelation and hence incentive compatibility does not apply; we focus instead on Nash equilibria.
%so we focus instead on equilibria of constraint-selection.
%The resulting mechanism is therefore not a direct revelation , and we study the equilibria of the resulting game.
%This separation between advertiser utilities and the message space of the autobidding mechanism is a primary feature of our model.
%with a general class of utility model, and they can only declares simple constraints (hard budget, maximum bid) to their autobidders, which not necessary capture their true complex preference. In other words, AIC is not well-defined in our model. Finally, our paper also investigates the approximate efficiency of overall markets.

\xhdr{Metagame between no-regret learning agents.}
\citet{KN-22a} explores the concept of a metagame involving rational agents who utilize regret-minimizing learning algorithms to play games on their behalf,
%Unlike our model where advertisers with complex preferences have a simple message space that may not capture their true preferences, the model of \citet{KN-22a} assumes that the message space encompasses all possible preferences. The focus of \citet{KN-22a} is investigating
and investigates
whether the agents
%of these learning algorithms have incentives
are incentivized
to manipulate or misrepresent their true preferences in various classic games.
In \citet{KN-22b}, the authors delve into a similar problem but within the context of auctions involving two agents with linear utility, %Specifically, they show the incentive for
showing that agents have incentive to misreport their true values in a second-price auction when both agents use multiplicative-weights learning algorithms. On the other hand, they find that truthful reporting forms a Nash equilibrium in the first-price auction when both agents use mean-based learning algorithms.
Compared to both \citet{KN-22a} and \citet{KN-22b}, this present paper considers a different auction setup with budget constraints, focuses on cases where advertiser preferences and autobidder instructions are different, and abstracts away from the learning process by assuming that the autobidders converge to bidding according to an FPPE of the simultaneous auction game. 
%and focuses on the case where advertiser preferences are more complex than the space of allowable instructions to autobidders.
%, and we analyze equilibria of the resulting game.
%has a distinct characteristic in the metagame: advertisers with complex preferences have a simple message space that may not capture their true preferences. Furthermore, our paper considers a more general auction setup with a general number of agents and heterogeneous items, in contrast to \citet{KN-22b} which primarily focuses on auctions involving two agents and identical items.
%Lastly, our paper also investigates the approximate efficiency of overall markets.

\xhdr{Price of anarchy for non-quasi linear agents} There is a long line of literature about the price of anarchy (PoA) -- the approximation between worst equilibrium and best outcome -- in the context of liquid welfare for non-quasi linear agents. Besides works already mentioned above, \citet{DP-14} introduce the concept of liquid welfare for agents with hard budget constraints. They prove the PoA for posting market clearing prices and the clinching auction. \citet{LX-15} design a sampling mechanism with a better PoA guarantee. All mechanisms studied in \citet{DP-14,LX-15} are truthful mechanisms. For non-truthful mechanisms, \citet{CST-15,CV-16,CV-18} study the PoA of the simultaneous Kelly mechanism, while \citet{AFGR-17} studies the PoA of the simultaneous first-price auction and second-price auction with no over-bidding. \citet{BCHNL-21} studies the PoA under ROI-optimal pure Nash equilibrium of the simultaneous second price auction, establishing a $2$-approximation and that such a pure Nash equilibrium always exists. \citet{ABM-19,LMP-22,meh-22,deng2022efficiency} study the PoA for the autobidders under various auctions. \citet{FT-23,GLLLS-23,LPSZ-23} study the dynamic of no-regret learning/budget-pacing players (autobidders) and provide the liquid welfare guarantees. It is important to highlight that
%previous research on autobidding has neglected the strategic behavior of
these works treat the autobidder constraints as exogenous and do not model them as strategic choices, focusing rather on the auction and autobidders' interaction. Additionally, except \citet{BCHNL-21}, the aforementioned studies assume that agents have a linear disutility for spending money up to a fixed budget. In contrast, our paper (like \citealp{BCHNL-21}) considers agents with a general convex disutility function for spending money with a hard budget.



==> Paper/prelim-old.tex <==
\label{sec:prelim}

\newcommand{\alloci}{\alloc_i}
\newcommand{\paymenti}{\price_i}
\newcommand{\randomalloc}{\mathbf{x}}
\newcommand{\randomallocs}{{\randomalloc}}
\newcommand{\randomalloci}{\randomallocs_i}
\newcommand{\randompayment}{\mathbf{p}}
\newcommand{\randompaymenti}{\randompayment_i}
\newcommand{\valuefuncderivativei}{\valuefuncderivative_i}
\newcommand{\valuefunctionderivativei}{\valuefuncderivative_i}
\newcommand{\moneycostderivativei}{\moneycostderivative_i}
\newcommand{\payment}{p}
\newcommand{\reportval}{\tilde\val}
\newcommand{\reportwealth}{\tilde\wealth}
\newcommand{\randomreportval}{\tilde{\mathbf\val}}
\newcommand{\randomreportwealth}{\tilde{\mathbf\wealth}}
\newcommand{\realsinf}{\reals_+^{\infty}}
\newcommand{\strategy}{\mathbf{s}}
\newcommand{\valuefunction}{\valuefunc}
\newcommand{\PoA}{\Gamma}
\newcommand{\purePoA}{\PoA_{\texttt{Pure}}}
\newcommand{\mixedPoA}{\PoA_{\texttt{Mixed}}}
\newcommand{\BayesPoA}{\PoA_{\texttt{Bayes}}}
\newcommand{\instances}{\mathcal{\instance}}
\newcommand{\typedist}{F}

\paragraph{Agent models.}
There are $n$ agents (advertisers),
and $m$ divisible items (impressions).
The outcome for agent $i$ is 
$(\alloci, \paymenti)$,
where $\alloci = (\alloc_{i1}, \dots, \alloc_{im})
\in [0, 1]^m$
is the allocation for each item $j$ and 
$\paymenti\in\reals_+$ is the payment.
Agent $i$'s utility model is 
defined as 
$(\ctri, \valuefunctioni, 
\truewealthi, \moneycosti)$:
Given outcome $(\alloci,
\paymenti)$,
agent $i$'s utility $\util_i(\alloci,\paymenti)$
is 
\begin{align*}
    \util_i(\alloci,\paymenti)
    \triangleq 
    \left\{
    \begin{array}{ll}
    \valuefunctioni\left(
    \sum_{j\in[m]} 
    \ctrij\allocij\right)
     -
    \moneycosti\left(\paymenti\right)& 
    \quad \text{if } \paymenti \leq \truewealthi\\
    -\infty     & 
     \quad \text{if } \paymenti > \truewealthi
    \end{array}
    \right.
\end{align*}
Here $\ctri = (\ctr_{i1}, \dots \ctr_{im})\in\reals_+^m$
where $\ctrij$
is the \emph{click-through rate}
of each item $j$;
$\valuefunctioni:\reals_+\rightarrow \reals_+$
is the \emph{valuation function}
mapping from the total number of received clicks 
to agent's valuation;
$\truewealthi\in \realsinf$
is the \emph{hard budget};\footnote{We use notation $\realsinf$
to denote the set of all non-negative real numbers and infinite,
i.e., $\realsinf = \reals_+ \cup \{\infty\}$.}
and 
$\moneycosti:\reals_+ \rightarrow\reals_+$
is the \emph{money cost function}
mapping from the payment to its impact in 
the
agent's utility.\footnote{An interpretation of 
money cost function $\moneycosti$ is as follows:
Agent $i$ has an outside option value for her money,
e.g., spending on another advertising platform.
In this case, $\moneycosti(\paymenti)$
is the utility hat buyer $i$ foregoes by paying 
$\paymenti$ to the current advertising platform (seller).}
We assume $\valuefunctioni$
is differentiable, 
weakly concave, and weakly increasing;
and money cost function 
$\moneycosti$
is differentiable, 
weakly convex,
and weakly increasing.
We write $\valuefunctionderivativei(\sum_j\ctrij\allocij)$
and 
$\moneycostderivativei(\paymenti)$
as the derivative of $\valuefunctioni$
and $\moneycosti$
at $\sum_j\ctrij\allocij$
and $\paymenti$, respectively.

Besides the general utility model defined above, we also highlight that 
two classic utility models as special cases of the general one.
\begin{enumerate}
    \item \textsl{(linear utility)} 
    An agent $i$ with linear utility $(\ctri, \vali)$, hereafter 
    \emph{linear agent},
    has
    click-through rate $\ctri\in\reals_+^m$,
    linear valuation function 
    $\valuefunctioni(\sum_{j}\ctrij\allocij) 
    = \val_i\cdot \sum_{j}\ctrij\allocij$
    where $\val_i$ is her \emph{value per click},
    no hard budget (i.e., $\truewealthi = \infty$),
    and identity money cost function $\moneycosti(\paymenti) = \paymenti$.

    \item \textsl{(budgeted utility)} 
    An agent $i$ with budgeted utility $(\ctri, \vali, \truewealthi)$, hereafter 
    \emph{budgeted agent},
    has
    click-through rate $\ctri\in\reals_+^m$,
    linear valuation function 
    $\valuefunctioni(\sum_{j}\ctrij\allocij) 
    = \val_i\cdot \sum_{j}\ctrij\allocij$
    where $\val_i$ is her \emph{value per click},
    hard budget $\truewealthi$,
    and identity money cost function $\moneycosti(\paymenti) = \paymenti$.
\end{enumerate}


\paragraph{First-price pacing equilibrium for budgeted agents}
Before presenting the mechanism studied in this paper for agents 
with general utility models,
we first revisit the \emph{first-price pacing equilibrium}
introduced in \citet{CKPSSSW-22}
for budgeted agents.

\begin{definition}[First-price pacing equilibrium]
For budgeted agents with $\{(\ctri, \val_i, \truewealth_i)\}_{i\in[n]}$,
a \emph{first-price pacing equilibrium (FPPE)}
is a tuple $(\alloc, \price)$ of 
allocation $\alloci\in[0,1]^m$ for each 
agent $i$,
and per-unit price $\pricej\in \reals_+$
for each item $j$ 
that satisfies the following properties
\begin{enumerate}
    \item \textsl{(highest bang-per-buck)} if $\allocij > 0$, then $j \in \argmax_{j'\in[m]}\frac{\val_i\ctr_{ij'}}{\price_{j'}}$
    and $\max_{j'\in[m]}\frac{\val_i\ctr_{ij'}}{\price_{j'}}\leq 1$;
    \item \textsl{(supply feasibility)} $\sum_{i\in[n]}\allocij \leq 1$
    and equality holds if $\pricej > 0$;
    \item \textsl{(budget feasibility)} $\sum_{j\in[m]}\allocij\pricej \leq \truewealthi$
    and the equality holds if $\max_{j\in[m]}\frac{\val_i\ctr_{ij}}{\pricej} < 1$.
\end{enumerate}
\end{definition}

The allocation and payment in FPPE can be interpreted as follows:
Each budgeted agent $i$ first
decides a \emph{pacing scalar $\pacescalar_i = \min
\left\{
\max_{j'\in[m]}\frac{\vali\ctr_{ij'}}{\price_{j'}}, 1\right\}\in[0, 1]
$},
and submits bid $\pacescalar_i\vali\ctrij$ for each item $j$.
Then the allocation is the highest-bids-win
and the payment is computed under the first-price format.
The FPPE has been studied as a natural allocation and payment
outcome for budgeted agents in the digital advertising market \citep{CKPSSSW-22}.
In particular, the FPPE is 
One desired property of FPPE is its theoretical
existence and uniqueness.

\begin{lemma}[\citealp{CKPSSSW-22}]
    For any set of budgeted agents,
    FPPE exists.
    The per-unit prices and utilities of budgeted agents are unique.
\end{lemma}

To illustrate FPPE, we present the following two examples.
Both examples will also be used to illustrate our main model in 
XYZ as well.
\begin{example}[Two linear agents and single item]
    There are two linear agents and one item. Suppose click-through rate $\ctr_{11} = \ctr_{21} = 1$ and value per click $\val_1 \geq \val_2$.
    In FPPE, the unique per-unit price of the item is $\price_1 = \val_1$.
    If $\val_1 > \val_2$,
    the allocation in FPPE is unique as
    $\alloc_{11} = 1, \alloc_{21} = 0$.
    If $\val_1 > \val_2$,
    any $\alloc_{11}, \alloc_{21}\in[0, 1]$ such that $\alloc_{11}+\alloc_{21} = 1$
    together with unique per-unit price $\price_1$ forms a FPPE.
\end{example}

\begin{example}[Two budgeted agents and two items]
    There are two budgeted agents and two items. Suppose click-through rate
    $\ctr_{ij} = \frac{1}{2} + \frac{1}{2}\indicator{i=j}$
    for each $i\in[2],j\in[2]$;
    value per click $\val_1 = \val_2 = 1$;
    and budget $\truewealth_1 = \truewealth_2 = \frac{1}{2}$.
    In FPPE, both per-unit price and allocation are unique:
    $\price_1 = \price_2 = \frac{1}{2}$ and 
    $\allocij = \indicator{i = j}$ for each $i\in[2], j\in[2]$,
    i.e., both agents get their favorite items.
\end{example}

\paragraph{Metagame of budgeted utility reporting for general agents}
For agents with general utility models, 
we consider the following \emph{metagame of budgeted utility reporting}
motivated by the digital advertising market:
Each agent $i$ decides on a message $(\reportval_i, \reportwealth_i) \in (\realsinf)^2$
reported to the seller (platform).\footnote{Throughout the paper, 
we use notation $\tilde{}$ to denote the budgeted utility model which agent report to the seller.}
Given a message profile
$\{(\reportval_i, \reportwealth_i)\}_{i\in[n]}$,
the seller implements
the allocation $\alloc$ and payment $\payment$ 
induced by the FPPE
assuming each agent $i$ has 
a budgeted utility with 
click-through rate $\ctri$,
value per click as $\reportval_i$
and 
hard budget $\reportwealth_i$.
Going forward, we will simplify the metagame of budgeted utility reporting
as \emph{metagame}, and the induced FPPE given a message profile as \emph{inner FPPE}.

An interpretation of the metagame is as follows.
In the digital advertising market, a platform has a set of $n$ advertisers (agents)
and $m$ impressions (items).
The platform knows the click-through rate $\ctrij$ for each pair of advertiser $i$ and impression $j$. 
However, the platform does not know all other parameters in
the general utility model $\{(\ctri, \valuefunctioni, \truewealthi, \moneycosti)\}_{i\in[n]}$ 
of the advertisers.
Hence,
the platform pretends each advertiser 
as if she has a budgeted utility, 
asks her to report her value per click as well as her hard budget,
and then implements the allocation and payment 
induced by FPPE given advertisers' reports.



\paragraph{Solution concepts.}
With slight abuse of notations, we use $\util_i(\reportval_i, \reportwealth_i, \reportval_{-i}, \reportwealth_{-i})$ to denote the utility 
of agent $i$ in the metagame when agent $i$ reports message
$(\reportval_i, \reportwealth_i)$ and other agents report message 
$(\reportval_{-i}, \reportwealth_{-i}) \triangleq 
\{(\reportval_{i'}, \reportwealth_{i'})\}_{i'\in[n]\backslash\{i\}}$.\footnote{
Similarly, we use notation $-i$ to denotes other $n-1$ agents excluding agent $i$.}
In this paper, we are interested in the \emph{pure Nash equilibrium} and 
\emph{mixed Nash equilibrium}
for the metagame where agents' utility models 
$\{(\ctri, \valuefunctioni, \truewealthi, \moneycosti)\}_{i\in[n]}$
are fixed.

\begin{definition}[Pure Nash equilibrium]
    For agents with utility models $\{(\ctri, \valuefunctioni, \truewealthi, \moneycosti)\}_{i\in[n]}$,
    a \emph{pure Nash equilibrium} is a message profile 
    $\{(\reportval_i, \reportwealth_i)\}_{i\in[n]}\in (\realsinf)^{2n}$ such that
    for every agent $i\in[n]$ and every
    message $(\reportval_i\primed, \reportwealth_i\primed)\in (\realsinf)^2$,
    \begin{align*}
        \util_i(\reportval_i, \reportwealth_i, \reportval_{-i}, \reportwealth_{-i})
        \geq
        \util_i(\reportval_i\primed, \reportwealth_i\primed, \reportval_{-i}, \reportwealth_{-i})
    \end{align*}
\end{definition}
\begin{definition}[Mixed Nash equilibrium]
    For agents with utility models $\{(\ctri, \valuefunctioni, \truewealthi, \moneycosti)\}_{i\in[n]}$,
    a \emph{mixed Nash equilibrium} is a product distribution of message profile
    $\{(\randomreportval_i, \randomreportwealth_i)\}_{i\in[n]}\in \prod_{i\in[n]}
    \Delta((\realsinf)^2)$
    such that 
    for every agent $i\in[n]$ and every message
    $(\reportval_i\primed, \reportwealth_i\primed)\in (\realsinf)^2$,
    \begin{align*}
        \expect[
        (\reportval_{i},\reportwealth_{i})
        \sim (\randomreportval_{i}, \randomreportwealth_{i}),
        (\reportval_{-i},\reportwealth_{-i})
        \sim (\randomreportval_{-i}, \randomreportwealth_{-i})
        ]
        {\util_i(\reportval_i, \reportwealth_i, \reportval_{-i}, \reportwealth_{-i})}
        \geq
        \expect[
        (\reportval_{-i},\reportwealth_{-i})
        \sim (\randomreportval_{-i}, \randomreportwealth_{-i})
        ]{
        \util_i(\reportval_i\primed, \reportwealth_i\primed, \reportval_{-i}, \reportwealth_{-i})
        }
    \end{align*}
\end{definition}

We also study the Bayesian setting
for the metagame where agents' utility models
$\{(\ctri, \valuefunctioni, \truewealthi, \moneycosti)\}_{i\in[n]}$
are drawn from prior distributions $\{\typedist_i\}_{i\in[n]}$ independently.
In this setting, a strategy $\strategy_i$ of agent $i$ is a stochastic 
mapping from agent $i$'s realized utility model 
$(\ctri, \valuefunctioni, \truewealthi, \moneycosti)$
to a randomized message $(\randomreportval_i, \randomreportwealth_i)$.
We consider the \emph{Bayesian Nash equilibrium} in this setting.

\begin{definition}[Bayesian Nash equilibrium]
For agents with prior distributions $\{\typedist_i\}_{i\in[n]}$,
a Bayesian Nash equilibrium is a strategy profile $\{\strategy_i\}_{i\in[n]}$
such that for every agent $i$, every realized utility model 
$(\ctri, \valuefunctioni, \truewealthi, \moneycosti)$,
and every message 
$(\reportval_i\primed, \reportwealth_i\primed)\in (\realsinf)^2$,
\begin{align*}
    \expect[ (\reportval_{i},\reportwealth_{i})
        \sim
        \strategy_i(\ctri, \valuefunctioni, \truewealthi, \moneycosti)]{
    \expect[(\ctr_{-i}, \valuefunction_{-i}, \truewealth_{-i}, \moneycost_{-i})
    \sim F_{-i}]
    {
    \expect[ (\reportval_{-i},\reportwealth_{-i})
        \sim
        \strategy_{-i}(\ctr_{-i}, \valuefunction_{-i}, \truewealth_{-i}, \moneycost_{-i})]
        {\util_i(\reportval_i, \reportwealth_i, \reportval_{-i}, \reportwealth_{-i})}
    }
    }
    \\
    \geq 
    \expect[(\ctr_{-i}, \valuefunction_{-i}, \truewealth_{-i}, \moneycost_{-i})
    \sim F_{-i}]
    {
    \expect[ (\reportval_{-i},\reportwealth_{-i})
        \sim
        \strategy_{-i}(\ctr_{-i}, \valuefunction_{-i}, \truewealth_{-i}, \moneycost_{-i})]
        {\util_i(\reportval_i\primed, \reportwealth_i\primed, \reportval_{-i}, \reportwealth_{-i})}
    }
\end{align*}
\end{definition}

\begin{remark}
    By definition, every pure Nash equilibrium is also a mixed Nash equilibrium;
and every mixed Nash equilibrium is also a Bayesian Nash equilibrium.\footnote{To see this, note that every problem instances where agents' utility models are fixed 
is equivalent to a problem instances where agents' utility models are drawn from 
single point-mass distribution in the Bayesian setting.}
\end{remark}

\paragraph{Transferable welfare and price of anarchy.}
We evaluate the performance of 
the metagame by its \emph{price of anarchy} with respect to 
the \emph{transferable welfare}.

\begin{definition}[Transferable welfare]
    For agents with utility models $\{(\ctri, \valuefunctioni, \truewealthi, \moneycosti)\}_{i\in[n]}$,
the \emph{transferable welfare} of a (possibly) 
randomized allocation $\randomalloc$
is 
\begin{align*}
    \twelfare^{\{(\ctri, \valuefunctioni, \truewealthi, \moneycosti)\}_{i\in[n]}}(\randomalloc) \triangleq \sum_{i\in[n]} \wtp_i(\randomalloc_i)
\end{align*}
where $\wtp_i(\randomalloc_i)$
is
agent $i$'s \emph{willingness to pay} for allocation $\randomalloc_i$
defined as
\begin{align*}
  \wtp^{(\ctri, \valuefunctioni, \truewealthi, \moneycosti)}_i(\randomalloc_i) \triangleq \min\left\{\truewealthi, 
\moneycost_i^{-1}\left( 
\expect[\alloci\sim\randomalloc_{i}]{
\valuefunctioni\left(\sum_{j\in[n]}
\ctrij\allocij \right)}
\right)
\right)\}
\end{align*}
\end{definition}
Our definition of the transferable welfare
recovers the classic definition of welfare and liquid welfare
for linear agents and budgeted agents respectively \citep{vic-61,DP-14}.
Moreover, among all feasible randomized allocations,
the optimal allocation maximizing the transferable welfare
is deterministic, since valuation function $\valuefunctioni$
is weakly concave.
With slight abuse of notation, in the Bayesian setting, 
we write $\twelfare(\strategy)$
as the expected transferable welfare for strategy profile $\strategy$,
i.e.,
\begin{align*}
    \twelfare(\strategy) \triangleq
    \sum_{i\in[n]}
    \expect[(\ctr_i, \valuefunc_i, \truewealth_i, \moneycost_i)
        \sim F_i]{
        \wtp_i(\randomalloci(\strategy_i(\ctr_i, \valuefunc_i, \truewealth_i, \moneycost_i), F_{-i}, \strategy_{-i}))}
\end{align*}
where $\randomalloci(\strategy_i(\ctr_i, \valuefunc_i, \truewealth_i, \moneycost_i), F_{-i}, \strategy_{-i}))$
is the randomized allocation of agent $i$ with realized utility model
$(\ctr_i, \valuefunc_i, \truewealth_i, \moneycost_i)$
computed in the interim stage, i.e.,
the randomness is taken over agent $i$'s strategy
and other agents' utility models as well as their strategies.

Given the definition of transferable welfare, 
we evaluate the performance of the metagame
by considering the approximation of transferable welfare
between the worst allocation
in all possible equilibrium with the optimal allocation and 
taking the infimum over all instances. 
\begin{definition}[Price of anarchy]
    The \emph{price of anarchy} of the metagame $\purePoA$
    (resp.\ $\mixedPoA$, $\BayesPoA$)
    under pure Nash equilibrium (resp.\ mixed Nash equilibrium, 
    Bayesian Nash equilibrium) is 
    \begin{align*}
        \purePoA \triangleq 
        \inf_{n, m}
        \inf_{\{\ctri, \valuefunctioni, \truewealthi, \moneycosti\}_{i\in[n]}}
        \frac{\inf_{\alloc \in \texttt{Pure}}\twelfare(\alloc)}{\max_{\alloc}\twelfare(\alloc)},
        \quad
        \mixedPoA \triangleq 
        \inf_{n, m}
        \inf_{\{\ctri, \valuefunctioni, \truewealthi, \moneycosti\}_{i\in[n]}}
        \frac{\inf_{\randomalloc \in \texttt{Mixed}}\twelfare(\randomalloc)}{\max_{\alloc}\twelfare(\alloc)}
        \\
        \BayesPoA\triangleq
        \inf_{n, m}
        \inf_{\{\typedist_i\}_{i\in[n]}}
        \frac{\inf_{\strategy \in \texttt{Bayes}}\twelfare(\strategy)}
        {\expect[\{\ctri, \valuefunctioni, \truewealthi, \moneycosti\}_{i\in[n]}
        \sim \{F_i\}_{i\in[n]}]
        {\max_{\alloc}\twelfare(\alloc)}}
    \end{align*}
\end{definition}

